Coherent Direct D-MIMO Localization: Analysis of Coherence Levels

Distributed multiple-input multiple-output (D-MIMO) offers favorable geometry for localization and sensing, with its greatest potential arising from joint coherent processing across panels. However, stringent frequency-synchronization and phase-calibration requirements, together with multimodal likelihood functions, complicate the estimation problem. Consequently, most existing methods process the panels noncoherently, potentially sacrificing localization accuracy. We present a unified family of Bayesian state filters based on concentrated Type-I and marginal Type-II likelihoods for wideband near-field D-MIMO systems. The Type-I filters realize (i) noncoherent, (ii) coherent, and (iii) carrier-phase-based processing. We show that a zero-mean Type-II model is inherently noncoherent under distributed processing, whereas observation stacking restores coherence. A recently proposed nonzero-mean Type-II model adapts to the coherence available in the data, a property termed ``soft coherence.'' We derive posterior Cram\'er--Rao lower bounds (PCRLBs) for all three coherence levels and show that each level is fundamentally tied to the number of phase parameters used for positioning or treated as nuisance parameters. Numerical results show that the filters closely approach their respective PCRLBs and that coherent processing substantially outperforms noncoherent processing. Our particle-based implementations parallelize over particles and panels, scale linearly with the observed data, and achieve runtimes of tens of milliseconds per time step under GPU acceleration.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}
@STRING{IEEE_J_OJSP = "{IEEE} Open J. Signal Process."}
@STRING{IEEE_J_OJCOMS = "{IEEE} Open J. Commun. Soc."}

==> figures/LHFs/arrays2D.tex <==
\node[centered, align=center, inner sep=0]
at (axis cs:-1.2,-0.8) {$\scriptscriptstyle j=1$};

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.881915592841427	-1.00978122699779\\
-1.07105077423031	-0.949736844031735\\
-1.11809224049191	-0.990248007400201\\
-0.928957059103024	-1.05029239036626\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.889052091841427	-1.03641500385396\\
-1.07818727323031	-0.9763706208879\\
-1.12522873949191	-1.01688178425637\\
-0.936093558103024	-1.07692616722242\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.889052091841427	-1.03641500385396\\
-1.07818727323031	-0.9763706208879\\
-1.07105077423031	-0.949736844031735\\
-0.881915592841427	-1.00978122699779\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.936093558103024	-1.07692616722242\\
-1.12522873949191	-1.01688178425637\\
-1.11809224049191	-0.990248007400201\\
-0.928957059103024	-1.05029239036626\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.889052091841427	-1.03641500385396\\
-0.936093558103024	-1.07692616722242\\
-0.928957059103024	-1.05029239036626\\
-0.881915592841427	-1.00978122699779\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-1.07818727323031	-0.9763706208879\\
-1.12522873949191	-1.01688178425637\\
-1.11809224049191	-0.990248007400201\\
-1.07105077423031	-0.949736844031735\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.905780592692628	-1.00779250781819\\
-0.935961738658939	-0.998210957344881\\
-0.943468355615577	-1.00467550469091\\
-0.913287209649266	-1.01425705516422\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.915789415301478	-1.01641190427956\\
-0.945970561267789	-1.00683035380626\\
-0.953477178224427	-1.01329490115229\\
-0.923296032258116	-1.0228764516256\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.925798237910329	-1.02503130074094\\
-0.95597938387664	-1.01544975026763\\
-0.963486000833278	-1.02191429761366\\
-0.933304854866967	-1.03149584808697\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.935807060519179	-1.03365069720231\\
-0.96598820648549	-1.02406914672901\\
-0.973494823442128	-1.03053369407504\\
-0.943313677475817	-1.04011524454835\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.946022120647709	-0.995017107187112\\
-0.97620326661402	-0.985435556713805\\
-0.983709883570658	-0.991900104059837\\
-0.953528737604347	-1.00148165453314\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.956030943256559	-1.00363650364849\\
-0.986212089222871	-0.994054953175181\\
-0.993718706179509	-1.00051950052121\\
-0.963537560213197	-1.01010105099452\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.96603976586541	-1.01225590010986\\
-0.996220911831721	-1.00267434963656\\
-1.00372752878836	-1.00913889698259\\
-0.973546382822048	-1.0187204474559\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.976048588474261	-1.02087529657124\\
-1.00622973444057	-1.01129374609793\\
-1.01373635139721	-1.01775829344396\\
-0.983555205430899	-1.02733984391727\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.98626364860279	-0.982241706556036\\
-1.0164447945691	-0.972660156082729\\
-1.02395141152574	-0.979124703428761\\
-0.993770265559428	-0.988706253902068\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.996272471211641	-0.990861103017412\\
-1.02645361717795	-0.981279552544105\\
-1.03396023413459	-0.987744099890137\\
-1.00377908816828	-0.997325650363444\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-1.00628129382049	-0.999480499478787\\
-1.0364624397868	-0.989898949005481\\
-1.04396905674344	-0.996363496351512\\
-1.01378791077713	-1.00594504682482\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-1.01629011642934	-1.00809989594016\\
-1.04647126239565	-0.998518345466856\\
-1.05397787935229	-1.00498289281289\\
-1.02379673338598	-1.01456444328619\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-1.02650517655787	-0.96946630592496\\
-1.05668632252418	-0.959884755451653\\
-1.06419293948082	-0.966349302797685\\
-1.03401179351451	-0.975930853270992\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-1.03651399916672	-0.978085702386336\\
-1.06669514513303	-0.968504151913029\\
-1.07420176208967	-0.974968699259061\\
-1.04402061612336	-0.984550249732368\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-1.04652282177557	-0.986705098847712\\
-1.07670396774188	-0.977123548374405\\
-1.08421058469852	-0.983588095720436\\
-1.05402943873221	-0.993169646193743\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-1.05653164438442	-0.995324495309087\\
-1.08671279035073	-0.98574294483578\\
-1.09421940730737	-0.992207492181812\\
-1.06403826134106	-1.00178904265512\\
}--cycle;
\node[centered, align=center, inner sep=0]
at (axis cs:-0.4,-0.8) {$\scriptscriptstyle j=2$};



\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.4631615156566	-1.00001566666667\\
-0.6374830952434	-1.00001566666667\\
-0.5368384843434	-1.00001566666667\\
-0.3625169047566	-1.00001566666667\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.4631615156566	-1.02856166266667\\
-0.6374830952434	-1.02856166266667\\
-0.5368384843434	-1.02856166266667\\
-0.3625169047566	-1.02856166266667\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.4631615156566	-1.02856166266667\\
-0.6374830952434	-1.02856166266667\\
-0.6374830952434	-1.00001566666667\\
-0.4631615156566	-1.00001566666667\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.3625169047566	-1.02856166266667\\
-0.5368384843434	-1.02856166266667\\
-0.5368384843434	-1.00001566666667\\
-0.3625169047566	-1.00001566666667\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.4631615156566	-1.02856166266667\\
-0.3625169047566	-1.02856166266667\\
-0.3625169047566	-1.00001566666667\\
-0.4631615156566	-1.00001566666667\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
-0.6374830952434	-1.02856166266667\\
-0.5368384843434	-1.02856166266667\\
-0.5368384843434	-1.00001566666667\\
-0.6374830952434	-1.00001566666667\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.470607592279202	-1\\
-0.498424865617521	-1\\
-0.482364555367521	-1\\
-0.454547282029202	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.449193845279202	-1\\
-0.477011118617521	-1\\
-0.460950808367521	-1\\
-0.433133535029202	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.427780098279202	-1\\
-0.455597371617521	-1\\
-0.439537061367521	-1\\
-0.411719788029202	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.406366351279202	-1\\
-0.434183624617521	-1\\
-0.418123314367521	-1\\
-0.390306041029202	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.507697290063628	-1\\
-0.535514563401947	-1\\
-0.519454253151947	-1\\
-0.491636979813628	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.486283543063628	-1\\
-0.514100816401947	-1\\
-0.498040506151947	-1\\
-0.470223232813628	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.464869796063628	-1\\
-0.492687069401947	-1\\
-0.476626759151947	-1\\
-0.448809485813628	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.443456049063628	-1\\
-0.471273322401947	-1\\
-0.455213012151947	-1\\
-0.427395738813628	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.544786987848053	-1\\
-0.572604261186372	-1\\
-0.556543950936372	-1\\
-0.528726677598053	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.523373240848053	-1\\
-0.551190514186372	-1\\
-0.535130203936372	-1\\
-0.507312930598053	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.501959493848053	-1\\
-0.529776767186372	-1\\
-0.513716456936372	-1\\
-0.485899183598053	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.480545746848053	-1\\
-0.508363020186372	-1\\
-0.492302709936372	-1\\
-0.464485436598053	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.581876685632479	-1\\
-0.609693958970798	-1\\
-0.593633648720798	-1\\
-0.565816375382479	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.560462938632479	-1\\
-0.588280211970798	-1\\
-0.572219901720798	-1\\
-0.544402628382479	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.539049191632479	-1\\
-0.566866464970798	-1\\
-0.550806154720798	-1\\
-0.522988881382479	-1\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
-0.517635444632479	-1\\
-0.545452717970798	-1\\
-0.529392407720798	-1\\
-0.501575134382479	-1\\
}--cycle;
\node[centered, align=center, inner sep=0]
at (axis cs:0.4,-0.8) {$\scriptscriptstyle j=3$};

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.596083465913306	-0.965327198861593\\
0.397852279686872	-1.00028070541116\\
0.403921892402273	-1.03470318965613\\
0.602153078628707	-0.999749683106568\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.600965118734953	-0.993012427758685\\
0.402733932508519	-1.02796593430825\\
0.40880354522392	-1.06238841855322\\
0.607034731450354	-1.02743491200366\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.600965118734953	-0.993012427758685\\
0.402733932508519	-1.02796593430825\\
0.397852279686872	-1.00028070541116\\
0.596083465913306	-0.965327198861593\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.607034731450354	-1.02743491200366\\
0.40880354522392	-1.06238841855322\\
0.403921892402273	-1.03470318965613\\
0.602153078628707	-0.999749683106568\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.600965118734953	-0.993012427758685\\
0.607034731450354	-1.02743491200366\\
0.602153078628707	-0.999749683106568\\
0.596083465913306	-0.965327198861593\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.402733932508519	-1.02796593430825\\
0.40880354522392	-1.06238841855322\\
0.403921892402273	-1.03470318965613\\
0.397852279686872	-1.00028070541116\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.57666020219855	-0.972323407927711\\
0.545027566098587	-0.977901095143067\\
0.54599612131913	-0.983394044756626\\
0.577628757419093	-0.97781635754127\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.577951609159274	-0.97964734074579\\
0.546318973059311	-0.985225027961146\\
0.547287528279854	-0.990717977574706\\
0.578920164379817	-0.98514029035935\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.579243016119998	-0.98697127356387\\
0.547610380020035	-0.992548960779226\\
0.548578935240578	-0.998041910392786\\
0.58021157134054	-0.99246422317743\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.580534423080721	-0.994295206381949\\
0.548901786980758	-0.999872893597305\\
0.549870342201301	-1.00536584321087\\
0.581502978301264	-0.999788155995509\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.534483354065266	-0.979760324214852\\
0.502850717965304	-0.985338011430208\\
0.503819273185846	-0.990830961043768\\
0.535451909285809	-0.985253273828412\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.53577476102599	-0.987084257032932\\
0.504142124926027	-0.992661944248288\\
0.50511068014657	-0.998154893861847\\
0.536743316246533	-0.992577206646491\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.537066167986714	-0.994408189851011\\
0.505433531886751	-0.999985877066367\\
0.506402087107294	-1.00547882667993\\
0.538034723207257	-0.999901139464571\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.538357574947437	-1.00173212266909\\
0.506724938847475	-1.00730980988445\\
0.507693494068017	-1.01280275949801\\
0.53932613016798	-1.00722507228265\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.492306505931983	-0.987197240501993\\
0.46067386983202	-0.992774927717349\\
0.461642425052563	-0.998267877330909\\
0.493275061152525	-0.992690190115553\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.493597912892706	-0.994521173320073\\
0.461965276792744	-1.00009886053543\\
0.462933832013286	-1.00559181014899\\
0.494566468113249	-1.00001412293363\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.49488931985343	-1.00184510613815\\
0.463256683753467	-1.00742279335351\\
0.46422523897401	-1.01291574296707\\
0.495857875073973	-1.00733805575171\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.496180726814154	-1.00916903895623\\
0.464548090714191	-1.01474672617159\\
0.465516645934733	-1.02023967578515\\
0.497149282034696	-1.01466198856979\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.450129657798699	-0.994634156789135\\
0.418497021698736	-1.00021184400449\\
0.419465576919279	-1.00570479361805\\
0.451098213019242	-1.00012710640269\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.451421064759423	-1.00195808960721\\
0.41978842865946	-1.00753577682257\\
0.420756983880002	-1.01302872643613\\
0.452389619979965	-1.00745103922077\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.452712471720146	-1.00928202242529\\
0.421079835620183	-1.01485970964065\\
0.422048390840726	-1.02035265925421\\
0.453681026940689	-1.01477497203885\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.45400387868087	-1.01660595524337\\
0.422371242580907	-1.02218364245873\\
0.42333979780145	-1.02767659207229\\
0.454972433901412	-1.02209890485693\\
}--cycle;
\node[centered, align=center, inner sep=0]
at (axis cs:1.2,-0.8) {$\scriptscriptstyle j=4$};

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.11809224049191	-0.990248007400201\\
0.928957059103024	-1.05029239036626\\
0.881915592841427	-1.00978122699779\\
1.07105077423031	-0.949736844031735\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.12522873949191	-1.01688178425637\\
0.936093558103024	-1.07692616722242\\
0.889052091841427	-1.03641500385396\\
1.07818727323031	-0.9763706208879\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.12522873949191	-1.01688178425637\\
0.936093558103024	-1.07692616722242\\
0.928957059103024	-1.05029239036626\\
1.11809224049191	-0.990248007400201\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.07818727323031	-0.9763706208879\\
0.889052091841427	-1.03641500385396\\
0.881915592841427	-1.00978122699779\\
1.07105077423031	-0.949736844031735\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
1.12522873949191	-1.01688178425637\\
1.07818727323031	-0.9763706208879\\
1.07105077423031	-0.949736844031735\\
1.11809224049191	-0.990248007400201\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEblue, fill=IEEEblue, fill opacity=0.3, forget plot]
table[row sep=crcr] {%
x	y\\
0.936093558103024	-1.07692616722242\\
0.889052091841427	-1.03641500385396\\
0.881915592841427	-1.00978122699779\\
0.928957059103024	-1.05029239036626\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.09421940730737	-0.992207492181812\\
1.06403826134106	-1.00178904265512\\
1.05653164438442	-0.995324495309087\\
1.08671279035073	-0.98574294483578\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.08421058469852	-0.983588095720436\\
1.05402943873221	-0.993169646193743\\
1.04652282177557	-0.986705098847712\\
1.07670396774188	-0.977123548374405\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.07420176208967	-0.974968699259061\\
1.04402061612336	-0.984550249732368\\
1.03651399916672	-0.978085702386336\\
1.06669514513303	-0.968504151913029\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.06419293948082	-0.966349302797685\\
1.03401179351451	-0.975930853270992\\
1.02650517655787	-0.96946630592496\\
1.05668632252418	-0.959884755451653\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.05397787935229	-1.00498289281289\\
1.02379673338598	-1.01456444328619\\
1.01629011642934	-1.00809989594016\\
1.04647126239565	-0.998518345466856\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.04396905674344	-0.996363496351512\\
1.01378791077713	-1.00594504682482\\
1.00628129382049	-0.999480499478787\\
1.0364624397868	-0.989898949005481\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.03396023413459	-0.987744099890137\\
1.00377908816828	-0.997325650363444\\
0.996272471211641	-0.990861103017412\\
1.02645361717795	-0.981279552544105\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.02395141152574	-0.979124703428761\\
0.993770265559428	-0.988706253902068\\
0.98626364860279	-0.982241706556036\\
1.0164447945691	-0.972660156082729\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.01373635139721	-1.01775829344396\\
0.983555205430899	-1.02733984391727\\
0.976048588474261	-1.02087529657124\\
1.00622973444057	-1.01129374609793\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
1.00372752878836	-1.00913889698259\\
0.973546382822048	-1.0187204474559\\
0.96603976586541	-1.01225590010986\\
0.996220911831721	-1.00267434963656\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.993718706179509	-1.00051950052121\\
0.963537560213197	-1.01010105099452\\
0.956030943256559	-1.00363650364849\\
0.986212089222871	-0.994054953175181\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.983709883570658	-0.991900104059837\\
0.953528737604347	-1.00148165453314\\
0.946022120647709	-0.995017107187112\\
0.97620326661402	-0.985435556713805\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.973494823442128	-1.03053369407504\\
0.943313677475817	-1.04011524454835\\
0.935807060519179	-1.03365069720231\\
0.96598820648549	-1.02406914672901\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.963486000833278	-1.02191429761366\\
0.933304854866967	-1.03149584808697\\
0.925798237910329	-1.02503130074094\\
0.95597938387664	-1.01544975026763\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.953477178224427	-1.01329490115229\\
0.923296032258116	-1.0228764516256\\
0.915789415301478	-1.01641190427956\\
0.945970561267789	-1.00683035380626\\
}--cycle;

\addplot[area legend, line width=0.1pt, draw=IEEEorange, fill=white!50!IEEEorange, forget plot]
table[row sep=crcr] {%
x	y\\
0.943468355615577	-1.00467550469091\\
0.913287209649266	-1.01425705516422\\
0.905780592692628	-1.00779250781819\\
0.935961738658939	-0.998210957344881\\
}--cycle;


==> figures/LHFs/trajectory.tex <==
\addplot [
color=black, 
only marks, 
mark size=0.2pt, 
mark=*, 
mark size = 0.02pt, 
mark size=0.1pt,
mark options={solid, line width=0pt,fill=black}
]
  table[row sep=crcr]{%
-1	0.25\\
-0.987437185929648	0.25929648241206\\
-0.974874371859296	0.268592964824121\\
-0.962311557788945	0.277889447236181\\
-0.949748743718593	0.287185929648241\\
-0.937185929648241	0.296482412060302\\
-0.924623115577889	0.305778894472362\\
-0.912060301507538	0.315075376884422\\
-0.899497487437186	0.324371859296482\\
-0.886934673366834	0.333668341708543\\
-0.874371859296482	0.342964824120603\\
-0.861809045226131	0.352261306532663\\
-0.849246231155779	0.361557788944724\\
-0.836683417085427	0.370854271356784\\
-0.824120603015075	0.380150753768844\\
-0.811557788944724	0.389447236180904\\
-0.798994974874372	0.398743718592965\\
-0.78643216080402	0.408040201005025\\
-0.773869346733668	0.417336683417085\\
-0.761306532663317	0.426633165829146\\
-0.748743718592965	0.435929648241206\\
-0.736180904522613	0.445226130653266\\
-0.723618090452261	0.454522613065327\\
-0.71105527638191	0.463819095477387\\
-0.698492462311558	0.473115577889447\\
-0.685929648241206	0.482412060301508\\
-0.673366834170854	0.491708542713568\\
-0.660804020100503	0.501005025125628\\
-0.648241206030151	0.510301507537688\\
-0.635678391959799	0.519597989949749\\
-0.623115577889447	0.528894472361809\\
-0.610552763819096	0.538190954773869\\
-0.597989949748744	0.54748743718593\\
-0.585427135678392	0.55678391959799\\
-0.57286432160804	0.56608040201005\\
-0.560301507537688	0.575376884422111\\
-0.547738693467337	0.584673366834171\\
-0.535175879396985	0.593969849246231\\
-0.522613065326633	0.603266331658291\\
-0.510050251256281	0.612562814070352\\
-0.49748743718593	0.621859296482412\\
-0.484924623115578	0.631155778894472\\
-0.472361809045226	0.640452261306533\\
-0.459798994974874	0.649748743718593\\
-0.447236180904523	0.659045226130653\\
-0.434673366834171	0.668341708542714\\
-0.422110552763819	0.677638190954774\\
-0.409547738693467	0.686934673366834\\
-0.396984924623116	0.696231155778894\\
-0.384422110552764	0.705527638190955\\
-0.371859296482412	0.714824120603015\\
-0.35929648241206	0.724120603015075\\
-0.346733668341708	0.733417085427136\\
-0.334170854271357	0.742713567839196\\
-0.321608040201005	0.752010050251256\\
-0.309045226130653	0.761306532663317\\
-0.296482412060302	0.770603015075377\\
-0.28391959798995	0.779899497487437\\
-0.271356783919598	0.789195979899498\\
-0.258793969849246	0.798492462311558\\
-0.246231155778895	0.807788944723618\\
-0.233668341708543	0.817085427135678\\
-0.221105527638191	0.826381909547739\\
-0.208542713567839	0.835678391959799\\
-0.195979899497487	0.844974874371859\\
-0.183417085427136	0.85427135678392\\
-0.170854271356784	0.86356783919598\\
-0.158291457286432	0.87286432160804\\
-0.14572864321608	0.8821608040201\\
-0.133165829145729	0.891457286432161\\
-0.120603015075377	0.900753768844221\\
-0.108040201005025	0.910050251256281\\
-0.0954773869346733	0.919346733668342\\
-0.0829145728643217	0.928643216080402\\
-0.0703517587939698	0.937939698492462\\
-0.0577889447236181	0.947236180904523\\
-0.0452261306532664	0.956532663316583\\
-0.0326633165829145	0.965829145728643\\
-0.0201005025125629	0.975125628140703\\
-0.00753768844221103	0.984422110552764\\
0.00502512562814084	0.993718592964824\\
0.0175879396984924	1.00301507537688\\
0.0301507537688441	1.01231155778894\\
0.0427135678391959	1.02160804020101\\
0.0552763819095476	1.03090452261307\\
0.0678391959798996	1.04020100502513\\
0.0804020100502512	1.04949748743719\\
0.0929648241206031	1.05879396984925\\
0.105527638190955	1.06809045226131\\
0.118090452261306	1.07738693467337\\
0.130653266331658	1.08668341708543\\
0.14321608040201	1.09597989949749\\
0.155778894472362	1.10527638190955\\
0.168341708542714	1.11457286432161\\
0.180904522613065	1.12386934673367\\
0.193467336683417	1.13316582914573\\
0.206030150753769	1.14246231155779\\
0.218592964824121	1.15175879396985\\
0.231155778894472	1.16105527638191\\
0.243718592964824	1.17035175879397\\
0.256281407035176	1.17964824120603\\
0.268844221105528	1.18894472361809\\
0.281407035175879	1.19824120603015\\
0.293969849246231	1.20753768844221\\
0.306532663316583	1.21683417085427\\
0.319095477386935	1.22613065326633\\
0.331658291457286	1.23542713567839\\
0.344221105527638	1.24472361809045\\
0.35678391959799	1.25402010050251\\
0.369346733668342	1.26331658291457\\
0.381909547738693	1.27261306532663\\
0.394472361809045	1.28190954773869\\
0.407035175879397	1.29120603015075\\
0.419597989949749	1.30050251256281\\
0.432160804020101	1.30979899497487\\
0.444723618090452	1.31909547738693\\
0.457286432160804	1.328391959799\\
0.469849246231156	1.33768844221106\\
0.482412060301508	1.34698492462312\\
0.494974874371859	1.35628140703518\\
0.507537688442211	1.36557788944724\\
0.520100502512563	1.3748743718593\\
0.532663316582914	1.38417085427136\\
0.545226130653266	1.39346733668342\\
0.557788944723618	1.40276381909548\\
0.57035175879397	1.41206030150754\\
0.582914572864321	1.4213567839196\\
0.595477386934673	1.43065326633166\\
0.608040201005025	1.43994974874372\\
0.620603015075377	1.44924623115578\\
0.633165829145729	1.45854271356784\\
0.64572864321608	1.4678391959799\\
0.658291457286432	1.47713567839196\\
0.670854271356784	1.48643216080402\\
0.683417085427136	1.49572864321608\\
0.695979899497488	1.50502512562814\\
0.708542713567839	1.5143216080402\\
0.721105527638191	1.52361809045226\\
0.733668341708543	1.53291457286432\\
0.746231155778895	1.54221105527638\\
0.758793969849246	1.55150753768844\\
0.771356783919598	1.5608040201005\\
0.78391959798995	1.57010050251256\\
0.796482412060302	1.57939698492462\\
0.809045226130653	1.58869346733668\\
0.821608040201005	1.59798994974874\\
0.834170854271357	1.6072864321608\\
0.846733668341709	1.61658291457286\\
0.85929648241206	1.62587939698492\\
0.871859296482412	1.63517587939699\\
0.884422110552764	1.64447236180905\\
0.896984924623115	1.65376884422111\\
0.909547738693467	1.66306532663317\\
0.922110552763819	1.67236180904523\\
0.934673366834171	1.68165829145729\\
0.947236180904523	1.69095477386935\\
0.959798994974874	1.70025125628141\\
0.972361809045226	1.70954773869347\\
0.984924623115578	1.71884422110553\\
0.99748743718593	1.72814070351759\\
1.01005025125628	1.73743718592965\\
1.02261306532663	1.74673366834171\\
1.03517587939698	1.75603015075377\\
1.04773869346734	1.76532663316583\\
1.06030150753769	1.77462311557789\\
1.07286432160804	1.78391959798995\\
1.08542713567839	1.79321608040201\\
1.09798994974874	1.80251256281407\\
1.1105527638191	1.81180904522613\\
1.12311557788945	1.82110552763819\\
1.1356783919598	1.83040201005025\\
1.14824120603015	1.83969849246231\\
1.1608040201005	1.84899497487437\\
1.17336683417085	1.85829145728643\\
1.18592964824121	1.86758793969849\\
1.19849246231156	1.87688442211055\\
1.21105527638191	1.88618090452261\\
1.22361809045226	1.89547738693467\\
1.23618090452261	1.90477386934673\\
1.24874371859296	1.91407035175879\\
1.26130653266332	1.92336683417085\\
1.27386934673367	1.93266331658291\\
1.28643216080402	1.94195979899497\\
1.29899497487437	1.95125628140704\\
1.31155778894472	1.9605527638191\\
1.32412060301508	1.96984924623116\\
1.33668341708543	1.97914572864322\\
1.34924623115578	1.98844221105528\\
1.36180904522613	1.99773869346734\\
1.37437185929648	2.0070351758794\\
1.38693467336683	2.01633165829146\\
1.39949748743719	2.02562814070352\\
1.41206030150754	2.03492462311558\\
1.42462311557789	2.04422110552764\\
1.43718592964824	2.0535175879397\\
1.44974874371859	2.06281407035176\\
1.46231155778894	2.07211055276382\\
1.4748743718593	2.08140703517588\\
1.48743718592965	2.09070351758794\\
1.5	2.1\\
};

==> figures/geometricModel/AP0.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.38431,0.60784}%
\definecolor{mycolor2}{rgb}{0.88235,0.63922,0.00000}%
%
\begin{tikzpicture}

\tikzset{line cap=round,line join=round}

\pgfdeclarelayer{behindBackground}
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfdeclarelayer{layer1}
\pgfdeclarelayer{layer2}
\pgfdeclarelayer{layer3}
\pgfsetlayers{behindBackground,background,main,layer1,layer2,layer3,foreground}   %% some 

\begin{axis}[%
width=0.655\figurewidth,
height=0.75\figurewidth,
at={(0\figurewidth,0\figurewidth)},
scale only axis,
plot box ratio=1 1.148 1.148,
clip=false,
xmin=-0.0285616626666667,
xmax=0.1675,
tick align=outside,
ymin=-0.1,
ymax=0.125,
zmin=-0.1,
zmax=0.125,
view={110}{27},
%axis background/.style={fill=white},
%axis x line*=bottom,
%axis y line*=left,
%axis z line*=left,
ticks=none,         % [B]
grid=none,          % [B]
%axis lines=center
axis line style={draw=none} % [B]
]
\begin{pgfonlayer}{foreground}
  \addplot3 [color=black,line width=1pt,arrows = {-Stealth[inset=0pt, scale=1.05, angle'=25]}]
   table[row sep=crcr] {%
  0	0	0\\
  0.1675	0	0\\
  };
   \node[align=center, inner sep=0]
  at (axis cs:0.186,0,0) {$x'$};
  \addplot3 [color=black,line width=1pt,arrows = {-Stealth[inset=0pt, scale=1.05, angle'=25]}]
   table[row sep=crcr] {%
  0	0	0\\
  0	0.125	0\\
  };
   \node[align=center, inner sep=0]
  at (axis cs:0,0.137,0) {$y'$};
  \addplot3 [color=black,line width=1pt,arrows = {-Stealth[inset=0pt, scale=1.05, angle'=25]}]
   table[row sep=crcr] {%
  0	0	0\\
  0	0	0.125\\
  };
   \node[align=center, inner sep=0]
  at (axis cs:0,0,0.137) {$z'$};
\end{pgfonlayer}
%\node[centered, align=center, inner sep=0]
%at (axis cs:0,0,0.15) {PA1};

\addplot3[area legend, line width=0.2pt, draw=mycolor1, fill=mycolor1, fill opacity=0.3, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
-1.85e-05	-0.0792308639	-0.0792308639\\
-1.85e-05	0.0792308639	-0.0792308639\\
-1.85e-05	0.0792308639	0.0792308639\\
-1.85e-05	-0.0792308639	0.0792308639\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor1, fill=mycolor1, fill opacity=0.3, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
-0.0285616626666667	-0.0792308639	-0.0792308639\\
-0.0285616626666667	0.0792308639	-0.0792308639\\
-0.0285616626666667	0.0792308639	0.0792308639\\
-0.0285616626666667	-0.0792308639	0.0792308639\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor1, fill=mycolor1, fill opacity=0.3, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
-0.0285616626666667	-0.0792308639	-0.0792308639\\
-0.0285616626666667	0.0792308639	-0.0792308639\\
-1.85e-05	0.0792308639	-0.0792308639\\
-1.85e-05	-0.0792308639	-0.0792308639\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor1, fill=mycolor1, fill opacity=0.3, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
-0.0285616626666667	-0.0792308639	0.0792308639\\
-0.0285616626666667	0.0792308639	0.0792308639\\
-1.85e-05	0.0792308639	0.0792308639\\
-1.85e-05	-0.0792308639	0.0792308639\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor1, fill=mycolor1, fill opacity=0.3, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
-0.0285616626666667	-0.0792308639	-0.0792308639\\
-0.0285616626666667	-0.0792308639	0.0792308639\\
-1.85e-05	-0.0792308639	0.0792308639\\
-1.85e-05	-0.0792308639	-0.0792308639\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor1, fill=mycolor1, fill opacity=0.3, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
-0.0285616626666667	0.0792308639	-0.0792308639\\
-0.0285616626666667	0.0792308639	0.0792308639\\
-1.85e-05	0.0792308639	0.0792308639\\
-1.85e-05	0.0792308639	-0.0792308639\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	-0.05888780425	-0.05888780425\\
0	-0.02676718375	-0.05888780425\\
0	-0.02676718375	-0.02676718375\\
0	-0.05888780425	-0.02676718375\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	-0.05888780425	-0.01606031025\\
0	-0.02676718375	-0.01606031025\\
0	-0.02676718375	0.01606031025\\
0	-0.05888780425	0.01606031025\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	-0.05888780425	0.02676718375\\
0	-0.02676718375	0.02676718375\\
0	-0.02676718375	0.05888780425\\
0	-0.05888780425	0.05888780425\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	-0.01606031025	-0.05888780425\\
0	0.01606031025	-0.05888780425\\
0	0.01606031025	-0.02676718375\\
0	-0.01606031025	-0.02676718375\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	-0.01606031025	-0.01606031025\\
0	0.01606031025	-0.01606031025\\
0	0.01606031025	0.01606031025\\
0	-0.01606031025	0.01606031025\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	-0.01606031025	0.02676718375\\
0	0.01606031025	0.02676718375\\
0	0.01606031025	0.05888780425\\
0	-0.01606031025	0.05888780425\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	0.02676718375	-0.05888780425\\
0	0.05888780425	-0.05888780425\\
0	0.05888780425	-0.02676718375\\
0	0.02676718375	-0.02676718375\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	0.02676718375	-0.01606031025\\
0	0.05888780425	-0.01606031025\\
0	0.05888780425	0.01606031025\\
0	0.02676718375	0.01606031025\\
}--cycle;

\addplot3[area legend, line width=0.2pt, draw=mycolor2, fill=white!50!mycolor2, line cap=round,line join=round,forget plot]
table[row sep=crcr] {%
x	y	z\\
0	0.02676718375	0.02676718375\\
0	0.05888780425	0.02676718375\\
0	0.05888780425	0.05888780425\\
0	0.02676718375	0.05888780425\\
}--cycle;
\addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	-0.042827494	0\\
0	-0.042827494	-0.05\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	-0.042827494	-0.05\\
0	0.007172506	-0.1\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0	0\\
0	0	-0.05\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0	-0.05\\
0	0.05	-0.1\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0.042827494	0\\
0	0.042827494	-0.05\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0.042827494	-0.05\\
0	0.092827494	-0.1\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0.007172506	-0.1\\
0	0.110327494	-0.1\\
};
 \node[align=center, inner sep=0]
at (axis cs:0,0.125,-0.1) {$\mathbf{p}_y$};
\addplot3 [color=black, only marks, mark size=1.5pt, mark=*, mark options={solid, black}]
 table[row sep=crcr] {%
0	0	-0.042827494\\
0	0	0\\
0	0	0.042827494\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0	-0.042827494\\
0	-0.05	-0.04282744\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	-0.05	-0.042827494\\
0	-0.1	0.007172506\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0	0\\
0	-0.05	0\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	-0.05	0\\
0	-0.1	0.05\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	0	0.042827494\\
0	-0.05	0.042827494\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	-0.05	0.042827494\\
0	-0.1	0.092827494\\
};
 \addplot3 [color=black, line width=0.3pt]
 table[row sep=crcr] {%
0	-0.1	0.007172506\\
0	-0.1	0.110327494\\
};
 \node[align=center, inner sep=0]
at (axis cs:0,-0.1,0.12) {$\mathbf{p}_z$};
\addplot3 [color=black, only marks, mark size=1.5pt, mark=*, mark options={solid, black}]
 table[row sep=crcr] {%
0	-0.042827494	0\\
0	0	0\\
0	0.042827494	0\\
};
 \end{axis}


\end{tikzpicture}%

==> figures/results/SFV-4plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%



\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\scriptsize},
  tick label style={font=\footnotesize},
}}


%\newcommand{\LWbound}{1pt}
%\newcommand{\LWestimates}{0.5pt}

%\newcommand{\lblMVAest}[1]{RMSE $s\!=\!#1$}
%\newcommand{\lblMVAmeb}[1]{MEB $s\!=\!#1$}
%\newcommand{\lblMVAuncertainty}[1]{Std. dev. $s\!=\!#1$}

\newcommand{\lblMVAest}[1]{RMSE REF}
\newcommand{\lblMVAmeb}[1]{noncoherent MEB}
\newcommand{\lblMVAestc}[1]{RMSE PROP}
\newcommand{\lblMVAmebc}[1]{coherent MEB}
%\newcommand{\lblMVAuncertainty}[1]{Std. dev.}
%\newcommand{\lblMVAuncertainty}[1]{$\interval{#1}$}
\newcommand{\lblMVAuncertainty}[1]{$\interval{50\%}$}

\def\datapath{./figures/data}   % path to data files

\begin{tikzpicture}

\begin{axis}[%
axis line style = thick,	% [B] thick axis lines 
width=0.245\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=1,
xmax=200,
%xlabel style={yshift=2mm},
xlabel={Step $n$},
ymin=0,
ymax=15,
tick align=inside,
ytick = {0,2,...,15},
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 3, 
    major grid style={very thin, lightgray!30},
ylabel={$\lVert \psfv{\,k}{n}{J}  - \psfvHat{s}{n}{J} \rVert$ in \SI{}{\centi\metre}},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\def\sSFVcolor{IEEEblue}        % color for current SFV
\def\sIndex{1}                  % index of current SFV

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAest{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAmeb{\sIndex}}
    
\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAestc{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAmebc{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAuncertainty{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh1.dat};%

\node[below, align=center,%
    rectangle,inner sep=0.5pt,rounded corners=0.65mm,minimum size=0.7em,
          fill=\sSFVcolor,
          text=white] at (axis cs:20,14.5) {\adjustbox{max width=0.65em}{$\scriptstyle\sIndex$}};
          %\label{pgf:sfv1}
\end{axis}

\begin{axis}[%
axis line style = thick,	% [B] thick axis lines 
width=0.245\figurewidth,
height=\figureheight,
at={(0.25\figurewidth,0\figureheight)},
scale only axis,
xmin=1,
xmax=200,
%xlabel style={yshift=2mm},
xlabel={Step $n$},
ymin=0,
ymax=15,
tick align=inside,
ytick = {0,2,...,15},
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 3, 
    major grid style={very thin, lightgray!30},
yticklabel=\empty,                      % [B] remove y-axis annotation
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\def\sSFVcolor{IEEEred}        % color for current SFV
\def\sIndex{2}                  % index of current SFV

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAest{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAmeb{\sIndex}}
    
\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAestc{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAmebc{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAuncertainty{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh1.dat};%

\node[below, align=center,%
    rectangle,inner sep=0.5pt,rounded corners=0.65mm,minimum size=0.7em,
          fill=\sSFVcolor,
          text=white] at (axis cs:20,14.5) {\adjustbox{max width=0.65em}{$\scriptstyle\sIndex$}};

\end{axis}

\begin{axis}[%
axis line style = thick,	% [B] thick axis lines 
width=0.245\figurewidth,
height=\figureheight,
at={(0.5\figurewidth,0\figureheight)},
scale only axis,
xmin=1,
xmax=200,
%xlabel style={yshift=2mm},
xlabel={Step $n$},
ymin=0,
ymax=15,
tick align=inside,
ytick = {0,2,...,15},
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 3, 
    major grid style={very thin, lightgray!30},
yticklabel=\empty,                      % [B] remove y-axis annotation
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\def\sSFVcolor{IEEEgreen}        % color for current SFV
\def\sIndex{3}                  % index of current SFV

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAest{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAmeb{\sIndex}}
    
\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAestc{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAmebc{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAuncertainty{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh1.dat};%

\node[below, align=center,%
    rectangle,inner sep=0.5pt,rounded corners=0.65mm,minimum size=0.7em,
          fill=\sSFVcolor,
          text=white] at (axis cs:20,14.5) {\adjustbox{max width=0.65em}{$\scriptstyle\sIndex$}};
\end{axis}

\begin{axis}[%
axis line style = thick,	% [B] thick axis lines 
width=0.245\figurewidth,
height=\figureheight,
at={(0.75\figurewidth,0\figureheight)},
scale only axis,
xmin=1,
xmax=200,
%xlabel style={yshift=2mm},
xlabel={Step $n$},
ymin=0,
ymax=15,
tick align=inside,
ytick = {0,2,...,15},
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 3, 
    major grid style={very thin, lightgray!30},
yticklabel=\empty,                      % [B] remove y-axis annotation
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\def\sSFVcolor{IEEElightblue}        % color for current SFV
\def\sIndex{4}                  % index of current SFV

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAest{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAmeb{\sIndex}}
    
\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWestimates]%
    table{\datapath/mapping-errors/RMSE-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAestc{\sIndex}}

\addplot [color=\sSFVcolor, line cap = round, line join=round, densely dashed, line width=\LWbound]%
    table{\datapath/mapping-errors/MEB-s\sIndex-coh1.dat};%
    \addlegendentry{\lblMVAmebc{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh0.dat};%
    \addlegendentry{\lblMVAuncertainty{\sIndex}}

\addplot[area legend, draw=none, fill=\sSFVcolor, fill opacity=0.1]%
    table{\datapath/mapping-errors/interval-s\sIndex-coh1.dat};%

\node[below, align=center,%
    rectangle,inner sep=0.5pt,rounded corners=0.65mm,minimum size=0.7em,
          fill=\sSFVcolor,
          text=white] at (axis cs:20,14.5) {\adjustbox{max width=0.65em}{$\scriptstyle\sIndex$}};%\label{pgf:sfv4}
\end{axis}



\end{tikzpicture}%

==> figures/results/scenario-det-rays-background.tex <==

\addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.121431144606923	-0.305973920991947\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.112135907853868	-0.279815295362446\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.102810100110852	-0.253570636950484\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0934535703126276	-0.227239520628721\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.115390696823291	-0.313896027611391\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.106023713566285	-0.287576679154121\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0966257183123387	-0.261170193191485\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0871965567953521	-0.234676136266612\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.10926957279128	-0.32192394192328\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0998297489677462	-0.295441896485149\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.090358462584103	-0.268871587435112\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0808555560825777	-0.242212572767877\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.103066145376365	-0.330059797930529\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0935523620956501	-0.303413045049934\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0840066558587743	-0.276676880512702\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.0744288657222368	-0.249850853538991\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.537886583448956	4	-0.0126620261638558\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.53599994549364	4	-0.00216809897884307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.534118153288	4	0.00829887499868598\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.532241188186827	4	0.0187389994778027\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.526775827752169	4	-0.014823752471844\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.5248999015857	4	-0.00430700177994603\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523028802844864	4	0.00618268556970353\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521162512919582	4	0.0166454139082803\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.515622503264112	4	-0.0169937610315976\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.513757384821553	4	-0.0064540888109369\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.511897075163215	4	0.00405840925911061\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.510041555715506	4	0.0145438381368011\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.504426364873643	4	-0.0191720995323307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.502572150958734	4	-0.00860940713567449\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.500722726865196	4	0.00192599962292006\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.498878074057307	4	0.0124342263338147\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0637884020032	-0.101769000151684\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06213096187395	-0.0861229589818673\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06047771430575	-0.0705164950986124\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.05882864341084	-0.0549494585231152\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0748989533857	-0.103085499152609\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0732359106856	-0.0875170587799596\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.07157705343489	-0.0719878001548322\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.06992236585288	-0.0564975755476025\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08589736415929	-0.1043887105142\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08422891594527	-0.0888971053405379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08256464564711	-0.0734442922747162\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.08090453759173	-0.0580301257915418\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09678532357923	-0.105678834397793\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09511166183643	-0.0902633100936512\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09344217007312	-0.0748861940403021\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.09177683272422	-0.0595473428733455\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.275016741636257	0.318464099554947\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.281649014588661	0.340712214916542\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.288238233874936	0.362815905744093\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.294784817365672	0.384776573794313\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.263426192772478	0.332561041575443\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.27013404172854	0.354889186490687\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.276798100230945	0.377071567897901\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.283418795696495	0.399109608522073\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.251702970525635	0.346819346876548\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.258487694689603	0.369227902953099\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.265227874704238	0.391489338816052\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.271923947806723	0.413605098570382\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.239844783776866	0.361241802019117\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.246707712303528	0.383731148202568\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.253525325589217	0.406071999448667\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.260298070975166	0.428265821663957\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.3227256843839	3.1772743156161	0.22618755589019\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32576102520213	3.17423897479787	0.23510310099458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32881066571741	3.17118933428259	0.244060647838386\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.33187470721861	3.16812529278139	0.253060493931981\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31750185847795	3.18249814152205	0.230991883124655\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32051266836299	3.17948733163701	0.239882530638814\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32353760474344	3.17646239525656	0.248814892407969\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32657676727378	3.17342323272622	0.257789262702725\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31232011633952	3.18767988366048	0.235757506123176\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31530669147439	3.18469330852561	0.244623366872182\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31830722268891	3.18169277731109	0.253530657236472\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.32132180803603	3.17867819196397	0.262479668293158\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31311900349251	3.18688099650749	0.258208407609945\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.31610930858271	3.18389069141729	0.267132175661891\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.991159848539033	0.265789947524383\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.987350755178758	0.280902581875283\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.983519624341664	0.296102650242015\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.979666264226472	0.311390913599003\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.99770580743776	0.273805047871219\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.993934436759458	0.288865559721062\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.990141355626273	0.304012769641958\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.986326376027868	0.319247428430406\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00418719150682	0.28174108054475\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00045298590247	0.296749759735325\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.996697390426655	0.311844410013976\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.992920220766769	0.32702577217777\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.0106049515867	0.289599209787227\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.00690736438431	0.304556345188937\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	1.003188701613	0.3195987335193\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.99944878256747	0.334727105750607\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.565174253005492	-0.219946772743362\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.561583398965443	-0.197491275200431\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.557993766058512	-0.175043414044675\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.554405353661905	-0.152603185381425\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.551447055534443	-0.222117578774727\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.547838493367619	-0.199536291477689\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.544231165208612	-0.176962726227206\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.540625070424547	-0.154396879062932\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.537565631927174	-0.224312773981479\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.533939189238341	-0.201604279721379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.530313993635908	-0.178903594616633\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.526690044476699	-0.156210714639732\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.523527368386541	-0.226532771707029\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.519882870311289	-0.203695629188974\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.51623963260921	-0.180866384417376\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.512597654626605	-0.158045033296036\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.912118731001735	4	-0.016708731386001\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.912576001584169	4	-0.00583533410247139\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.913032269580855	4	0.0050142227820611\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.913487538285504	4	0.0158400175884114\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.901581529845063	4	-0.0165021615844915\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.90204984285177	4	-0.00564109463688522\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.902517130203475	4	0.00519618542569555\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.90298339526593	4	0.0160097566614629\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.891067787574463	4	-0.0162960516676675\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.891547092760417	4	-0.00544728713152698\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.892025349383278	4	0.00537774385359263\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.892502560880158	4	0.0161791190844736\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.880577425937548	4	-0.0160904001014801\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.881067673310735	4	-0.00525391014707255\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.881556849372818	4	0.00555889941115834\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.882044957631581	4	0.0163481061097306\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48638224524632	3.01361775475368	-0.0269007603290558\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48725106831988	3.01274893168012	-0.0154941673743061\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48811859499174	3.01188140500826	-0.00410459460103307\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48898482816137	3.01101517183863	0.00726799605698714\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47946882760321	3.02053117239679	-0.0257063717054005\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48033747843498	3.01966252156502	-0.0143702800433674\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.48120484102663	3.01879515897337	-0.00305100020893773\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.4820709182418	3.0179290817582	0.00825150516898576\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47263934580998	3.02736065419002	-0.0245264841620204\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47350776458132	3.02649223541868	-0.0132600277718489\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47437490326335	3.02562509673665	-0.00201017865785913\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.47524076468436	3.02475923531564	0.00922309987274139\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46589228049144	3.03410771950856	-0.0233608352058118\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46676040957962	3.03323959042038	-0.0121631639239768\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.4676272667155	3.0323727332845	-0.000981899077390547\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.46849285469248	3.03150714530752	0.0101829953647518\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.787528431992443	-0.170473881302008\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.783826995472351	-0.15099594786531\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.780124066348989	-0.131510159957258\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.776419643719339	-0.112016512825924\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.794072405600304	-0.168256201303825\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.790396489233142	-0.148905221131802\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.786719100250862	-0.129546488730641\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.783040237768365	-0.110179999440959\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.800531349343121	-0.166067336982822\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.79688060454599	-0.146841665898882\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.79322840672333	-0.1276083428446\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.789574755007493	-0.10836736325075\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.806906909791271	-0.16390673033458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.803280995058272	-0.14480475589696\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.799653646501292	-0.125695227815348\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.796024863269679	-0.106578141608363\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEEblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.668017536654152	0.308394121583095\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.670277019654357	0.328850481456709\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.672542095904788	0.349357480144355\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.674812786199945	0.36991530591027\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.6534326670454	0.305501297516042\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.655685316523917	0.326056244797117\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.65794357022552	0.346662329421666\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.660207449089842	0.367319742459371\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.638701543091929	0.302579464750271\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.640947107823332	0.323233953068746\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.643198287232844	0.343940084656196\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.645455102404742	0.364698053443761\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.623821953791154	0.299628184746278\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.62606017597274	0.320383181616372\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.62830402274524	0.341190335223985\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-3	0.630553515336993	0.36204984241913\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04227938154491	4	0.239656183297002\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03976177254897	4	0.250054333129968\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03723765163295	4	0.26047937829135\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03470699349902	4	0.270931423265417\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03211014702548	4	0.23770920261751\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02958423893929	4	0.248084974596827\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02705180996657	4	0.258487532678155\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0245128348232	4	0.268916980722096\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02197964962768	4	0.235769638467478\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01944552394739	4	0.246123127488271\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01690486865836	4	0.256503294046329\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01435765849107	4	0.266910241383528\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0118876684334	4	0.233837448550379\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00934540590608	4	0.244168748911575\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00679660528874	4	0.254526618901629\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0042412413273	4	0.264911161148586\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58660640495456	2.91339359504544	0.248675686375164\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58386720830482	2.91613279169517	0.260259659541907\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.58112901607392	2.91887098392608	0.271839385054236\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57839182770948	2.92160817229052	0.283414865248042\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57940846507169	2.92059153492831	0.246088265093267\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57668961253085	2.92331038746915	0.257592217997309\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57397175002286	2.92602824997714	0.269091981894744\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57125487700705	2.92874512299295	0.280587559073209\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.57230988290969	2.92769011709031	0.243536559625293\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56961107573759	2.93038892426241	0.254961590178205\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.5669132445189	2.9330867554811	0.266382489166026\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56421638872432	2.93578361127567	0.277799258829458\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56530861532367	2.93469138467633	0.241019835528246\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.56262956128918	2.93737043871082	0.252367019200635\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.55995146942656	2.94004853057344	0.263710127576012\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
2.55727433921756	2.94272566078244	0.275049162849424\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.646569565148188	0.310217457064253\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.653727408850739	0.33046557935495\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.660861022922039	0.350645160817288\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.667970530181842	0.370756548884028\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.651470344886514	0.305663228148336\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.65857147495637	0.325781932400888\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.665648729843089	0.345832994215716\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.672702229753112	0.36581675415803\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.656305100419357	0.30117035464152\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.663350390066484	0.321161278860841\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.670372151303177	0.341085441499938\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.677370501795982	0.360943176436209\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.661075157054671	0.296737604952891\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.668065459788268	0.316602356364934\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.675032573427637	0.336401209973997\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
4	0.681976613170287	0.35613449314357\\
1.03109047374758	2.31174330286659	0.16865766631995\\
};
























 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
0.912118731001735	4	-0.016708731386001\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
0.912576001584169	4	-0.00583533410247139\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
0.913032269580855	4	0.0050142227820611\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
0.913487538285504	4	0.0158400175884114\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
0.901581529845063	4	-0.0165021615844915\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
0.90204984285177	4	-0.00564109463688522\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
0.902517130203475	4	0.00519618542569555\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
0.90298339526593	4	0.0160097566614629\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
0.891067787574463	4	-0.0162960516676675\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
0.891547092760417	4	-0.00544728713152698\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
0.892025349383278	4	0.00537774385359263\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
0.892502560880158	4	0.0161791190844736\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
0.880577425937548	4	-0.0160904001014801\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
0.881067673310735	4	-0.00525391014707255\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
0.881556849372818	4	0.00555889941115834\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
0.882044957631581	4	0.0163481061097306\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
2.48638224524632	3.01361775475368	-0.0269007603290558\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
2.48725106831988	3.01274893168012	-0.0154941673743061\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
2.48811859499174	3.01188140500826	-0.00410459460103307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
2.48898482816137	3.01101517183863	0.00726799605698714\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
2.47946882760321	3.02053117239679	-0.0257063717054005\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
2.48033747843498	3.01966252156502	-0.0143702800433674\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
2.48120484102663	3.01879515897337	-0.00305100020893773\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
2.4820709182418	3.0179290817582	0.00825150516898576\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
2.47263934580998	3.02736065419002	-0.0245264841620204\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
2.47350776458132	3.02649223541868	-0.0132600277718489\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
2.47437490326335	3.02562509673665	-0.00201017865785913\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
2.47524076468436	3.02475923531564	0.00922309987274139\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
2.46589228049144	3.03410771950856	-0.0233608352058118\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
2.46676040957962	3.03323959042038	-0.0121631639239768\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
2.4676272667155	3.0323727332845	-0.000981899077390547\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
2.46849285469248	3.03150714530752	0.0101829953647518\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
4	0.787528431992443	-0.170473881302008\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
4	0.783826995472351	-0.15099594786531\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
4	0.780124066348989	-0.131510159957258\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
4	0.776419643719339	-0.112016512825924\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
4	0.794072405600304	-0.168256201303825\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
4	0.790396489233142	-0.148905221131802\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
4	0.786719100250862	-0.129546488730641\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
4	0.783040237768365	-0.110179999440959\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
4	0.800531349343121	-0.166067336982822\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
4	0.79688060454599	-0.146841665898882\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
4	0.79322840672333	-0.1276083428446\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
4	0.789574755007493	-0.10836736325075\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
4	0.806906909791271	-0.16390673033458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
4	0.803280995058272	-0.14480475589696\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
4	0.799653646501292	-0.125695227815348\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
4	0.796024863269679	-0.106578141608363\\
};





 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
1.04227938154491	4	0.239656183297002\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
1.03976177254897	4	0.250054333129968\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
1.03723765163295	4	0.26047937829135\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
1.03470699349902	4	0.270931423265417\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
1.03211014702548	4	0.23770920261751\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
1.02958423893929	4	0.248084974596827\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
1.02705180996657	4	0.258487532678155\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
1.0245128348232	4	0.268916980722096\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
1.02197964962768	4	0.235769638467478\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
1.01944552394739	4	0.246123127488271\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
1.01690486865836	4	0.256503294046329\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
1.01435765849107	4	0.266910241383528\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
1.0118876684334	4	0.233837448550379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
1.00934540590608	4	0.244168748911575\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
1.00679660528874	4	0.254526618901629\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
1.0042412413273	4	0.264911161148586\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
2.58660640495456	2.91339359504544	0.248675686375164\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
2.58386720830482	2.91613279169517	0.260259659541907\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
2.58112901607392	2.91887098392608	0.271839385054236\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
2.57839182770948	2.92160817229052	0.283414865248042\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
2.57940846507169	2.92059153492831	0.246088265093267\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
2.57668961253085	2.92331038746915	0.257592217997309\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
2.57397175002286	2.92602824997714	0.269091981894744\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
2.57125487700705	2.92874512299295	0.280587559073209\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
2.57230988290969	2.92769011709031	0.243536559625293\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
2.56961107573759	2.93038892426241	0.254961590178205\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
2.5669132445189	2.9330867554811	0.266382489166026\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
2.56421638872432	2.93578361127567	0.277799258829458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
2.56530861532367	2.93469138467633	0.241019835528246\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
2.56262956128918	2.93737043871082	0.252367019200635\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
2.55995146942656	2.94004853057344	0.263710127576012\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
2.55727433921756	2.94272566078244	0.275049162849424\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
4	0.646569565148188	0.310217457064253\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
4	0.653727408850739	0.33046557935495\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
4	0.660861022922039	0.350645160817288\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
4	0.667970530181842	0.370756548884028\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
4	0.651470344886514	0.305663228148336\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
4	0.65857147495637	0.325781932400888\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
4	0.665648729843089	0.345832994215716\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
4	0.672702229753112	0.36581675415803\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
4	0.656305100419357	0.30117035464152\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
4	0.663350390066484	0.321161278860841\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
4	0.670372151303177	0.341085441499938\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
4	0.677370501795982	0.360943176436209\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
4	0.661075157054671	0.296737604952891\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
4	0.668065459788268	0.316602356364934\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
4	0.675032573427637	0.336401209973997\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
4	0.681976613170287	0.35613449314357\\
};

==> figures/results/scenario-det-rays-foreground.tex <==

\addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
-3	0.121431144606923	-0.305973920991947\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
-3	0.112135907853868	-0.279815295362446\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
-3	0.102810100110852	-0.253570636950484\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
-3	0.0934535703126276	-0.227239520628721\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
-3	0.115390696823291	-0.313896027611391\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
-3	0.106023713566285	-0.287576679154121\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
-3	0.0966257183123387	-0.261170193191485\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
-3	0.0871965567953521	-0.234676136266612\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
-3	0.10926957279128	-0.32192394192328\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
-3	0.0998297489677462	-0.295441896485149\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
-3	0.090358462584103	-0.268871587435112\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
-3	0.0808555560825777	-0.242212572767877\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
-3	0.103066145376365	-0.330059797930529\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
-3	0.0935523620956501	-0.303413045049934\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
-3	0.0840066558587743	-0.276676880512702\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
-3	0.0744288657222368	-0.249850853538991\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
0.537886583448956	4	-0.0126620261638558\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
0.53599994549364	4	-0.00216809897884307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
0.534118153288	4	0.00829887499868598\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
0.532241188186827	4	0.0187389994778027\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
0.526775827752169	4	-0.014823752471844\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
0.5248999015857	4	-0.00430700177994603\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
0.523028802844864	4	0.00618268556970353\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
0.521162512919582	4	0.0166454139082803\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
0.515622503264112	4	-0.0169937610315976\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
0.513757384821553	4	-0.0064540888109369\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
0.511897075163215	4	0.00405840925911061\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
0.510041555715506	4	0.0145438381368011\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
0.504426364873643	4	-0.0191720995323307\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
0.502572150958734	4	-0.00860940713567449\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
0.500722726865196	4	0.00192599962292006\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
0.498878074057307	4	0.0124342263338147\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.924624474154102	-1.00623400625455	-0.550334296060567\\
4	1.0637884020032	-0.101769000151684\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.934633296762953	-1.01485340271593	-0.509594589177156\\
4	1.06213096187395	-0.0861229589818673\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.944642119371803	-1.0234727991773	-0.468854882293745\\
4	1.06047771430575	-0.0705164950986124\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.954650941980654	-1.03209219563868	-0.428115175410334\\
4	1.05882864341084	-0.0549494585231152\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.964866002109183	-0.993458605623475	-0.557517805570266\\
4	1.0748989533857	-0.103085499152609\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.974874824718034	-1.00207800208485	-0.516778098686856\\
4	1.0732359106856	-0.0875170587799596\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.984883647326885	-1.01069739854623	-0.476038391803445\\
4	1.07157705343489	-0.0719878001548322\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.994892469935735	-1.0193167950076	-0.435298684920034\\
4	1.06992236585288	-0.0564975755476025\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.00510753006426	-0.980683204992399	-0.564701315079966\\
4	1.08589736415929	-0.1043887105142\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.01511635267312	-0.989302601453774	-0.523961608196555\\
4	1.08422891594527	-0.0888971053405379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.02512517528197	-0.99792199791515	-0.483221901313144\\
4	1.08256464564711	-0.0734442922747162\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.03513399789082	-1.00654139437653	-0.442482194429734\\
4	1.08090453759173	-0.0580301257915418\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.04534905801935	-0.967907804361323	-0.571884824589666\\
4	1.09678532357923	-0.105678834397793\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0553578806282	-0.976527200822698	-0.531145117706255\\
4	1.09511166183643	-0.0902633100936512\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.06536670323705	-0.985146597284074	-0.490405410822844\\
4	1.09344217007312	-0.0748861940403021\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-1.0753755258459	-0.99376599374545	-0.449665703939433\\
4	1.09177683272422	-0.0595473428733455\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
-3	0.275016741636257	0.318464099554947\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
-3	0.281649014588661	0.340712214916542\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
-3	0.288238233874936	0.362815905744093\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
-3	0.294784817365672	0.384776573794313\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
-3	0.263426192772478	0.332561041575443\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
-3	0.27013404172854	0.354889186490687\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
-3	0.276798100230945	0.377071567897901\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
-3	0.283418795696495	0.399109608522073\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
-3	0.251702970525635	0.346819346876548\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
-3	0.258487694689603	0.369227902953099\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
-3	0.265227874704238	0.391489338816052\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
-3	0.271923947806723	0.413605098570382\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
-3	0.239844783776866	0.361241802019117\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
-3	0.246707712303528	0.383731148202568\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
-3	0.253525325589217	0.406071999448667\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
-3	0.260298070975166	0.428265821663957\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
2.3227256843839	3.1772743156161	0.22618755589019\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
2.32576102520213	3.17423897479787	0.23510310099458\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
2.32881066571741	3.17118933428259	0.244060647838386\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
2.33187470721861	3.16812529278139	0.253060493931981\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
2.31750185847795	3.18249814152205	0.230991883124655\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
2.32051266836299	3.17948733163701	0.239882530638814\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
2.32353760474344	3.17646239525656	0.248814892407969\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
2.32657676727378	3.17342323272622	0.257789262702725\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
2.31232011633952	3.18767988366048	0.235757506123176\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
2.31530669147439	3.18469330852561	0.244623366872182\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
2.31830722268891	3.18169277731109	0.253530657236472\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
2.32132180803603	3.17867819196397	0.262479668293158\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
2.31311900349251	3.18688099650749	0.258208407609945\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
2.31610930858271	3.18389069141729	0.267132175661891\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.476486073823362	-1	0.412244832823362\\
4	0.991159848539033	0.265789947524383\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.455072326823362	-1	0.449334530607787\\
4	0.987350755178758	0.280902581875283\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.433658579823362	-1	0.486424228392213\\
4	0.983519624341664	0.296102650242015\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.412244832823362	-1	0.523513926176638\\
4	0.979666264226472	0.311390913599003\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.513575771607787	-1	0.433658579823362\\
4	0.99770580743776	0.273805047871219\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.492162024607787	-1	0.470748277607787\\
4	0.993934436759458	0.288865559721062\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.470748277607787	-1	0.507837975392213\\
4	0.990141355626273	0.304012769641958\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.449334530607787	-1	0.544927673176638\\
4	0.986326376027868	0.319247428430406\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.550665469392213	-1	0.455072326823362\\
4	1.00418719150682	0.28174108054475\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.529251722392213	-1	0.492162024607787\\
4	1.00045298590247	0.296749759735325\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.507837975392213	-1	0.529251722392213\\
4	0.996697390426655	0.311844410013976\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.486424228392213	-1	0.566341420176638\\
4	0.992920220766769	0.32702577217777\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.587755167176638	-1	0.476486073823362\\
4	1.0106049515867	0.289599209787227\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.566341420176638	-1	0.513575771607787\\
4	1.00690736438431	0.304556345188937\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.544927673176638	-1	0.550665469392213\\
4	1.003188701613	0.3195987335193\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
-0.523513926176638	-1	0.587755167176638\\
4	0.99944878256747	0.334727105750607\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.56132816175884	-0.977858726342169	-0.563265272199926\\
-3	0.565174253005492	-0.219946772743362\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.562619568719564	-0.985182659160248	-0.521088424066642\\
-3	0.561583398965443	-0.197491275200431\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.563910975680288	-0.992506591978328	-0.478911575933358\\
-3	0.557993766058512	-0.175043414044675\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.565202382641011	-0.999830524796407	-0.436734727800074\\
-3	0.554405353661905	-0.152603185381425\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.519151313625556	-0.98529564262931	-0.563265272199926\\
-3	0.551447055534443	-0.222117578774727\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.52044272058628	-0.99261957544739	-0.521088424066642\\
-3	0.547838493367619	-0.199536291477689\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.521734127547004	-0.999943508265469	-0.478911575933358\\
-3	0.544231165208612	-0.176962726227206\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.523025534507727	-1.00726744108355	-0.436734727800074\\
-3	0.540625070424547	-0.154396879062932\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.476974465492273	-0.992732558916451	-0.563265272199926\\
-3	0.537565631927174	-0.224312773981479\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.478265872452996	-1.00005649173453	-0.521088424066642\\
-3	0.533939189238341	-0.201604279721379\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.47955727941372	-1.00738042455261	-0.478911575933358\\
-3	0.530313993635908	-0.178903594616633\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.480848686374444	-1.01470435737069	-0.436734727800074\\
-3	0.526690044476699	-0.156210714639732\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.434797617358989	-1.00016947520359	-0.563265272199926\\
-3	0.523527368386541	-0.226532771707029\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.436089024319712	-1.00749340802167	-0.521088424066642\\
-3	0.519882870311289	-0.203695629188974\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.437380431280436	-1.01481734083975	-0.478911575933358\\
-3	0.51623963260921	-0.180866384417376\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.43867183824116	-1.02214127365783	-0.436734727800074\\
-3	0.512597654626605	-0.158045033296036\\
};

 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0753755258459	-0.99376599374545	0.449665703939433\\
-3	0.668017536654152	0.308394121583095\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.06536670323705	-0.985146597284074	0.490405410822844\\
-3	0.670277019654357	0.328850481456709\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.0553578806282	-0.976527200822698	0.531145117706255\\
-3	0.672542095904788	0.349357480144355\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.04534905801935	-0.967907804361323	0.571884824589666\\
-3	0.674812786199945	0.36991530591027\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.03513399789082	-1.00654139437653	0.442482194429734\\
-3	0.6534326670454	0.305501297516042\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.02512517528197	-0.99792199791515	0.483221901313144\\
-3	0.655685316523917	0.326056244797117\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.01511635267312	-0.989302601453774	0.523961608196555\\
-3	0.65794357022552	0.346662329421666\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
1.00510753006426	-0.980683204992399	0.564701315079966\\
-3	0.660207449089842	0.367319742459371\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.994892469935735	-1.0193167950076	0.435298684920034\\
-3	0.638701543091929	0.302579464750271\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.984883647326885	-1.01069739854623	0.476038391803445\\
-3	0.640947107823332	0.323233953068746\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.974874824718034	-1.00207800208485	0.516778098686856\\
-3	0.643198287232844	0.343940084656196\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.964866002109183	-0.993458605623475	0.557517805570266\\
-3	0.645455102404742	0.364698053443761\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.954650941980654	-1.03209219563868	0.428115175410334\\
-3	0.623821953791154	0.299628184746278\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.944642119371803	-1.0234727991773	0.468854882293745\\
-3	0.62606017597274	0.320383181616372\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.934633296762953	-1.01485340271593	0.509594589177156\\
-3	0.62830402274524	0.341190335223985\\
};
 \addplot3 [color=IEEElightblue,line cap = round, line join = round, line width = 0.15pt, draw opacity =0.5]
 table[row sep=crcr] {%
0.924624474154102	-1.00623400625455	0.550334296060567\\
-3	0.630553515336993	0.36204984241913\\
};



==> figures/results/scenario-det-traj.tex <==
\addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999097315186919	0.240119845720588	-0.998329213122516\\
-0.938412095353681	0.295440126566335	-0.949231614583555\\
-0.878512791615236	0.340806297596779	-0.897664364211227\\
-0.816611331132436	0.388391284107827	-0.846652518350923\\
-0.756264247299061	0.430953857706298	-0.788542795559308\\
-0.693346798677602	0.477179850170322	-0.732806726098525\\
-0.633599009497513	0.525691123326287	-0.676768599237468\\
-0.577290825638977	0.574995702674751	-0.62150517088954\\
-0.522309512888715	0.624423455192063	-0.563569290256212\\
-0.465574742731491	0.673509682453996	-0.505666770494669\\
-0.408892490796794	0.719829021405084	-0.4466054956301\\
-0.352503658971736	0.766191572476398	-0.387410026197205\\
-0.297805366356346	0.812078150921203	-0.32558236930593\\
-0.243030960615153	0.85623754604451	-0.266362897759654\\
-0.193520760069313	0.904286350006819	-0.206959562961663\\
-0.141157391253395	0.953475887168867	-0.147201815584372\\
-0.0907455166952493	1.00139735951368	-0.0872885080405619\\
-0.0425576690079486	1.04778289551989	-0.0244577705657749\\
0.00282492915169044	1.09781824649243	0.0438777373380001\\
0.0565737955837675	1.15187541298268	0.106313216204646\\
0.10797019440556	1.20087217888338	0.172377656132818\\
0.161325119672917	1.25350548595618	0.237191095676087\\
0.21515978458401	1.31753096196156	0.300213086496812\\
0.271392805977068	1.37424111359057	0.362520098681723\\
0.33201801548201	1.43988655879183	0.427342396078996\\
0.391186315944183	1.50307631027328	0.495517768370902\\
0.445452114069583	1.56734539496914	0.566020288498512\\
0.506908482655378	1.63732088245499	0.634263296387283\\
0.549331935555102	1.6982240836136	0.699553937681523\\
0.604175723754949	1.76574419525826	0.765610972521112\\
0.659242072905705	1.82706975910274	0.835674754685076\\
0.713341541594064	1.89135293476561	0.902719944809226\\
0.770566008293583	1.94223570293987	0.964915878680431\\
0.827908195113713	1.99664706311779	1.02845572132607\\
0.890029784434075	2.04669553968328	1.09704364513822\\
0.955033659834317	2.09854691738488	1.16135988571675\\
1.01606760509757	2.14580206338748	1.21349562315363\\
1.07817559373134	2.21111847854855	1.27513029909803\\
1.1385821153485	2.26186625269289	1.32688609329567\\
1.20282493344029	2.32082152819043	1.39144809294066\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999667657862896	0.238173218303069	-0.997920668690405\\
-0.935784903697031	0.294398781427412	-0.949305133532812\\
-0.871210886795331	0.339217052961964	-0.902298536164682\\
-0.808200323443767	0.381929987661314	-0.849842262277774\\
-0.745813121953649	0.427107037955903	-0.798055905865515\\
-0.685129650788503	0.471942116021726	-0.745323886694096\\
-0.625304784298019	0.513570237308726	-0.693036976465682\\
-0.561810557637919	0.5554630076023	-0.643233500134224\\
-0.497163268612965	0.602609195051863	-0.589181958819995\\
-0.432870421577076	0.647717260435037	-0.541959806017581\\
-0.364732968296831	0.69175127298335	-0.492664363513962\\
-0.293457473207169	0.737765842164415	-0.443461715072101\\
-0.221934597662915	0.781366467477909	-0.396141012609215\\
-0.151103072946458	0.829666097750292	-0.352774052167906\\
-0.079247201751869	0.875330162963369	-0.306992134685458\\
-0.0065383115673814	0.920822809406805	-0.261741840358181\\
0.0644181911695005	0.969729747414371	-0.222088542729676\\
0.133873375463614	1.01213439957069	-0.174695113950791\\
0.211492204651671	1.05545602117726	-0.134289503229383\\
0.285919287914461	1.09413121789221	-0.0965963536127306\\
0.360094750580293	1.141824701382	-0.0564671814732959\\
0.437112530752416	1.18201692282175	-0.0158825087122953\\
0.511901831117608	1.22021870252017	0.0238666390745128\\
0.589930337717635	1.26811685005856	0.0683396505306249\\
0.668505584305252	1.31221622217147	0.102603112503561\\
0.739820170185275	1.35102097343292	0.137093133287093\\
0.817936143758984	1.39689732988944	0.171108615644905\\
0.89195169614011	1.43951244671421	0.204191235630114\\
0.968833705356383	1.47991378231493	0.227407522908481\\
1.04335471652829	1.53088700243087	0.254942466392028\\
1.11826650658343	1.57120971867254	0.276889956690151\\
1.19464354405239	1.61076484245047	0.300673516767108\\
1.272374741656	1.64905852456528	0.32068422032466\\
1.35515506597905	1.68737253394039	0.34225510062944\\
1.43732706164774	1.71610694613945	0.361396622647346\\
1.52164483412661	1.74963531223171	0.381795171980213\\
1.59752818231351	1.7863372178692	0.393402774599737\\
1.68048549684154	1.82243685751266	0.411131597581458\\
1.76939850653048	1.84988554472865	0.429142328458342\\
1.85293455268544	1.88858911443502	0.447308380711106\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999924837645672	0.241729177915146	-0.997478542776999\\
-0.937681164454054	0.292192750777386	-0.946703338527673\\
-0.878568289169036	0.343650225908645	-0.905308451817009\\
-0.818919711852958	0.394420933981825	-0.860678227362683\\
-0.754598519921171	0.440324111021316	-0.816337589535641\\
-0.689433670270014	0.489478495783867	-0.771326094999197\\
-0.626931673928238	0.534328670500652	-0.724755812370957\\
-0.566270433800586	0.583945836072204	-0.673426835276538\\
-0.5027953539105	0.633129182445539	-0.617329134314982\\
-0.443648624447506	0.681483771291245	-0.557108680896433\\
-0.381459744230073	0.724035331737841	-0.500230688911273\\
-0.321631027984259	0.76620000505117	-0.445800818212269\\
-0.259610519426787	0.816590856645716	-0.389021038288267\\
-0.196360582528207	0.863726388066227	-0.329800722523275\\
-0.138093303928964	0.911039500425341	-0.26642811127088\\
-0.0803888829457074	0.964797150196262	-0.208107030910868\\
-0.0211098465411437	1.01986537164632	-0.14941524298466\\
0.0424767654185755	1.0735123437897	-0.0850116423601921\\
0.102890399436442	1.12647594020454	-0.0267406652018197\\
0.1638152334735	1.17812365106589	0.0335642712888511\\
0.217369303309985	1.22710835879745	0.0923958316330016\\
0.273212289080171	1.2769121142545	0.151282815622763\\
0.326735137756616	1.32810755374869	0.208531645226444\\
0.37725296408845	1.37561128013418	0.266859890366238\\
0.429410292599422	1.42541532145426	0.328279951489699\\
0.481162847280057	1.47170369969262	0.389705496781714\\
0.52932906959137	1.52164030506356	0.449005272619135\\
0.574000185312082	1.56991382284694	0.505705798064868\\
0.619548005893587	1.60567741835183	0.55876119786146\\
0.662750942195111	1.64296270893025	0.615527738407152\\
0.707841582658699	1.68811455830587	0.672353114429739\\
0.750445765376639	1.73566971057371	0.730152122611179\\
0.796494069861394	1.78355092966546	0.786834106374463\\
0.839344706221885	1.83297375351583	0.850164601489153\\
0.87931395490178	1.89326684830717	0.90916643430478\\
0.915777648722567	1.94770717605551	0.959944434582392\\
0.949782110304803	1.99867803352606	1.02079645971072\\
0.983925357006963	2.05455423479001	1.08344051779624\\
1.01075553830751	2.10281458745752	1.13305205104931\\
1.04379994530776	2.15211816265308	1.1907194622744\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999478013440514	0.239121487946158	-0.999664169531621\\
-0.937919876202622	0.300262643840738	-0.949440908815235\\
-0.872945467509057	0.340046629608734	-0.896844670300923\\
-0.804632616432495	0.391936590717664	-0.839258657082587\\
-0.742691908422451	0.442684134614955	-0.781659198657779\\
-0.673202502243283	0.495630071255598	-0.719673845258915\\
-0.608168576948165	0.54780125920894	-0.651868795849366\\
-0.544810218600067	0.607407133032499	-0.579597294613321\\
-0.487314311397158	0.665107114801059	-0.509448534652274\\
-0.432317215081443	0.720341586380996	-0.439604476220697\\
-0.376675469530773	0.776095232950088	-0.369240626938829\\
-0.327117596602069	0.838461179420792	-0.302687526082584\\
-0.270657245407119	0.893645480317961	-0.2334230398002\\
-0.217031304029397	0.951272579562135	-0.16979722191176\\
-0.16313207559679	1.0019400607661	-0.101346322294367\\
-0.110643155564647	1.0579217936251	-0.032360869655571\\
-0.0571374588816951	1.11765721426541	0.0321714731982948\\
-0.00268375698680666	1.17624748971723	0.0957200692271709\\
0.0600950417554353	1.23908422052683	0.155574377739027\\
0.116628584544364	1.29854070254098	0.221616645435937\\
0.174352152453095	1.35911963201167	0.282043748453936\\
0.226881686004214	1.41883910376421	0.342040959781102\\
0.278859926509455	1.47489728216788	0.409194268661487\\
0.338077194537511	1.53169947861436	0.478150815151479\\
0.389425510186719	1.59133650957836	0.54159794166849\\
0.440920309230101	1.64134669664039	0.614851913131274\\
0.500769228324601	1.69736098010417	0.684263666035433\\
0.557427566640788	1.74929691731827	0.757367514396136\\
0.620095323988923	1.80111935439877	0.825193497402672\\
0.679861845802182	1.8504353721842	0.888987578365886\\
0.749867191447688	1.9049557385142	0.959037787026043\\
0.816187231743557	1.95461102350735	1.02605016818157\\
0.882605878828086	2.01233926787184	1.09987866918675\\
0.945865302569833	2.06557461300503	1.16485708437803\\
1.0054864236239	2.11745255540829	1.24129861209178\\
1.07355599734616	2.17706887679202	1.30473662224727\\
1.14074214222072	2.22275149504989	1.37680807708408\\
1.21409580086994	2.27917271594911	1.44486037917327\\
1.28265929370191	2.33709720180578	1.51601873073528\\
1.35064422845006	2.39357851378861	1.58384642030979\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998394363748421	0.241391636925528	-0.999676549414364\\
-0.936918381121223	0.298669992849192	-0.952094821158014\\
-0.875767908208196	0.343758352253392	-0.902905729901582\\
-0.815197212569857	0.392635576534526	-0.852626760192742\\
-0.753561249753385	0.440544606832965	-0.804526772703398\\
-0.688172570774846	0.490685192407003	-0.75064146760025\\
-0.624898115728265	0.546176192777976	-0.699077403445479\\
-0.561099281407153	0.602664714348731	-0.647079927584265\\
-0.49883757961662	0.65759771439262	-0.596232810753198\\
-0.435796183985938	0.710038888086768	-0.545440631051465\\
-0.373558648862864	0.769846214817057	-0.498040297105428\\
-0.314811782972639	0.828358498517937	-0.449357447921745\\
-0.2524024449055	0.896486465279975	-0.400265727976023\\
-0.192428253892741	0.962132014710789	-0.352285981124797\\
-0.13614184645904	1.0347170348175	-0.302497530760353\\
-0.0789206302516105	1.10277525703474	-0.248021472590597\\
-0.0251768291052274	1.17080059360707	-0.194291800797375\\
0.0293264326133252	1.2338702608214	-0.139257610005553\\
0.0861150100645423	1.30144023970158	-0.0886725710442827\\
0.143442980144328	1.36360002529055	-0.0369989662238396\\
0.201833597136823	1.43654387106327	0.0139565168372836\\
0.264952058314463	1.49954728847255	0.0605763557484886\\
0.327707811149283	1.56599261571286	0.110653745496687\\
0.394652125690023	1.63494296894629	0.160483867893581\\
0.452484459751574	1.70202312042417	0.210802665712741\\
0.5188420244303	1.76826251934115	0.265571934717872\\
0.583542550314195	1.83009966842947	0.317526540822369\\
0.652423235208146	1.89615201453503	0.371432798691608\\
0.722234329351696	1.95296742904529	0.427563973234104\\
0.797316877094472	2.00265708470708	0.483030450142666\\
0.872521777413502	2.06269868321607	0.544082891500222\\
0.942497800152492	2.10832357916145	0.597794893697672\\
1.02164341774071	2.16643438555882	0.659641741117754\\
1.09658968206325	2.22547782002623	0.722617067153515\\
1.16500599235602	2.28256003924498	0.778822768177995\\
1.23073515842758	2.33094914084345	0.832729757842996\\
1.30930344784289	2.38209429114025	0.887390751044605\\
1.38102199640084	2.43537171679772	0.947746989953797\\
1.45358138892782	2.49672284031577	1.01248982293028\\
1.52283257003745	2.54991729243403	1.0745339534392\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999206536821372	0.240614747710416	-0.999073765700739\\
-0.935747572771599	0.302554105470016	-0.949879809824215\\
-0.870085126440494	0.346651400973685	-0.898353459256663\\
-0.801329617155861	0.391252537491979	-0.844179580165398\\
-0.727861053855633	0.437286842337528	-0.793252966531727\\
-0.659903423554284	0.481716265764999	-0.742017905787137\\
-0.588749767361451	0.526441936775682	-0.687609600606862\\
-0.521788163477617	0.569496176155087	-0.635303353428615\\
-0.452161445437019	0.612263906426604	-0.583944864080208\\
-0.384968777677234	0.653505830051902	-0.53273794985631\\
-0.319373798657001	0.699595877740737	-0.480702393197372\\
-0.25002209192796	0.745477200657465	-0.426650616009033\\
-0.183112722215193	0.790983304225942	-0.367161808439276\\
-0.116039073883759	0.832499824607219	-0.305981387013783\\
-0.0491504999613637	0.872769645838886	-0.239981629032361\\
0.0134816638648992	0.917597551479742	-0.178202779981601\\
0.0776509297510142	0.956300051644895	-0.121771618324796\\
0.14816734953278	1.00064341847066	-0.0626745455673806\\
0.209082679261966	1.03734764337466	-0.00566020908517983\\
0.270636163818125	1.08074926264287	0.0485983283630865\\
0.335290536577594	1.11599847599121	0.111213780993127\\
0.398364715998242	1.15735503127916	0.170549149837201\\
0.462491158506485	1.19526592435404	0.228020511597368\\
0.526985046473297	1.23750385738186	0.281181029826116\\
0.595398138508177	1.28667294923754	0.340404343741137\\
0.654031403299382	1.33332692039148	0.400327171479644\\
0.715529531168409	1.38070372121129	0.464413802530454\\
0.774004358053077	1.42673058628537	0.532988378815541\\
0.832772151192636	1.46705069051013	0.599592577059147\\
0.888441175422733	1.51648837018956	0.662001696238218\\
0.946164642931846	1.56144889657937	0.72553379100922\\
1.00727868284173	1.61147515367677	0.792025434252592\\
1.0605874770109	1.66222244787825	0.852979107012315\\
1.11579267058985	1.71036936269883	0.913129270544734\\
1.17362794424683	1.7652853772959	0.985685724399741\\
1.23473228422935	1.81102251786995	1.05801304258326\\
1.29133062734567	1.86213339013939	1.12443621282147\\
1.35060711126922	1.92355931891312	1.19781805762717\\
1.4072385425516	1.9799713390525	1.26482317833978\\
1.4677627386464	2.03973471946858	1.33607070297014\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997883052500354	0.239562788719727	-0.999762184395189\\
-0.940996731810911	0.299202210121269	-0.948236377052586\\
-0.87911351281499	0.346255871198857	-0.898271486084\\
-0.823675025519549	0.389823822937065	-0.838610405547637\\
-0.769904405349007	0.434968934088193	-0.780165200632715\\
-0.712807781097405	0.474518048507076	-0.71472077338568\\
-0.65255664237385	0.520020696850162	-0.652418996932862\\
-0.595516806784177	0.558357933009645	-0.585080714163673\\
-0.538107912019687	0.602900647134081	-0.527400225730435\\
-0.483908647992432	0.644795766482449	-0.470550629464525\\
-0.43519436620072	0.690958385027276	-0.419232662240288\\
-0.382523690858809	0.735316388859158	-0.362577962272532\\
-0.329902162460523	0.776602583521377	-0.306884233448779\\
-0.278082033030916	0.828359581808442	-0.249840917333089\\
-0.225079816712181	0.876241512989808	-0.19531162091268\\
-0.170900832214055	0.925176847067152	-0.144054855766131\\
-0.116742834690869	0.973018330820666	-0.0893300328887857\\
-0.0624394644136377	1.02153583572487	-0.0448568270436764\\
-0.00577332859339685	1.07044479374776	-0.000920093897412682\\
0.0553641530800267	1.12488706094108	0.0436711281739225\\
0.114230016053197	1.17850102451915	0.0856520695225139\\
0.176789081501078	1.22591104014739	0.125805264868109\\
0.235512507891229	1.28004758400266	0.167331607676494\\
0.295535859530024	1.32939277352212	0.209155733249646\\
0.353722194315284	1.38011443215806	0.249022341216393\\
0.414532535755917	1.43675919406431	0.287667774705727\\
0.479258626095354	1.49600354249477	0.329848877583506\\
0.53173124446456	1.55555084735801	0.369697097335034\\
0.592932355954638	1.60842797308848	0.40975237770025\\
0.655115745090827	1.66474625526034	0.444502588779189\\
0.715754777221152	1.72403338974776	0.483427225629467\\
0.781599442546714	1.77381994572981	0.519613707393719\\
0.838067541498961	1.82717185638151	0.554225113916129\\
0.896449291980583	1.88818802403999	0.595879865356262\\
0.950550526056233	1.94171452484885	0.637873644316729\\
1.00895588826109	1.98508109395879	0.666801709341455\\
1.07027089243773	2.03911541539847	0.697469444289449\\
1.13282803001197	2.09728817885692	0.735774512405907\\
1.20244497662939	2.14622201057137	0.768879084125373\\
1.26927320717982	2.19726941539339	0.796044395505939\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00063716616188	0.241454311329808	-0.998645583687718\\
-0.937205208924317	0.301802541380557	-0.952111243642743\\
-0.876642622141368	0.34868600566378	-0.898622993834135\\
-0.819781338820658	0.395331527475424	-0.847474210687307\\
-0.758410314173534	0.444448998456875	-0.797983044158325\\
-0.693252783818156	0.497173217701488	-0.749053419622195\\
-0.629842025464283	0.550715637495785	-0.701412945984744\\
-0.566563601183096	0.60211363522896	-0.649075231225138\\
-0.506677778174417	0.657528260049903	-0.597745300773904\\
-0.438572139081411	0.717734841290323	-0.546013837285958\\
-0.372168895391132	0.777188744693852	-0.492202320471858\\
-0.315253685667198	0.838041290093364	-0.439557757902515\\
-0.251982770072643	0.897644255227291	-0.389011336626355\\
-0.192999006836236	0.960516347810662	-0.340087475761595\\
-0.136795947951068	1.02179893723344	-0.296563342468607\\
-0.0812706194522889	1.08396767647464	-0.248736117013248\\
-0.019614308991939	1.15097630173867	-0.20135460959152\\
0.0417152550813636	1.20744694247774	-0.154055536670709\\
0.10067181800372	1.26969969681178	-0.111070634989086\\
0.157637409496742	1.33124632079093	-0.0681202175718269\\
0.212813424725048	1.39292093026006	-0.020604002537148\\
0.272804998892333	1.45274837527847	0.0261000654517899\\
0.329804275226962	1.51344214336638	0.0676143578808853\\
0.387463218245537	1.57707583713732	0.118925726664259\\
0.446315174987434	1.63949739106265	0.165910214173213\\
0.5064195008976	1.7003305700312	0.215719432735994\\
0.560510198525291	1.75796494449459	0.260280536278802\\
0.623292017097367	1.825073278648	0.309005428639286\\
0.681940798166191	1.89490853929142	0.351218557850494\\
0.735341556594547	1.96304288399763	0.400036837865433\\
0.787907995854191	2.02429818414479	0.45033159091882\\
0.839314956909585	2.09842254323848	0.498438832575956\\
0.889821271244156	2.15752778842198	0.54592261509251\\
0.945814327792981	2.21859733023748	0.599545551758071\\
0.998989254242033	2.29081859034814	0.65084179676585\\
1.0555744088369	2.35574590616082	0.707343019389085\\
1.10345036676242	2.42200679028767	0.75968714801057\\
1.15266204462236	2.48423228126415	0.810776648317614\\
1.20538345445542	2.56802674263579	0.859657922911382\\
1.25750965581708	2.6253702260006	0.914616958698115\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999761700001014	0.239403006681903	-1.00064917212024\\
-0.937083741657319	0.294373445482623	-0.950469718385001\\
-0.866498553188442	0.339414873676002	-0.902809632387336\\
-0.795910058453806	0.382635376069131	-0.855747809311152\\
-0.722870800432642	0.425582219247966	-0.817688634859142\\
-0.650288491168251	0.468951313780107	-0.767575540394902\\
-0.57731033225852	0.514846285250778	-0.723355474033801\\
-0.509280094747592	0.562004399035181	-0.682855542108367\\
-0.443350252481358	0.615311835089838	-0.641896614799916\\
-0.36974734708259	0.668287915692574	-0.601156746642196\\
-0.297977393833331	0.722467178519768	-0.558465022701712\\
-0.222637099954328	0.771493790058387	-0.511730091595466\\
-0.14733763734938	0.822020443010629	-0.474378458458396\\
-0.0695166124726907	0.87151120941725	-0.431700718223935\\
0.00557842257860166	0.918921857558559	-0.388990247379048\\
0.0786352692641716	0.966885612175444	-0.346295891777934\\
0.151804010102404	1.01138556058554	-0.305464995906099\\
0.229184125424188	1.0587036306456	-0.264266006828897\\
0.303815765674651	1.10430062535515	-0.224765862907762\\
0.373161398829609	1.1514467749324	-0.185326287399925\\
0.449074088647261	1.19623366026015	-0.147777091255457\\
0.523856329732424	1.2401467952344	-0.109307611772504\\
0.597050856067149	1.28166219814115	-0.0733329690362184\\
0.666429531420284	1.34028457446826	-0.0357997775499501\\
0.734325524569692	1.39224101652019	0.00773283710159763\\
0.797214043380172	1.44181150257172	0.0432169956484051\\
0.860060750666171	1.48836632867528	0.0800071987863419\\
0.931424530450094	1.53670570482633	0.121163547677733\\
1.00062948743957	1.58978171720524	0.164634962687663\\
1.06316780852666	1.63763103683876	0.210132750385208\\
1.14239457049625	1.68275328595518	0.253975943840862\\
1.21261184245252	1.7298573092557	0.289613858523382\\
1.2852054776753	1.77838257977673	0.328176939380943\\
1.35716420480542	1.82792492289509	0.367898821959726\\
1.43219241032717	1.8799483647952	0.408911875974675\\
1.50751959665862	1.91701301547635	0.451607809764857\\
1.57498585601223	1.95862414773015	0.49433054244464\\
1.65492450528847	2.00299315142748	0.535073312125774\\
1.72552426370735	2.0446060887609	0.588618345274859\\
1.80027746548308	2.09282137366448	0.638922438455971\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996557484340456	0.238127046917851	-1.00033070407717\\
-0.93513036312295	0.294731733763121	-0.949236022945345\\
-0.872248630463624	0.33502965491585	-0.902049049719279\\
-0.811783366682228	0.373738005004437	-0.850490665650075\\
-0.743483424008749	0.420488362023471	-0.802506016003737\\
-0.678178150151024	0.464440157062153	-0.754900619054351\\
-0.613837722533753	0.505346708182796	-0.703550884169227\\
-0.550773095256114	0.544149676926005	-0.654597133463295\\
-0.484783111725279	0.576553565383625	-0.601380901785099\\
-0.419891026595235	0.602767477244866	-0.549539256249417\\
-0.355936053713014	0.628793672874905	-0.491666868401052\\
-0.287871815613709	0.657796338689459	-0.433591164827056\\
-0.223142450241228	0.687876582257511	-0.37692982574188\\
-0.1576564849622	0.716018257216614	-0.320710851529268\\
-0.0902147955503067	0.747648995606423	-0.260003452656784\\
-0.020992257203037	0.782254675672127	-0.202098856176548\\
0.0447952876140054	0.816035904893276	-0.139867454421879\\
0.107240191087314	0.845079539501693	-0.0830441012464023\\
0.166325622747975	0.878813853349971	-0.0204600605168311\\
0.227368626549095	0.913951924739406	0.0382483035671166\\
0.292686560664903	0.948482884708528	0.0986522426200731\\
0.355256906569886	0.978937354953976	0.159478173175479\\
0.417232181140286	1.00983197106356	0.224787873848702\\
0.481064852892179	1.04740121192606	0.291947225524282\\
0.543566132632117	1.08224217749785	0.357307703517591\\
0.608078679972692	1.11415210912127	0.429078478255093\\
0.672066702127995	1.14766939923219	0.49671352484031\\
0.732981496090601	1.18166390481801	0.568159265928992\\
0.783627929520301	1.21376666421331	0.640942806117818\\
0.8344997953883	1.24690171289741	0.716566771170719\\
0.885039902463244	1.28073374473318	0.786940207782146\\
0.930708452832229	1.3115687574571	0.860905840384476\\
0.98360931213329	1.34306895639374	0.939576414751668\\
1.03603582288931	1.37468961101943	1.01230001250279\\
1.08966971776071	1.40527663662884	1.08296245920174\\
1.13626295165955	1.42561490088607	1.15306202232274\\
1.19215253749428	1.45547645371559	1.22816334027747\\
1.24157209939946	1.47269876202887	1.30333572842356\\
1.30164444783406	1.49081693517748	1.38450619067058\\
1.35424781864775	1.51250693156614	1.46719124853321\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998143503907388	0.237834720674987	-0.997862096085271\\
-0.936119373375667	0.29635870836499	-0.948464643518147\\
-0.877015955066647	0.33924871954674	-0.903160394177027\\
-0.812590672948743	0.384192528212344	-0.858675410842631\\
-0.749281978678445	0.43131747400185	-0.814889078940378\\
-0.683932352360197	0.479000083663537	-0.772748103589553\\
-0.623711676075119	0.531963156861454	-0.73212274666469\\
-0.564845833995446	0.581550208705826	-0.694764928561899\\
-0.5055480002133	0.628453895740117	-0.65908097128571\\
-0.444316879162597	0.674607389249144	-0.623936411013735\\
-0.380007057096599	0.724880882819921	-0.58393302298713\\
-0.309997303481852	0.7756871852443	-0.543238813205964\\
-0.239000843607946	0.830241204981572	-0.500675070154326\\
-0.172836106117607	0.882627757546596	-0.460227256581453\\
-0.106308300553263	0.938201516825577	-0.41703412596941\\
-0.0471534947563634	0.989288780128619	-0.371691141212866\\
0.0117366833573346	1.04837825859809	-0.331429212711511\\
0.0727443352361	1.09819029551659	-0.293151152697399\\
0.135386836081989	1.15896980561673	-0.254126685777976\\
0.198628929069509	1.20673347677698	-0.213717569504495\\
0.258673408497719	1.25994052522973	-0.173099333122474\\
0.320150846837991	1.31866106270209	-0.134773249158211\\
0.378929026791078	1.38521212080011	-0.0983565558729863\\
0.437873959975012	1.44270196064706	-0.0614942750998124\\
0.492321536975069	1.50285652136453	-0.025457833716979\\
0.546318410874817	1.55391028322688	0.0166150332734676\\
0.605540743583913	1.60912346203265	0.0588836632214943\\
0.666835145503873	1.66369002246334	0.101656455169822\\
0.72514641941733	1.71731321995269	0.150913802880084\\
0.782775627550259	1.76859293944252	0.196711908174917\\
0.845024159096932	1.83350206120734	0.240048580285645\\
0.905431261187945	1.89610129815776	0.285097770227969\\
0.967434816477778	1.96053005994677	0.329864810774429\\
1.0263995539753	2.02495426435714	0.372367418412664\\
1.08691134623291	2.08659693821654	0.423219304952599\\
1.14247857492891	2.15222889688014	0.470000266194938\\
1.20268458384461	2.22302768969197	0.520221362073296\\
1.2639002057665	2.29081616581861	0.567124247456189\\
1.31723846452443	2.3636705289299	0.616132282466592\\
1.37474288671603	2.42693167401703	0.661817703761842\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00142900461296	0.240147957678304	-0.998406460851612\\
-0.938197324332236	0.295334718464668	-0.952216015599749\\
-0.876839873964868	0.350178567484294	-0.901017568029402\\
-0.817496685826353	0.39618640386396	-0.849058939655302\\
-0.754302742769883	0.44098662705796	-0.794953670378155\\
-0.69192095378022	0.486774376254353	-0.748227583885473\\
-0.631354894185067	0.540080255498246	-0.701509102663529\\
-0.567160208013936	0.589033886692762	-0.65416397239147\\
-0.498960196856029	0.639448901286538	-0.606626205052239\\
-0.433302647164134	0.690927832605153	-0.559422133930822\\
-0.367502040962729	0.740061535168137	-0.510308694318523\\
-0.304932952225055	0.795547537011483	-0.462312130639576\\
-0.246133728336513	0.844070893732651	-0.416333206049848\\
-0.183151079213261	0.89667013869535	-0.372597622473266\\
-0.123073122467333	0.949187994951381	-0.323872478356829\\
-0.0599848181730635	1.00269707003528	-0.283246784079472\\
-0.000309752347445189	1.0556467315861	-0.235367346343113\\
0.063173487596274	1.10473570297316	-0.189521452313285\\
0.123886762248131	1.15126495604683	-0.149011666221997\\
0.186443847513615	1.19844426176845	-0.107739925708104\\
0.24693645963093	1.24410024797039	-0.0705626168191486\\
0.308258490539158	1.28967133235073	-0.0290909828346624\\
0.367846196243475	1.32535456310175	0.00330638897666914\\
0.427108524834924	1.36331730750391	0.0424891208927427\\
0.487278962720125	1.40173273654597	0.078392918436746\\
0.545400045400908	1.43415701456405	0.118292343076596\\
0.609133393740637	1.46883226202543	0.155340761660565\\
0.665965407605042	1.50147064154481	0.192594451722163\\
0.726813411340104	1.53465599570732	0.231493014982381\\
0.78525879049664	1.56803461360385	0.269073261142687\\
0.838786959347744	1.58847390345152	0.303170465642419\\
0.892005642473626	1.61372688249988	0.343783246671645\\
0.950855960118939	1.64824200717464	0.372693398799394\\
1.0072378680843	1.6714115179774	0.404857575435964\\
1.06370903706535	1.69829559562477	0.440066723251571\\
1.12481121783017	1.73151505961917	0.474039891532218\\
1.18624750005605	1.76011557948633	0.50961939888103\\
1.24513870865576	1.79057214961095	0.545563326536426\\
1.30048742944756	1.81247736836193	0.580687749516901\\
1.35829865956036	1.84178797899312	0.611136084006384\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.000431929394	0.242108810241391	-0.996613678930367\\
-0.935395247542184	0.296696837414976	-0.949268898252742\\
-0.873466293320584	0.336764606567942	-0.904652114447874\\
-0.810857531351084	0.385165017454719	-0.862627261291802\\
-0.745019123144069	0.428570708651443	-0.823328312950029\\
-0.679732999223635	0.477891179298135	-0.778109137581995\\
-0.614085299734276	0.525537029290357	-0.73407857204494\\
-0.553436679857362	0.568002879711038	-0.688347702132144\\
-0.48873106549623	0.614967439871658	-0.643905357028129\\
-0.4257494399878	0.661433413824767	-0.600762487765264\\
-0.363236170211182	0.707915303996083	-0.558763809627151\\
-0.303957803765229	0.753165135814846	-0.520776306799409\\
-0.24553924893707	0.79938725917993	-0.481019442302414\\
-0.188214276627694	0.849078387009438	-0.440856542605533\\
-0.128743658521414	0.894051825053391	-0.404589860691225\\
-0.0744397850636842	0.944413409009806	-0.37611361594768\\
-0.0203425627323284	0.989312849002061	-0.342400349984501\\
0.0359658143602226	1.04358101270269	-0.312861974034751\\
0.0925091039836771	1.09763602470283	-0.286264633099817\\
0.144807044968857	1.15212865150002	-0.25918860109279\\
0.195680860483034	1.21246766894415	-0.233152024596562\\
0.240935939112717	1.27762167330057	-0.204539391843426\\
0.291908249317216	1.34282715546215	-0.175139414471213\\
0.340000559067686	1.4063321122499	-0.147170027959631\\
0.39158194427972	1.46969012595874	-0.118719167386497\\
0.442579932439202	1.5367482694804	-0.0870962927934579\\
0.488893576129766	1.6060146048989	-0.0532176495575057\\
0.532908376754002	1.67309253795844	-0.0226400508827586\\
0.577611649866443	1.75170206681924	0.0101117423579534\\
0.622171702248338	1.82756434998143	0.0446559497183861\\
0.666018123806787	1.8964131217669	0.0834059606004055\\
0.715364591791782	1.97093698788423	0.11904090063922\\
0.759105280982104	2.04473207028721	0.15684534030507\\
0.801045366455763	2.11641537296264	0.198211436191412\\
0.852682136375208	2.19166312589285	0.242416508774737\\
0.897160014769339	2.26941307026482	0.277077230807292\\
0.949585212081186	2.35692661164114	0.316272231060444\\
0.991432937900816	2.43551139464911	0.355832102985598\\
1.04250084342095	2.51861318429785	0.400757017845699\\
1.08025195696505	2.60354495538013	0.44687055238035\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999675674549572	0.240809603814368	-0.996921683921689\\
-0.936509765495007	0.295010362876939	-0.946156867203659\\
-0.877103012466081	0.340598187773546	-0.897014585165409\\
-0.818272275394896	0.387880425247887	-0.845897554927339\\
-0.7612194144048	0.435420541447693	-0.794485899749282\\
-0.704979922365958	0.479729633550489	-0.741286744571794\\
-0.639208909238037	0.52062089366172	-0.692090257591796\\
-0.577984003417673	0.563109006909322	-0.642529064414549\\
-0.517015284371299	0.609516847928064	-0.592728708926859\\
-0.453773579922665	0.653794869828183	-0.541515223852534\\
-0.390079089332476	0.697274369166527	-0.485863733536751\\
-0.327504657776601	0.739934896551448	-0.429486405389553\\
-0.262046441398609	0.782759138766421	-0.37033900678668\\
-0.200656581709071	0.823695585443169	-0.314480824297384\\
-0.135284097210144	0.856714784846357	-0.255904593947051\\
-0.0762283681468417	0.903093108106359	-0.202002253319113\\
-0.0157703330350061	0.945477958711656	-0.149355461581598\\
0.0496086043769402	0.983430956724827	-0.0939053984881232\\
0.118090518779486	1.02445102772296	-0.0402722598189369\\
0.193554947819586	1.06240224522367	0.0130537006441972\\
0.267871710043001	1.09142390631313	0.0672498013698857\\
0.340769264519242	1.13167393744778	0.126832226891232\\
0.415027483905811	1.1684706298973	0.185288116350222\\
0.493316719837835	1.20831694210164	0.246903465407932\\
0.569107983300983	1.24994792427442	0.306778315649002\\
0.643339190981587	1.28563769326021	0.362948265532255\\
0.717433211087527	1.32212580465582	0.420520769832319\\
0.789162984553019	1.36187154184974	0.47776243035757\\
0.857169685997231	1.4034313712596	0.529632835913584\\
0.924296060951781	1.43705292018788	0.591922695395719\\
0.99248551362416	1.46425018627655	0.653714754855534\\
1.06219677563893	1.49906144777219	0.716928985872617\\
1.12793576496037	1.532796602114	0.784138692702429\\
1.19188657303142	1.57148097241137	0.851479263160206\\
1.25398166792128	1.61627880764542	0.925146542849287\\
1.31955955764024	1.6621984086671	0.994470907699137\\
1.38426700887822	1.70276569314377	1.07090787017195\\
1.44694614785174	1.73113117810826	1.13828249090098\\
1.51331152355335	1.77379614841949	1.20205150378024\\
1.58202688317567	1.80498441091493	1.26572979578591\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998523188471092	0.24048552892452	-1.00170842600049\\
-0.935694876595461	0.294255158763531	-0.953312919699704\\
-0.873418569530788	0.338750563478147	-0.903297305057812\\
-0.805937368358524	0.384714228935152	-0.856472366409174\\
-0.73644881916597	0.432362602700558	-0.809117172270303\\
-0.666096514273311	0.47435451738839	-0.762009897867566\\
-0.591687476407541	0.515490821271538	-0.714647926220729\\
-0.520202312442606	0.554686755200702	-0.668895876428494\\
-0.445075328958954	0.597204489312534	-0.620528376394389\\
-0.373611501295216	0.636541202900459	-0.573202326591494\\
-0.295549321703794	0.675197984979172	-0.531126962977454\\
-0.219949517412132	0.716566562050213	-0.489533313473778\\
-0.147744684498745	0.762571193658453	-0.449373578371776\\
-0.0747871774099083	0.805580254413355	-0.405371776163637\\
-0.000202109465291554	0.846650434434639	-0.363725599102718\\
0.0753779075001549	0.888742353086232	-0.324305521727015\\
0.148253855657127	0.930235521506898	-0.283263750983281\\
0.223504508926574	0.977710040914858	-0.241468903491411\\
0.298977616156341	1.02924642998083	-0.201342160570331\\
0.371607400002179	1.08011982849191	-0.158799968742345\\
0.44370301713544	1.12859088483185	-0.119848679034722\\
0.515670821589246	1.17716622598193	-0.0756963960955148\\
0.584310341113133	1.22100853665103	-0.0380155945506723\\
0.659067341253921	1.26929434150498	-0.00232670106254471\\
0.732343555720719	1.32066213858617	0.0353356334245465\\
0.80901870036679	1.36620824688496	0.0765995747885008\\
0.884830417415499	1.42409074044718	0.117268979460787\\
0.953978596030018	1.47702275851655	0.157121450691774\\
1.02794018824188	1.5266594734392	0.194957906169915\\
1.0977445584735	1.5784186864705	0.235820516626036\\
1.16676120248622	1.62998773548756	0.282958365704768\\
1.23308664372872	1.68333826260255	0.329986096163865\\
1.30143636944258	1.7270812039364	0.375240226634142\\
1.36936122985612	1.7726067393875	0.423324001247358\\
1.42882773716402	1.8141801079722	0.465804077238354\\
1.49270864182533	1.86094409073697	0.517680618134507\\
1.55421912696374	1.90875222482126	0.564929672971485\\
1.61189952531815	1.95651327017592	0.617552476208053\\
1.68018299996685	2.01627387974435	0.671481385110162\\
1.74317521048629	2.07317420510261	0.725931570315693\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996266401555801	0.241065408109953	-0.997524270030674\\
-0.935616037530966	0.298961037372814	-0.951290848895173\\
-0.874271186655702	0.341871700352364	-0.899247061247083\\
-0.809770474953617	0.390197258806424	-0.845434199766446\\
-0.744783683903365	0.440345301405434	-0.792957324392102\\
-0.67832651014073	0.489964877939231	-0.74178982719984\\
-0.614311038930228	0.537634431299462	-0.686781912050792\\
-0.550704392560502	0.587461630952286	-0.628914223909\\
-0.485076361067475	0.645340318151365	-0.570181501562755\\
-0.422779396086289	0.693670264799247	-0.513776130221047\\
-0.358407445522421	0.745514559139438	-0.45387248940336\\
-0.294554756489185	0.800494452650882	-0.395580236585909\\
-0.228370504371983	0.857626438502614	-0.340759525021052\\
-0.164919570666964	0.918189069285596	-0.284081000782394\\
-0.100428300424231	0.975671411156861	-0.233126161714587\\
-0.0364873631808184	1.03354529816135	-0.174485607486058\\
0.03039503565278	1.09414494202886	-0.120043416591615\\
0.0966370966310939	1.15705947319445	-0.0604133705478779\\
0.164139675264674	1.21258994170563	-0.00387211094833333\\
0.234579919298428	1.27117994893513	0.0555895249896556\\
0.305604083576958	1.33347476322621	0.115301323866013\\
0.379635059950721	1.3991913971082	0.179514850063613\\
0.445239738524514	1.45915603264508	0.244340787753376\\
0.511424747596353	1.53032589957715	0.308376282465888\\
0.587592606715259	1.59903285665379	0.373734646131174\\
0.662927073760067	1.66167057488262	0.442080929446937\\
0.733463540853294	1.72478466110331	0.505233329322579\\
0.808293643815278	1.79699096215508	0.569880227308837\\
0.8822383050201	1.85960945772145	0.63979966364737\\
0.956602348522238	1.92284929365042	0.707140390382085\\
1.03346178189316	1.98734342347434	0.773131982992607\\
1.09750265277435	2.03994716096301	0.839721978493359\\
1.17178781605971	2.09700204093048	0.91469809006404\\
1.24578754766594	2.1606719798423	0.990379204647398\\
1.32598663784628	2.22737527943389	1.06791622348461\\
1.39326662282973	2.27572595369693	1.14591160953309\\
1.46317253085109	2.3362594425709	1.22851334309658\\
1.53616151781272	2.39669887221766	1.30699230440716\\
1.60590422014942	2.44918304097556	1.38804621914146\\
1.67886003856337	2.51380092142403	1.46795566141155\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996553195622749	0.241428731307668	-0.998680181989563\\
-0.936946398371795	0.296336888334277	-0.952899488956145\\
-0.868689540023367	0.344896077759647	-0.908049532780763\\
-0.797570013485324	0.392245353521358	-0.858788927314199\\
-0.727135133834651	0.439187572096872	-0.810245505490446\\
-0.656863674494348	0.491748415547409	-0.762986536853851\\
-0.589304108632216	0.535215398766491	-0.710713696252079\\
-0.521841596907772	0.583515855202647	-0.663010546813638\\
-0.459070593961333	0.632181652937738	-0.617375011773583\\
-0.396084333707836	0.68122609357534	-0.566609871526138\\
-0.331537023497307	0.728529095980444	-0.516462479103587\\
-0.270461608280935	0.776666307276697	-0.468661122470562\\
-0.208959096208436	0.82253710485579	-0.418560260672453\\
-0.148109906408346	0.867854260607204	-0.368559657787423\\
-0.0852661901429587	0.911916664075609	-0.322616294682748\\
-0.0281724629784662	0.956549830375345	-0.273431922590461\\
0.0316297453834707	1.00411955573829	-0.226040408533207\\
0.0940424900614943	1.04969457192387	-0.177012415465904\\
0.153463820027174	1.09871927638879	-0.12832482154147\\
0.208426073295889	1.14300127994308	-0.0758349198329008\\
0.263029737410235	1.18294801174318	-0.027244607005956\\
0.309987666860116	1.22848019726555	0.0183252554270275\\
0.355168539900888	1.27011340902465	0.0641514958055227\\
0.400838745159028	1.31232369003444	0.104748933688482\\
0.446210174248702	1.3561230716174	0.14553077380875\\
0.490297226838374	1.39353204803897	0.184628834162501\\
0.53132077982562	1.43449859590389	0.225259351355798\\
0.579360011591246	1.47423522063302	0.265770644211078\\
0.620114687428883	1.5137881427356	0.310008645574089\\
0.662268500042963	1.56344772551497	0.35352676324262\\
0.704181777392747	1.61483448149668	0.393366649469507\\
0.74416992319634	1.67017122458545	0.4359345662294\\
0.786861093748554	1.72853097027624	0.480056910850364\\
0.825863620126442	1.77262520011	0.519936418871072\\
0.867748587436645	1.81846500584132	0.559978643448845\\
0.904348079717769	1.87077411002873	0.601503898989438\\
0.939957131715918	1.91938102343195	0.647163560902774\\
0.984100613984313	1.968429123356	0.687504026488806\\
1.01875351501244	2.01604337703786	0.72948485477501\\
1.04955551295515	2.071497787221	0.76585638322754\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998879902201073	0.240496085513992	-0.99988366606658\\
-0.939370794986175	0.299688628768168	-0.950860526824933\\
-0.873789045122942	0.345583716334724	-0.904156203431173\\
-0.804188423871314	0.397335530731634	-0.85364545886601\\
-0.738232606420457	0.45007556760859	-0.806257935093803\\
-0.673380637037804	0.504234232855233	-0.75674450493024\\
-0.609847130544732	0.562259906775999	-0.704740058997178\\
-0.544257641839152	0.613043902150979	-0.657951432356445\\
-0.474965162789158	0.664304469295863	-0.611695161932119\\
-0.407099820977274	0.724749841543837	-0.558969937446712\\
-0.33348289548803	0.783060905035537	-0.506787300641006\\
-0.26540003473959	0.841948910151505	-0.457250201837349\\
-0.195976614764264	0.897326878189592	-0.409250105902261\\
-0.123554371748513	0.955647713582156	-0.356437774225914\\
-0.0552666572992857	1.00993096643663	-0.308400481284111\\
0.0144717608967379	1.06703826389719	-0.25437161816529\\
0.0911764688052082	1.11871904774566	-0.206025367099183\\
0.163761483087618	1.16945201153436	-0.153264874298582\\
0.237617842680693	1.21996092266649	-0.103993833305754\\
0.31463664029243	1.2789093299813	-0.0549133951063001\\
0.393438353942507	1.33219400122285	-0.00456118324455546\\
0.470623632413837	1.38843610152572	0.0422677329824553\\
0.5526201097657	1.44449013484385	0.0885204495478698\\
0.634651552228326	1.50616302618079	0.136904016950607\\
0.72025096587917	1.5724370314638	0.189311364249635\\
0.794706215447156	1.63153022791049	0.240944076360831\\
0.880896683430186	1.70352199722535	0.295045005811415\\
0.966734560096649	1.76698222317146	0.338746543162434\\
1.05158054734628	1.83490239619738	0.383807170676711\\
1.14501742093597	1.90974711679438	0.428760396921591\\
1.23643583967319	1.97863582803307	0.464731570803217\\
1.32462125867028	2.04379879798905	0.504847827125861\\
1.41534672207407	2.10608913194866	0.539949721838696\\
1.51144870099735	2.16982541766346	0.577831754697006\\
1.59059562940606	2.2382519077932	0.614215323291034\\
1.67620167064393	2.30195908047853	0.648005908040606\\
1.76144098834775	2.36756621870626	0.684560028601531\\
1.85342007642594	2.43203666681135	0.712997443832887\\
1.93248096066779	2.50270747971638	0.742465233245272\\
2.01662392343828	2.55281677520205	0.766402992723045\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998186840084946	0.241238126532768	-0.99575913010429\\
-0.93910655074124	0.295197335550279	-0.94816137861081\\
-0.879566605680491	0.34774384672798	-0.904031152519019\\
-0.815485814067297	0.39518190071445	-0.855337447663044\\
-0.751283235483321	0.447638161782792	-0.807095082872336\\
-0.68777329853078	0.498580686058877	-0.759130780209098\\
-0.623532697387901	0.54981545761173	-0.712553875593714\\
-0.560444288094363	0.596732133763351	-0.669823215352021\\
-0.500923289589524	0.649962270044387	-0.630354768568722\\
-0.439217692788261	0.70269553082119	-0.597529292235517\\
-0.382377505947668	0.753636233053346	-0.565417465490072\\
-0.326986875308349	0.808659484033586	-0.533639240895368\\
-0.276188885195786	0.863493979132822	-0.50445883928031\\
-0.220440558413139	0.922386013886069	-0.476520822699489\\
-0.167307434473189	0.984501715839633	-0.450362731923827\\
-0.115980537432391	1.04575834750217	-0.42361032661191\\
-0.0605358746356502	1.10209660914717	-0.398929354089092\\
-0.0124327974852918	1.16072501346216	-0.371653134877353\\
0.034373815565122	1.22345447538754	-0.342406795347864\\
0.083441933861303	1.28633735897505	-0.315279287820554\\
0.129345241622559	1.3499962899717	-0.286714139511742\\
0.173700219918909	1.40807926239857	-0.261012966568939\\
0.216862447993608	1.46865706647241	-0.23840836540336\\
0.263608652318412	1.53897001686056	-0.205886321889335\\
0.30119146157233	1.60681819495591	-0.181663804550202\\
0.339887347097249	1.6722033398497	-0.155163638663346\\
0.377296124081438	1.73704096989589	-0.129173329717089\\
0.419244588911832	1.80532865269098	-0.103187554488832\\
0.461599638526467	1.874338641162	-0.080219185013098\\
0.500299350194451	1.95379052822162	-0.0602792524145983\\
0.542228900556564	2.02021763986239	-0.0325275099175743\\
0.579641688465665	2.08746259300911	-0.00937972038193605\\
0.623227073988167	2.15365560616595	0.0195321961606601\\
0.665600501944054	2.2253126287606	0.0434950617180265\\
0.712914359812287	2.29086498906892	0.0728816646467084\\
0.762924661189738	2.3626291983752	0.101602939638156\\
0.809700720262381	2.42841258189739	0.128586396792931\\
0.858518206548166	2.49392383211801	0.155222973011852\\
0.908667903130117	2.56441707039368	0.174748914416757\\
0.953441004133035	2.62692835231056	0.193056381098966\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998501463206577	0.240622048850611	-0.997956032982096\\
-0.937380092684389	0.299739589435348	-0.948773765656467\\
-0.87288428821746	0.347166221913456	-0.894320302504629\\
-0.807684610880128	0.396017859973276	-0.835151346077745\\
-0.744529176595335	0.444283635809204	-0.776977159531321\\
-0.684774500862059	0.497270244904476	-0.722827206419273\\
-0.623058659794482	0.552846761725483	-0.674611875493064\\
-0.557856907490218	0.603684184662123	-0.624846806898406\\
-0.496017379702059	0.652288335401447	-0.573934216827273\\
-0.43300214697173	0.697762032164445	-0.529414021468079\\
-0.371599276837317	0.741167709577692	-0.484825068934523\\
-0.309379588785731	0.78443817232376	-0.435807416039495\\
-0.248278621653015	0.823641573001581	-0.391412712832659\\
-0.190766229789827	0.863015670568478	-0.352671634355826\\
-0.132950857574769	0.900897601534577	-0.315171867906392\\
-0.0785247158253818	0.939622352569191	-0.273730439469658\\
-0.0208412267141289	0.977094025030942	-0.236186927751407\\
0.0332996331060053	1.01712525855086	-0.19707575583392\\
0.0849339521357008	1.06091755685768	-0.162941831995224\\
0.143076282026755	1.11128190240168	-0.129669269501444\\
0.20129723334914	1.153573022764	-0.0894201939493836\\
0.259652317216535	1.19729800428796	-0.0599667397297685\\
0.315237186577836	1.24883014064212	-0.024474621888829\\
0.365262307022047	1.29946267625776	0.0084960433227074\\
0.411739106210097	1.35514135094607	0.0410666842690655\\
0.456330172505233	1.39810397050393	0.0749012268964479\\
0.502916568478967	1.4489316490109	0.108553878157218\\
0.550320654886159	1.49342870763487	0.143259081876911\\
0.597633145833903	1.54265003791567	0.186611771047641\\
0.651254439085877	1.58989861541072	0.225795991854095\\
0.706089601716066	1.63824149921117	0.265464746672398\\
0.755232603225867	1.68050412134056	0.302410296115793\\
0.801892633952299	1.72176174228032	0.338168917135952\\
0.851107023511234	1.7598184382646	0.379277603095691\\
0.910045444506951	1.79817423689589	0.419285501841558\\
0.961868295151989	1.84519947095436	0.456521047292635\\
1.01436343173049	1.88725122739054	0.489987371502914\\
1.06542357727094	1.93391401759271	0.52582168386404\\
1.11707626417437	1.98249589454058	0.560983146840853\\
1.16637519937206	2.02691607247731	0.594805476282318\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99941386444476	0.23981958381857	-0.99940192455211\\
-0.935790783494671	0.295973440151058	-0.946644440945783\\
-0.870953484147256	0.337920676615916	-0.895624035090351\\
-0.806049533947736	0.38222421949771	-0.84251474270725\\
-0.740628400801643	0.422809568428598	-0.785407613821271\\
-0.680530627252956	0.462177667265037	-0.732220734954956\\
-0.61755393063427	0.500809723334486	-0.677468006362588\\
-0.553039189053207	0.537744681941029	-0.619959926684529\\
-0.489261787921256	0.578833756878931	-0.563527496873362\\
-0.423585694721391	0.628139430911374	-0.507387672388164\\
-0.358626023549135	0.671992438111445	-0.451438345867636\\
-0.296604452183055	0.718979492251215	-0.394927180571802\\
-0.233893918287818	0.762479305620649	-0.344553852355452\\
-0.167105297522116	0.806033925762861	-0.294907121623299\\
-0.100313319827201	0.85173982157492	-0.243923305374739\\
-0.0347131128428459	0.899667072910527	-0.188163931381889\\
0.0318992766133705	0.951575077588766	-0.1292858123271\\
0.0939587124992772	1.0023203271045	-0.0722763537621054\\
0.155471461729173	1.05367549544397	-0.0178115528891776\\
0.217321132960819	1.11225191889027	0.0369684793519381\\
0.27554528441688	1.16293097072858	0.0897093697707379\\
0.326660311383942	1.21901725621047	0.140407098341125\\
0.385442278344885	1.27733913367489	0.19077295311036\\
0.442732556338243	1.33109214322283	0.242704778539406\\
0.496396603946829	1.38733670957261	0.29438914405709\\
0.555329633902037	1.44313816929292	0.346349961766558\\
0.620033187587347	1.49933564394949	0.390839968070357\\
0.681681133192265	1.55385734626562	0.444059387189137\\
0.744135120431133	1.60681685856481	0.497028103161948\\
0.806308037579827	1.66159800091263	0.548153405497722\\
0.868407163507737	1.71062740831277	0.599199521246646\\
0.934676220674764	1.76448356459484	0.647910551823576\\
0.994983441668676	1.81627499769647	0.706145087474844\\
1.05601828200952	1.87000952781779	0.763689518130537\\
1.11861872131484	1.92268947511914	0.822631392863396\\
1.18239123002556	1.97118733942239	0.883338236373165\\
1.24547410558845	2.00886829986752	0.942097873926395\\
1.30541690925659	2.06605985835185	1.00160730671751\\
1.37020522015701	2.1142811032267	1.06388348153475\\
1.43553978055996	2.15908326526873	1.1259099546486\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999628468123505	0.239790642200563	-0.99897927759309\\
-0.939925800908706	0.296042592806576	-0.949064983131013\\
-0.875266349827194	0.341981759663927	-0.899805478039031\\
-0.804988157029969	0.388379733543896	-0.848054750657497\\
-0.730863878676326	0.439183077783096	-0.798524228362854\\
-0.657229628784629	0.486499827915499	-0.74908000212884\\
-0.591572705893785	0.534692114499472	-0.692385359734553\\
-0.523491044983277	0.580256089716363	-0.637898006433409\\
-0.457554556262484	0.626900853575511	-0.579719222240134\\
-0.389307561274564	0.675277867740183	-0.520757303740208\\
-0.321688393728467	0.722238445144696	-0.462161158743266\\
-0.261025051333469	0.772806747316398	-0.398790377925144\\
-0.201063345419251	0.825260249199859	-0.33289621954988\\
-0.142939694616152	0.880967357489524	-0.271365782089549\\
-0.0813910921469937	0.936155200593185	-0.207630848641898\\
-0.0210017469487869	0.98501080558381	-0.146600239202634\\
0.0408571880641842	1.03141430640984	-0.0835191396259772\\
0.102559629102903	1.08339897598826	-0.0226885379086642\\
0.163285941463538	1.13423531389365	0.0368329525571538\\
0.219276401783637	1.17918896804226	0.0982186832816128\\
0.276765559566223	1.23679105028662	0.163320752261187\\
0.333328969610198	1.28749214820276	0.231279035800933\\
0.388619171172642	1.34493843504955	0.292770640756229\\
0.444828414861031	1.40285138095071	0.357407266050898\\
0.494106637458335	1.45481133434207	0.417668955022045\\
0.551519976997145	1.50744282891953	0.479277005462752\\
0.609527334442341	1.56374080085298	0.533384600137526\\
0.660641882932611	1.61065360475036	0.591186262409852\\
0.707875668819173	1.6616160999572	0.644315273213129\\
0.759877049222264	1.70183406754071	0.698100463494905\\
0.807391382574032	1.74113329991917	0.747273110092868\\
0.860306972237768	1.78248401822611	0.806325190862904\\
0.913578169490901	1.82597288384577	0.87063592936746\\
0.969532391995316	1.86960373815914	0.930738166463832\\
1.01990463281503	1.91287429474502	1.00193963235164\\
1.07299453257888	1.95180604141512	1.07103755000408\\
1.12383537811516	1.99496799553102	1.13293339534748\\
1.17997811518489	2.032273860388	1.20544540890979\\
1.23499557658421	2.06542254474042	1.27272747378511\\
1.29846587084545	2.10068936214979	1.33756443870261\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999289387007216	0.237332812311051	-0.99865554709324\\
-0.936795955100432	0.295679216182619	-0.947864624687105\\
-0.876927253238595	0.343276485769654	-0.901835879960475\\
-0.807559195861177	0.394613411621275	-0.854747083355907\\
-0.743768546633476	0.446741482146726	-0.809483242443629\\
-0.678382896751087	0.498546391877843	-0.768793193958187\\
-0.610558805239572	0.546513126155076	-0.724701612024884\\
-0.544798088817717	0.594782594672072	-0.682477760140318\\
-0.477717423893348	0.644362771969552	-0.639171197285377\\
-0.414418358748862	0.691799180516605	-0.600266258985882\\
-0.351400665563637	0.73769750361156	-0.560931573073746\\
-0.285030344315029	0.792222367499755	-0.520799493921138\\
-0.215875518663512	0.839978188612703	-0.482957520864315\\
-0.150297843540294	0.886646079218679	-0.447237042402936\\
-0.0834243279194481	0.941460547367289	-0.410865954985957\\
-0.0120904358143467	0.989775199494328	-0.368771018321348\\
0.0604389596442129	1.03455854433696	-0.321992784550233\\
0.128151640113722	1.08341974135171	-0.279405541600614\\
0.196461201678463	1.12184412337843	-0.236337765105618\\
0.261364979629248	1.16835261839804	-0.194519704650955\\
0.321670162964917	1.21348011410584	-0.148443088243086\\
0.386880370280435	1.25469593481258	-0.101284454693346\\
0.450604139635742	1.29798441047623	-0.0553452158533105\\
0.519616769322175	1.33857252486657	-0.00927014479227918\\
0.586521906558447	1.38208814561038	0.0334872371659635\\
0.651479688190949	1.42906114369178	0.0822244820957161\\
0.715133057155426	1.46881180996613	0.134969932829681\\
0.778497133532508	1.50840607572028	0.184921140176153\\
0.844392620888717	1.55205640548613	0.235492388502672\\
0.913743415717288	1.60113650258431	0.288495733080519\\
0.978645205210958	1.63933218766213	0.338369617629305\\
1.04825500823173	1.68263559166572	0.393018859135845\\
1.12063304513119	1.7377561187081	0.436865577122685\\
1.18924802745821	1.78313708669981	0.487671860194042\\
1.25671338534207	1.82607100488179	0.540897220914599\\
1.33248467847619	1.87102929043667	0.581395060032421\\
1.39846247339973	1.91831311160546	0.624230507074932\\
1.46414328393671	1.9681844481162	0.672364141523025\\
1.53497308785455	2.01054778187278	0.70841517391463\\
1.60973388371968	2.06134501267281	0.757824264378024\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998744597993324	0.239697364611478	-1.00082330309869\\
-0.934967296140122	0.29989064312524	-0.950157034366223\\
-0.86972779897256	0.344447275570136	-0.898492931569805\\
-0.80380434347782	0.395393403286442	-0.847069314899717\\
-0.736630584077776	0.442494611847942	-0.789790776091889\\
-0.674003912521172	0.487020472623881	-0.73099047887085\\
-0.611323579525427	0.536326358550417	-0.679711199720687\\
-0.547947112786439	0.579137292523701	-0.625531639441308\\
-0.481311197084737	0.625684368217938	-0.576752741050633\\
-0.409642341342085	0.671437090276521	-0.524345978719481\\
-0.336718700514058	0.719340455289502	-0.468647733249641\\
-0.263515877624212	0.764537815183044	-0.412902093600487\\
-0.193170181448085	0.817074647324963	-0.355392900262836\\
-0.121621247147764	0.85974469495509	-0.296083232311909\\
-0.0529290729005914	0.913964513283499	-0.234183540893584\\
0.018066553158035	0.967257398950404	-0.174826262009692\\
0.0855842031244479	1.01565889554435	-0.109527439163188\\
0.153506741555135	1.06719276334748	-0.0450340921768153\\
0.220285061205617	1.11310777866069	0.0210252373313124\\
0.281497338579451	1.17102949831046	0.0829191434970286\\
0.339841322499021	1.22475310286617	0.142844238515142\\
0.401649742735817	1.28167213514423	0.201115439123611\\
0.463472286329777	1.32816451866386	0.255587450212393\\
0.529027501161274	1.38937239025773	0.310707537689259\\
0.596295164673068	1.44161626270088	0.360966187991806\\
0.665240306388588	1.49373270512595	0.418294113130643\\
0.734892174207189	1.54703805668162	0.471188238947233\\
0.802609297475846	1.59677301506572	0.519727335807\\
0.876217114705428	1.64423008323368	0.577104341061865\\
0.946329772400645	1.69834838831746	0.636998461431551\\
1.01487012611064	1.74117426820574	0.693202951143347\\
1.07895364097138	1.80104867708122	0.747922193424177\\
1.14008865783622	1.84884542085864	0.792570040054611\\
1.19945130966865	1.90334134584269	0.842317791907883\\
1.25928968363361	1.96176365750833	0.888586581774754\\
1.32203621734675	2.01759594992835	0.933677571088026\\
1.38257667373151	2.0641937818398	0.978972812005777\\
1.44072191073415	2.12339258232747	1.03295774611234\\
1.50546098626268	2.18206423228079	1.07036803043518\\
1.55975887555877	2.23136827473192	1.11391344887868\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998885511378266	0.241910664800918	-0.996976547477393\\
-0.940040387614954	0.29766777320707	-0.951626881813066\\
-0.875761564352633	0.347260468102953	-0.907998660757468\\
-0.816470024118318	0.392983354135737	-0.858395523848572\\
-0.754390311738232	0.436969118715538	-0.807615616507622\\
-0.696814774846039	0.489813934789821	-0.756835415722019\\
-0.638662270138816	0.541508877072344	-0.704843504179646\\
-0.574028968528997	0.591552378645295	-0.647513506425095\\
-0.509217796623769	0.641755340240551	-0.592825936813614\\
-0.443576874144499	0.690388034449658	-0.536188529144945\\
-0.383392334500443	0.745883388683918	-0.481844860460854\\
-0.32076791702083	0.799986152509635	-0.427792737651208\\
-0.262775469604114	0.850507944820221	-0.372664024183134\\
-0.205120722121782	0.902966353198475	-0.317669078495082\\
-0.146466695321946	0.95216406785298	-0.262405454807257\\
-0.0944402357188441	1.00064680946135	-0.211676887176349\\
-0.0387710902211556	1.04811022977455	-0.155471755459173\\
0.0155118148154992	1.09073778226011	-0.100539150071169\\
0.0740883287702382	1.13531226263472	-0.0482031999438352\\
0.133198466176663	1.17946127642741	0.00682531674891407\\
0.186390976823255	1.22438350327784	0.0622041620040903\\
0.240426482745683	1.27381480766936	0.118910359755193\\
0.298220804718212	1.31774535893661	0.182176961892837\\
0.350962282352541	1.36020652557454	0.240485424587223\\
0.415578450780406	1.40564377342666	0.305952817557809\\
0.470425707641884	1.44524272280929	0.372190904752373\\
0.529456695012825	1.48131013532241	0.43712942967256\\
0.585962618128176	1.51817796589832	0.499198162661889\\
0.637974139056772	1.56445863246761	0.565512641325222\\
0.694442306998844	1.61081872437219	0.633828917433982\\
0.744965992305821	1.66223244724247	0.702182438107963\\
0.798239336855592	1.70818277921315	0.770943857544714\\
0.847036322537959	1.75413794824888	0.842854623769122\\
0.900452089866363	1.79544184131232	0.915267609387747\\
0.948305547722496	1.83679549021743	0.983009012267143\\
0.998056758900664	1.88047852779191	1.05674893858474\\
1.05288580690814	1.92371468087948	1.13069712490679\\
1.1109080787291	1.96615330191371	1.20299207227131\\
1.171317220047	2.001858577902	1.27624387367332\\
1.23238388325872	2.03815751318162	1.34446825975575\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00001242079505	0.236996152839202	-0.99819153226049\\
-0.934071827168765	0.296812721566474	-0.94900119376642\\
-0.869154732172692	0.344744304962989	-0.900387001894552\\
-0.79642778770078	0.394936458189387	-0.850653752790028\\
-0.724114088376697	0.438060104253512	-0.801718915695451\\
-0.650537362239834	0.485391800508191	-0.747573480286097\\
-0.57773296631891	0.529078210200821	-0.692855667079673\\
-0.504445910849418	0.582120446020019	-0.638795725563779\\
-0.429242111180558	0.633573562556222	-0.581522457967665\\
-0.355596050621327	0.689397248334908	-0.529820957518047\\
-0.277605823264592	0.744025645700843	-0.47633578096978\\
-0.199464303040165	0.801486135250879	-0.41671253912194\\
-0.122780568721429	0.861266032837976	-0.362785688665567\\
-0.0440789177556352	0.915108996921414	-0.311361944494187\\
0.0376143232755785	0.964246304458507	-0.259084321432278\\
0.114555016102637	1.01717209054488	-0.197963055414828\\
0.187652303337601	1.06501729941302	-0.137974963125784\\
0.26584750854522	1.12235537817069	-0.0722826722553435\\
0.342214514737491	1.17232645876298	-0.00694439717821829\\
0.425095419691448	1.23003949135393	0.0603241347804975\\
0.506051039720301	1.28562175609566	0.127239496273135\\
0.588726789046525	1.3455447752446	0.196363111926027\\
0.672750288388868	1.39837087970005	0.266023417678813\\
0.763300391205067	1.4537587327465	0.340530625352004\\
0.845050678727478	1.51670035775515	0.415465343803769\\
0.933384432083729	1.5761458834542	0.491962714885336\\
1.02078988600718	1.63705539115459	0.571323212294579\\
1.10603932995362	1.70225133901559	0.650189837848793\\
1.18831784754637	1.76770875406839	0.733853873662714\\
1.26777717813386	1.82873884287846	0.812237617839167\\
1.34952679680076	1.9049332078562	0.899655597811849\\
1.43023232104486	1.97248192837176	0.982938615477784\\
1.50815864026067	2.03757105632708	1.06420760837613\\
1.59801144846906	2.1096956557521	1.14491569803146\\
1.67678481840977	2.16956626187837	1.224696605501\\
1.75765028520496	2.23070549876961	1.29624968926503\\
1.84149806923614	2.29541484691098	1.37234131875728\\
1.92514715181643	2.37122963631975	1.44830650358269\\
1.9971120621971	2.43906794267888	1.52812329081828\\
2.08444550915334	2.50715141416051	1.60504175661068\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998959593193632	0.240823525972835	-0.999191176356675\\
-0.937010795032799	0.300216708677304	-0.950798757480133\\
-0.87334516007607	0.346598183946491	-0.898595061458361\\
-0.807243845062648	0.395176248501185	-0.846686296870997\\
-0.738726750337258	0.44901308854195	-0.792835340129378\\
-0.674809951292105	0.501516665581982	-0.735094708555018\\
-0.613246013689922	0.565083374984484	-0.683987868051571\\
-0.54891879701058	0.620154772982619	-0.626935790129387\\
-0.494581278850229	0.678818587696362	-0.570675149732432\\
-0.437961561225523	0.736192162727018	-0.510339127697848\\
-0.382006970165087	0.792729988358544	-0.456813446877408\\
-0.324940245612966	0.845608906805838	-0.406925583598001\\
-0.265459355197348	0.901028253007747	-0.358317956109875\\
-0.208780879225109	0.955769508095268	-0.312279004473023\\
-0.148822244643829	1.01457655363819	-0.268603560105727\\
-0.0903744801752249	1.06876803256187	-0.224527404626605\\
-0.0304028315660734	1.1214519565387	-0.178812812022271\\
0.0261867198232864	1.1799634297082	-0.135150437802118\\
0.0842436869465917	1.23110491121767	-0.0898054785672626\\
0.146511414082153	1.281126012722	-0.0454046688802251\\
0.200467321021819	1.32709893484523	-0.00216007815982188\\
0.257103877359511	1.3730911663498	0.0435746712649696\\
0.309144408186614	1.42404195628767	0.0868939116132905\\
0.360342798483346	1.47345591400591	0.134641943185379\\
0.414149720803435	1.5178097101618	0.18064810862728\\
0.472514186448061	1.56764316127003	0.229361709620298\\
0.527780466255169	1.62124292067037	0.283387300713208\\
0.581130005235912	1.66993874378876	0.342200478945902\\
0.634407725475579	1.72488377066727	0.396223324057947\\
0.692139517135441	1.77217418895066	0.454341751580407\\
0.743921075392271	1.82214649284332	0.51454618724282\\
0.79654300926419	1.87985002499337	0.577410328918531\\
0.854115664323511	1.92543174209933	0.644217003467266\\
0.90022435501774	1.96793687696675	0.709619137513361\\
0.966890599445676	2.01567905004838	0.781902994752975\\
1.02199232452066	2.0599629255512	0.849641584649331\\
1.07923862695916	2.10860169005699	0.922623894353172\\
1.13476459690299	2.1487117346492	0.992759550697976\\
1.19308301456914	2.2052443731381	1.06277004046379\\
1.23738648649508	2.25464620386159	1.12787503622771\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997171050210162	0.242309090692241	-0.996856148079034\\
-0.937953212107463	0.291755435391893	-0.950300294838887\\
-0.874338901098554	0.338380256899547	-0.897086027350147\\
-0.809936557705549	0.386072686519136	-0.848017856588324\\
-0.745226017347575	0.428677698644661	-0.794412132155935\\
-0.682260929886819	0.46539293664249	-0.741298955255845\\
-0.614482118094976	0.501047798801286	-0.686561242554906\\
-0.548526305100165	0.542715800119847	-0.631653466289102\\
-0.485189318634579	0.576620933496199	-0.574101718415877\\
-0.422431078751044	0.615974476458091	-0.515009777648744\\
-0.361523563236864	0.654856634204266	-0.456808022333485\\
-0.303253140899515	0.694586018559849	-0.399680829704244\\
-0.246141853522201	0.728963767175671	-0.336187767877396\\
-0.18904891675754	0.767986409842892	-0.277333602911615\\
-0.134219016517722	0.808695614020911	-0.215408219074509\\
-0.0747573033008048	0.843606849702167	-0.156692217518261\\
-0.020439103678019	0.880994131762678	-0.100807855237628\\
0.0308231566903629	0.920606330591664	-0.0416489872792073\\
0.0808987896925517	0.960693259966886	0.0132311483872555\\
0.13503506867386	0.998287652151354	0.0690422961662859\\
0.189121798651164	1.04605663037633	0.126899421908199\\
0.241632307076704	1.09533521782169	0.18321581161012\\
0.289088449535143	1.14818569882429	0.240838878250628\\
0.341635793937148	1.19844786306698	0.298515739981637\\
0.390620499027097	1.2514446960535	0.358623049495604\\
0.44037802866175	1.3057942783143	0.423754115037171\\
0.492366191100857	1.35979320576295	0.487627553340278\\
0.546959208579579	1.41876008517543	0.548116684093643\\
0.604939244749512	1.46904829359612	0.607578124750659\\
0.660573994833797	1.51906110742651	0.670788838088915\\
0.714346576479404	1.56530781521669	0.734290947927073\\
0.773232220495355	1.61769114305016	0.795908073882546\\
0.827056078168975	1.6685483539366	0.865222302470622\\
0.884649168799789	1.71609847453967	0.931142573225979\\
0.94279561381222	1.75541818859283	0.996761328191133\\
1.00365240816101	1.80281039374679	1.0601130003862\\
1.06139464529507	1.84850973278397	1.1218372490159\\
1.11176811346607	1.9064506906578	1.19580671838589\\
1.16752068001643	1.96114731062464	1.26199259438727\\
1.21242801334302	2.01176867289048	1.33151190333676\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99881542207184	0.239720675091591	-0.997009706141376\\
-0.93765438649253	0.293302287911362	-0.950338539456461\\
-0.869224040670987	0.341062677973897	-0.908219846069401\\
-0.802830145121424	0.384962598225273	-0.860089905537413\\
-0.736439119814415	0.428485983725362	-0.810663876648319\\
-0.6720725014157	0.473118919162488	-0.76157666135308\\
-0.60245268510537	0.512837574179635	-0.713395481161917\\
-0.535784511961406	0.553593169948548	-0.669184674280052\\
-0.46943362475402	0.590316720273654	-0.62140876858919\\
-0.405174768763193	0.627116208757717	-0.567639410473795\\
-0.341413477227322	0.658247247352008	-0.511749739559889\\
-0.274952109312681	0.686808168155472	-0.452594442425038\\
-0.212133355944118	0.712822282752146	-0.392052513313729\\
-0.150238256484949	0.747561761275763	-0.33143886344707\\
-0.0880784706303454	0.779728865981586	-0.274808037601344\\
-0.027241009211033	0.812778617646553	-0.217757421531806\\
0.0295094920265874	0.845846977734625	-0.158777798795608\\
0.0844644599779759	0.87003809891487	-0.101148612229172\\
0.136126783426729	0.901627949880876	-0.0450344538206197\\
0.185331432392828	0.934700539268137	0.0137375670675768\\
0.239245711797525	0.970980696186618	0.0698762516650012\\
0.293065230290556	1.00615936608342	0.126745002362658\\
0.3467361272706	1.04080800777651	0.181111997680564\\
0.40050250221656	1.06991908897503	0.243173940796566\\
0.45338491730481	1.10579333147593	0.298056240101713\\
0.505927408420464	1.14584979740738	0.358049174784228\\
0.557187442254682	1.18059088957487	0.419798414594443\\
0.612581072679843	1.21840820756129	0.480505434749133\\
0.668686584045907	1.26003803946999	0.538491828149655\\
0.718193141856078	1.29689957895612	0.598880508895309\\
0.768156830112073	1.33572758034375	0.660334870951474\\
0.823054801709109	1.37014354126151	0.721016806931345\\
0.872970513785764	1.4010853048614	0.778265407102967\\
0.916461767262063	1.42736373941219	0.841438082322793\\
0.9581234247532	1.46346311122217	0.908784035508842\\
1.00940237580738	1.48260922256318	0.977998602327537\\
1.05518353083684	1.50182569737712	1.04318962620448\\
1.10058996882661	1.52886099630075	1.10921458286862\\
1.14632596156738	1.55772619054662	1.17340932362644\\
1.19255061153981	1.5795581201526	1.23465112685251\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997012033215349	0.24330068421086	-0.997794551516377\\
-0.935046798425955	0.298331143526988	-0.948599736134172\\
-0.877277236483502	0.342459339848217	-0.902726415850275\\
-0.814669154167901	0.393082259395234	-0.856981882805012\\
-0.749920772611216	0.437942885646406	-0.807679066289984\\
-0.683661094653007	0.48777849040452	-0.755918285862468\\
-0.615854413113115	0.535417746192292	-0.699236077390068\\
-0.547529425554012	0.585554814945076	-0.646623772223913\\
-0.480691576204443	0.634305277389931	-0.595065014043382\\
-0.419153196352777	0.677119078228366	-0.539491424340906\\
-0.355294414861889	0.721092523051041	-0.486892311783569\\
-0.2908482045041	0.76611903355803	-0.431675315929284\\
-0.223698482560711	0.813334032213213	-0.37485043208904\\
-0.152302963352282	0.858028083916582	-0.32025107240638\\
-0.0841121191825706	0.914284559544938	-0.262546904637881\\
-0.0112241195221479	0.960153916225502	-0.207302417851785\\
0.0611541607231782	1.01720944185419	-0.154038639758797\\
0.130875427844638	1.07857116786437	-0.0947173547830037\\
0.200704812438192	1.13373001560595	-0.0419674127951958\\
0.274121980040014	1.19084234531123	0.00894577875177411\\
0.347242506776232	1.24223765103077	0.0546834713958657\\
0.418169622218477	1.29420207593525	0.0981704153936394\\
0.493912617695954	1.3510320642693	0.142897087055774\\
0.567470216808397	1.41680221662017	0.188926013040699\\
0.642893850621634	1.4797344126437	0.235581895090041\\
0.712250478568749	1.54312912430285	0.277834221027388\\
0.781320156877461	1.60995409592037	0.31834794263671\\
0.851328636946908	1.66759827741845	0.356788027957719\\
0.922317692307335	1.73136632070841	0.394917838158719\\
0.993139273470782	1.79275987572677	0.433501894570389\\
1.06208109058572	1.85260995675399	0.478472772888404\\
1.13085998158348	1.9080268871646	0.526415361146105\\
1.20561838425786	1.96031745717501	0.573650695661233\\
1.27940775815342	2.02909199764573	0.615813676925079\\
1.34812676516791	2.08579132681223	0.662019367126311\\
1.42323235006741	2.15256453372894	0.709438559981014\\
1.50163366840412	2.22009740292004	0.768343110669741\\
1.57865052890917	2.27819189196283	0.825738759724162\\
1.64886201638829	2.3423943225935	0.882816717518549\\
1.71839996723213	2.40376474448927	0.939394887715484\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998176300892813	0.237865833133155	-0.998194406771928\\
-0.937303139918043	0.301206038514602	-0.955159411637351\\
-0.877955500618571	0.341612321654935	-0.901700143340558\\
-0.815697139260197	0.38866548598159	-0.847394338464941\\
-0.754143895367212	0.430870756298495	-0.795036705558929\\
-0.695123827072046	0.47192298746436	-0.740694369683829\\
-0.636612473235756	0.513406346603183	-0.689101644847527\\
-0.575032286854936	0.553967385215815	-0.638111316675945\\
-0.513083470553701	0.595876225786883	-0.587766782640912\\
-0.444961479073543	0.640597481984597	-0.537032591693204\\
-0.375109129653081	0.686710488668791	-0.487021612306725\\
-0.305788006071599	0.738137242989012	-0.436234430769775\\
-0.236235057231604	0.790671883468174	-0.386684809936003\\
-0.166272574417097	0.844525951527236	-0.33937749510591\\
-0.0957488805514085	0.899234206104683	-0.294071544167977\\
-0.0287840323751033	0.947013920874275	-0.251677305336781\\
0.0370096021764849	0.998177322843597	-0.217118878873802\\
0.106559765166078	1.04915798202384	-0.185801895940089\\
0.175524576186528	1.09731864515887	-0.159031018255411\\
0.247090072300033	1.14257724693	-0.130554407973902\\
0.320650086654296	1.18591216187324	-0.0992287650876434\\
0.396506940491463	1.23054750219539	-0.0663487510487194\\
0.473262288155237	1.27090201263435	-0.0358039625641331\\
0.547150548605702	1.32022030747578	-0.00922259580246202\\
0.617612867216872	1.3638636895872	0.0196621500621873\\
0.694060621126363	1.41300564579005	0.0496943384016945\\
0.766817069046539	1.4620538715338	0.0795899787416229\\
0.840694727531361	1.51379585644396	0.107119387534553\\
0.916371968829657	1.55932985424325	0.137390991854598\\
0.986270069766298	1.60614246401446	0.157036274438943\\
1.05994897286179	1.65659647997805	0.177171941443293\\
1.14236102668261	1.70095270256798	0.198267012071467\\
1.22077245933225	1.7449746750989	0.217168008824423\\
1.30174902847641	1.80233641298785	0.236217088454865\\
1.38498294775674	1.84450456804972	0.257150003929835\\
1.46323256195656	1.89905012349442	0.281349483875322\\
1.54165447658842	1.94970008162033	0.299185692966051\\
1.61540358604717	1.9928729763946	0.317860407036865\\
1.69469191291839	2.04210792162139	0.335359285789529\\
1.7690063979206	2.08325071458976	0.348953423649663\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999026809756535	0.240084072736964	-0.997186525363316\\
-0.937873815393769	0.28967113699289	-0.947090346365476\\
-0.876860272021384	0.336162596714522	-0.899783480302242\\
-0.815991866953933	0.374145979761952	-0.845304774590324\\
-0.751994476824377	0.415632959899356	-0.794475312091002\\
-0.686778194362638	0.458797438851635	-0.739701187755375\\
-0.627605385818242	0.503830515606959	-0.68005789915831\\
-0.566547545387096	0.545637617384054	-0.622607224593526\\
-0.503936658596177	0.594855401902417	-0.564993427143466\\
-0.438320011588788	0.642782608333275	-0.504658429485865\\
-0.375478476232125	0.687192464260465	-0.44526305176219\\
-0.308159911482955	0.73004697263157	-0.39000716087015\\
-0.241156607477187	0.777411022254915	-0.336463856328745\\
-0.174061770631356	0.82403155585738	-0.277345976009463\\
-0.10486370531114	0.873540001962725	-0.215885276501215\\
-0.0368351010875903	0.921968606119207	-0.154301419672757\\
0.0352965784408696	0.969923748653492	-0.0985417381874972\\
0.107365650539453	1.01483411074924	-0.0439649237183216\\
0.17852823118301	1.06499157184381	0.0123500405207406\\
0.252988118991231	1.10798188326143	0.0692998063376193\\
0.324674321103164	1.15050947084429	0.121003339138511\\
0.397949577684284	1.19501616192912	0.180555936746498\\
0.473364431316479	1.24268040914959	0.239097947298748\\
0.545629887653631	1.28511754885857	0.29474247897868\\
0.624062823757318	1.33446554971271	0.348368203238439\\
0.696902145321275	1.37974103052407	0.39702875778487\\
0.765864186848373	1.42323863456084	0.448953727889677\\
0.835407573261454	1.47151330209006	0.496716204694803\\
0.911822953534982	1.52218291835479	0.545612252387766\\
0.987355304340101	1.57533580662666	0.597840773942296\\
1.06699119232964	1.62074241684759	0.640775965105837\\
1.1443542979802	1.66500212822931	0.694792355215661\\
1.22386349796091	1.71069188308638	0.740759768098063\\
1.30120078908873	1.75939351204546	0.780265499927767\\
1.38056713543597	1.8047598494121	0.824418111341939\\
1.45858501764373	1.8591800544068	0.867882324642663\\
1.53586213295151	1.90467116231381	0.911349175518199\\
1.61166310691167	1.95393255513782	0.950029641586803\\
1.69261146201018	2.00780060703468	0.993757001465706\\
1.76463446750705	2.05253411494051	1.03503570205977\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997879915141782	0.240723834463188	-0.999168889014659\\
-0.93748846371567	0.29578431763191	-0.949112663857146\\
-0.877506879767706	0.340666471202947	-0.901367203309815\\
-0.81828102223304	0.385778399581687	-0.851568414035801\\
-0.758475161648497	0.41728631044418	-0.790800486192482\\
-0.696758803682568	0.450605705924523	-0.733853644270089\\
-0.63012978521123	0.483857723835722	-0.676504194955924\\
-0.559901449700274	0.51515558376121	-0.620472334296321\\
-0.486488222387591	0.548557895308757	-0.560535094181325\\
-0.414254584382845	0.58645423104225	-0.50402883411144\\
-0.34326554769929	0.620158009652069	-0.444362201889022\\
-0.270252541405304	0.656875971545244	-0.386990669966016\\
-0.196781722409483	0.691933541867233	-0.327018374141601\\
-0.119339712032173	0.728207606773953	-0.270446554979799\\
-0.0392375618379667	0.762284876798912	-0.212516762445096\\
0.0415057536030486	0.804345008496095	-0.157295862094667\\
0.121531736053101	0.844624971425868	-0.0991319209041784\\
0.203639614171569	0.888855805124475	-0.0394044528791185\\
0.289487572404761	0.928857570711002	0.0231126599104726\\
0.376117204545984	0.968847786826805	0.0854360726969179\\
0.465095317817891	1.00740476415502	0.146591123438999\\
0.557493651169457	1.04422051330196	0.203524848471919\\
0.646824089656116	1.0780964891026	0.264323063934983\\
0.742863385230756	1.11676734553909	0.321822907861678\\
0.837293289437147	1.14754467520788	0.378478008567543\\
0.930407683833772	1.18480623858365	0.435963850931195\\
1.02223084245309	1.21310923073638	0.493826434766483\\
1.11237642567779	1.24304141275884	0.552845848946321\\
1.20135571679794	1.27085977331896	0.607994156445073\\
1.28703691402899	1.29764923427642	0.66330445628818\\
1.37928290914193	1.32455573233626	0.723390635976518\\
1.46633572506791	1.34360319370611	0.784467614375736\\
1.55746169070873	1.37249197476557	0.839519989063708\\
1.64768587859859	1.40569684452051	0.896841338311787\\
1.73632235954012	1.43182115355377	0.95415872997896\\
1.83167783360269	1.46284562124802	1.00858384733011\\
1.92885825317725	1.50539079342544	1.06530005971972\\
2.01950827512859	1.53759128973342	1.11422387640636\\
2.10790145732014	1.57350020728463	1.1586601154678\\
2.20074517062483	1.6147083344714	1.21414273416725\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998900049507609	0.23946258346467	-1.00236186302348\\
-0.93806067009773	0.302519151556484	-0.950950613184611\\
-0.875000445130725	0.34699679525257	-0.898855919643974\\
-0.807523332820102	0.399939492504463	-0.851285822771237\\
-0.738732635501012	0.445773708896972	-0.796963483493859\\
-0.669092704552241	0.501131436994574	-0.745389357327111\\
-0.60005637424219	0.548687998038143	-0.69339381968737\\
-0.533763555398126	0.601989143068871	-0.640513674384112\\
-0.466344084745919	0.654606823009821	-0.586634068745826\\
-0.398007404048346	0.710458816879273	-0.538198073873161\\
-0.327189986256386	0.759940545504296	-0.487007320007984\\
-0.257946654787438	0.809827569760894	-0.43996819690865\\
-0.191281519487314	0.861244261710227	-0.390965179810164\\
-0.12319918263032	0.911170938031984	-0.338469896876595\\
-0.0529063399520557	0.960457796370175	-0.284931000275585\\
0.0121370572840651	1.01574173164898	-0.229259852347004\\
0.0765303206470667	1.06787582952735	-0.170580592335158\\
0.143069308250466	1.11454289464276	-0.109509190008538\\
0.213559308238234	1.16392499238551	-0.0477897791321512\\
0.28721610406568	1.20789589857908	0.0114510218586177\\
0.358532529241753	1.25616075697514	0.0722959106392453\\
0.429327405177635	1.30578607630807	0.134477890687541\\
0.497203519831442	1.34870442139244	0.203180353825679\\
0.562254232382814	1.38330899227083	0.272396949975959\\
0.627976942961598	1.42390989812496	0.339621055467874\\
0.692711245350603	1.4621327251151	0.407176703813703\\
0.762052428146664	1.50546194634553	0.471666439366706\\
0.827083674656355	1.54118103022161	0.533528892923807\\
0.890655771335466	1.58813836406917	0.599556143715644\\
0.954075158083042	1.63126448288713	0.663433784543702\\
1.02342161611523	1.6765237438917	0.71983928635955\\
1.08952057837475	1.71923291006883	0.788377876124591\\
1.15523463036122	1.76660637978147	0.848800343627862\\
1.22134094805314	1.80706547855688	0.911423939221318\\
1.29078921686894	1.84387595527152	0.97058517630706\\
1.36389256135558	1.88184790069749	1.0292848380178\\
1.43414786255193	1.91928223170295	1.08661624506537\\
1.505150003754	1.964961398413	1.14547873735732\\
1.58129992660558	2.01361853179068	1.20726886686901\\
1.65858077122085	2.04374268460611	1.26623010975458\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998224655000947	0.239227642880987	-0.999584344680839\\
-0.938183365774556	0.296710244772038	-0.946828230357148\\
-0.879421108616024	0.342070775244995	-0.900653004904123\\
-0.82166056995277	0.388358721989544	-0.848728249590131\\
-0.758672746177095	0.437676404337165	-0.788815227408785\\
-0.696234678416448	0.483323644158982	-0.729668316975941\\
-0.630062237071506	0.526957723359955	-0.667599634269856\\
-0.56084383392734	0.573351786524257	-0.607117278261738\\
-0.494568391194088	0.623461572408495	-0.543282847000905\\
-0.430201062649796	0.67302141323129	-0.487191414986097\\
-0.365669219281314	0.710817066887927	-0.429540589155897\\
-0.301635764688841	0.757472276670488	-0.374631948451446\\
-0.238711485346451	0.794631524275093	-0.317800635707675\\
-0.176862364651176	0.832099208634916	-0.263700362004811\\
-0.113587870139848	0.871146482061936	-0.205391907212626\\
-0.052673869772478	0.906205089617722	-0.144114067397178\\
0.00804271305616219	0.948575148488696	-0.0829298377588602\\
0.0674849271209098	0.982415880306125	-0.0180213627134236\\
0.128903075544697	1.01730880235047	0.0530535798275169\\
0.190907749431681	1.04886893016138	0.121320853201782\\
0.252379156510826	1.08621983747133	0.193804436751609\\
0.315139499419469	1.12452651095244	0.26797162831777\\
0.378953618905509	1.15149262954047	0.340684298480034\\
0.442835878587877	1.18590449879145	0.416311108173326\\
0.505513346867512	1.2138013079254	0.484497381543919\\
0.566919430330379	1.24261920680413	0.555585856389909\\
0.631971287720878	1.27395118423471	0.631424174361061\\
0.693379736982473	1.30330890834518	0.706850974285168\\
0.753057309240758	1.33605743490273	0.779416091847091\\
0.816047411858848	1.36629210562833	0.853668317339531\\
0.884083930531003	1.40540869704547	0.926000431825431\\
0.947072681365749	1.43618280163544	1.00001698100536\\
1.00663420203886	1.47123221470779	1.07640235977588\\
1.0691447990303	1.5009622286756	1.15093479724517\\
1.12606186973462	1.5446864200095	1.22701164262742\\
1.17974472675541	1.58769448825149	1.30355404511283\\
1.2329264835621	1.62665571917759	1.37577149928208\\
1.28210258936641	1.66271999651647	1.44977142231725\\
1.33055578649617	1.7028061616776	1.52665462199228\\
1.37903574812156	1.74629378364962	1.60168294795199\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00068039801429	0.240653644756187	-0.999024335894011\\
-0.937253295640987	0.300747056284595	-0.948466637951207\\
-0.873652877040978	0.338650004030541	-0.895336306301265\\
-0.808113604720478	0.388253193978652	-0.841404607716261\\
-0.743978307833414	0.436430858469606	-0.788134022778441\\
-0.682478371160331	0.490718587451654	-0.737315538042155\\
-0.620992286937752	0.5365139577963	-0.68702622812266\\
-0.559126266454237	0.586339083846549	-0.638445314630722\\
-0.494960379644859	0.633528757751934	-0.589898566209941\\
-0.428543946918859	0.683150244550394	-0.542683692201893\\
-0.362373878711569	0.73042517132893	-0.492837526232333\\
-0.292264814548535	0.778709195805616	-0.443338481202199\\
-0.222913209015542	0.818688459852304	-0.39347693392683\\
-0.151905178353261	0.855789346155398	-0.347375085952224\\
-0.0786397332109598	0.893602641023956	-0.298894449829859\\
-0.0083435986758045	0.933263829790044	-0.255519614643458\\
0.0692654400206779	0.972730838622875	-0.207740520051098\\
0.143898911173719	1.00587304301728	-0.157196654923438\\
0.224904696508977	1.03794175311786	-0.110746295232362\\
0.308109665172005	1.07450635599904	-0.0650790587178632\\
0.391693928912089	1.10759844889851	-0.016851449573118\\
0.475247228923485	1.14339743846377	0.0330466799342419\\
0.558987369576932	1.1779462152993	0.0877520837481897\\
0.641236597108186	1.21279989619249	0.139539230690144\\
0.730327880690867	1.24736327756213	0.196787522417735\\
0.818403581360737	1.27869592800771	0.254486754886065\\
0.911133894349329	1.32304172617135	0.311510344469394\\
1.00196265849277	1.36857489729479	0.363292126884496\\
1.08499303940429	1.41039054155304	0.416193982274278\\
1.17357355895132	1.45437433853469	0.465193744115268\\
1.27108916573045	1.49585615817136	0.511198188920007\\
1.36738815203217	1.5288777946603	0.559249988865571\\
1.46459792584918	1.57099099022238	0.60704842066653\\
1.56212782255143	1.61255482846046	0.657140249559243\\
1.65101905229456	1.64009040659743	0.697355172143784\\
1.73689753157938	1.68738904946681	0.743162119241309\\
1.83612693015357	1.72298066468903	0.788077066694301\\
1.93577383028603	1.7571649821941	0.834936806521095\\
2.03580061539425	1.79740284902888	0.871827160397645\\
2.14640774918638	1.82927946907133	0.91891253168607\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00078365475287	0.23992355535741	-0.999728671012028\\
-0.935891642953166	0.300091825089731	-0.951474389462341\\
-0.87418466838095	0.346093476197099	-0.909218351198902\\
-0.812655596659914	0.38997905399921	-0.866003938379414\\
-0.752169420156563	0.43787424959484	-0.822649289058851\\
-0.693160374216775	0.485257210769055	-0.783997105360234\\
-0.633899961413753	0.536927934143049	-0.750349007416267\\
-0.578063148420872	0.585347426857786	-0.713390213594638\\
-0.522336889168724	0.633788617358528	-0.680267083935142\\
-0.466170272683795	0.679281679845899	-0.648519521131764\\
-0.413201259798065	0.729604239953143	-0.61380063664545\\
-0.356193498793296	0.777507316190032	-0.577618642803768\\
-0.300237980555567	0.824550367130647	-0.539948180551264\\
-0.239572284860228	0.872342499049926	-0.501372323047942\\
-0.180259819052109	0.922921441578816	-0.462921887665123\\
-0.121082899804986	0.974075155469182	-0.427164662472606\\
-0.0596028969316553	1.02779599155048	-0.389515978863963\\
0.00501546932763867	1.07894707697658	-0.348259722788119\\
0.0710579821881429	1.13287548301642	-0.309723734836253\\
0.14031608034427	1.18204009515857	-0.272939079172506\\
0.201524037587837	1.22856440719882	-0.238853614006538\\
0.263305609475994	1.2749900556921	-0.205138519084251\\
0.32685918959988	1.32175041691463	-0.173873034309376\\
0.391412762787077	1.3758752709622	-0.14299065739635\\
0.452820392377637	1.42970299149503	-0.115271006907894\\
0.517680455999868	1.47537224732817	-0.0883101602986723\\
0.579419045623243	1.53030767951344	-0.0581559539972585\\
0.637925300760748	1.5806756508248	-0.0350750467162361\\
0.695185422632207	1.63571118302487	-0.00440397548219863\\
0.756929900314464	1.69009717857704	0.0185571639265925\\
0.815811620634022	1.75058499785149	0.042499890303336\\
0.870765183520883	1.80180156512811	0.064911783031098\\
0.928885152338001	1.84612847431331	0.0876981845852584\\
0.989320626855028	1.90289284182915	0.104575673815243\\
1.04275871276515	1.96252053390895	0.120934328141935\\
1.09530686760527	2.02619255868345	0.1387665029957\\
1.15094350015327	2.09891026242926	0.154727215184451\\
1.20222732319365	2.16430494030975	0.169206799873526\\
1.2573556028871	2.22674555926012	0.181193062032712\\
1.31218258441105	2.28963419120086	0.191422453652016\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997765059396343	0.239368119619885	-0.998632467358541\\
-0.93937373323242	0.30214329108609	-0.949185409875145\\
-0.875430882826985	0.348818635030752	-0.899319098786669\\
-0.814920588751239	0.390444458877849	-0.849219374066013\\
-0.756449272533883	0.434456193704606	-0.804731821703027\\
-0.697587230861426	0.479936607372494	-0.758398834170475\\
-0.639413273211574	0.532570180522667	-0.716201607484398\\
-0.583250669876915	0.580930796622951	-0.66750582265269\\
-0.527361234888502	0.625535916742555	-0.619366080362518\\
-0.473860540054439	0.675138429741735	-0.573455403431676\\
-0.416842602137691	0.718787849718638	-0.526531922360328\\
-0.355517228729186	0.761941008670046	-0.481906741047513\\
-0.29924429795684	0.797860286506303	-0.43411365788437\\
-0.241579316760711	0.842665495279437	-0.38576965554492\\
-0.186214436407172	0.884510695935943	-0.33955466820198\\
-0.131472460259029	0.922322507515103	-0.291391040471825\\
-0.0818283018778097	0.965781306244273	-0.243710623772155\\
-0.0289450444715565	1.01362678155263	-0.196341134494746\\
0.0192766868295891	1.06065271318524	-0.147124525310489\\
0.0663651930763715	1.10930768509397	-0.095297947451749\\
0.117825522326872	1.15754189666042	-0.0483557043478084\\
0.164682153080368	1.20379487712617	-0.00279573383468452\\
0.211010479540805	1.25258364544966	0.0411455465734933\\
0.255594040030545	1.30692149575259	0.0922078762991131\\
0.298254564870538	1.35645848800623	0.142000608966418\\
0.342873876235389	1.40253907038574	0.189173183692991\\
0.392926276047407	1.4486794048328	0.23175092839643\\
0.43680424289492	1.48816583448801	0.276156170773253\\
0.4807378215762	1.53137364047456	0.322775513737631\\
0.526620198531542	1.56920228882126	0.359127831373691\\
0.56591489672637	1.61693229148691	0.404238742203233\\
0.610099917813616	1.65270722008485	0.447338321696072\\
0.652502599965383	1.69384746474384	0.485782584780267\\
0.700410178129929	1.73198556856864	0.52402903078929\\
0.752113576201318	1.76889797773974	0.565405797293733\\
0.801923949775538	1.80660358681109	0.605765402145737\\
0.857822291965766	1.84933557779032	0.644559486875519\\
0.914588074077971	1.88384810618892	0.689810740450099\\
0.961631798383387	1.92606158107412	0.731858711330456\\
1.0148826543844	1.96115444333319	0.774784027441618\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00124092589185	0.239816003778784	-0.998979463466204\\
-0.937288483883964	0.298652216485728	-0.947305080414681\\
-0.874324015956683	0.346679988346124	-0.895911654551714\\
-0.813086423541777	0.396488056541292	-0.843166313898894\\
-0.751010436713365	0.446269804704144	-0.78817970307042\\
-0.682882612520197	0.493528138625298	-0.736862023324279\\
-0.613861780293297	0.545395910931668	-0.682527468420955\\
-0.538838020915168	0.590867343909261	-0.625300948241179\\
-0.466039239828263	0.641714009902162	-0.569903590745812\\
-0.398667635275314	0.69222350235383	-0.520227774555629\\
-0.330008627457289	0.747162137589701	-0.46170774691253\\
-0.260499094905648	0.801375354698887	-0.40616405740866\\
-0.186767739138402	0.856294633077699	-0.351163497386381\\
-0.111019062347564	0.908056769338158	-0.294500064696019\\
-0.0350835522365496	0.958857705356086	-0.240772170645303\\
0.0426463628396927	1.0186034213848	-0.190925113936523\\
0.11791103936777	1.0705704139845	-0.141053473742598\\
0.197839296599261	1.12843363279935	-0.0872794812274623\\
0.277347790307844	1.1823768445215	-0.0310909748515738\\
0.360988620334964	1.23250037248435	0.026051780568783\\
0.438124102287111	1.27967137325163	0.0790201668357556\\
0.515206366190743	1.33008348979629	0.129780283140996\\
0.599816880653003	1.38299679982594	0.182631115781806\\
0.678888828794389	1.43166401753439	0.234165040762675\\
0.758029893448463	1.48160154547055	0.286636606059209\\
0.841015536434754	1.52993908396869	0.336523085378486\\
0.924889234355651	1.581273031991	0.381659253479001\\
1.00387249973436	1.62711092001131	0.425831594133192\\
1.08168968192146	1.67569786099973	0.463410534659372\\
1.16164203108494	1.72351386188058	0.504984800696315\\
1.23737000582405	1.77232198652142	0.549479689877577\\
1.31104377052331	1.82690193330057	0.595304293111153\\
1.38668724076	1.87766090010812	0.632646767553519\\
1.46437653667485	1.92354642765666	0.674047007503459\\
1.54456738776447	1.97765707938978	0.710337580898264\\
1.62013027426845	2.02878200653533	0.745168892467828\\
1.70279727725444	2.08362349291647	0.787683450570283\\
1.78568175922823	2.13599486884661	0.819525740697244\\
1.87154876593784	2.19139625223957	0.863728576209412\\
1.94806169574255	2.24685221306749	0.907639684684533\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99935194721902	0.238681935338578	-0.998614880487704\\
-0.940335836971935	0.294976492649077	-0.948870499024057\\
-0.874908791475569	0.341477802018139	-0.896921152791689\\
-0.812388641867099	0.385690279888144	-0.844281874115211\\
-0.750864214281315	0.429173650735838	-0.792088891824479\\
-0.690905511463685	0.464874821347287	-0.740351533534099\\
-0.631977740516516	0.503337534656834	-0.685425691263554\\
-0.571132209431751	0.54134772890941	-0.631745062895502\\
-0.507316451248349	0.579404089114587	-0.579542816811058\\
-0.441180989267618	0.615904911165074	-0.528489391519457\\
-0.372345206888199	0.650356337398777	-0.47468554690201\\
-0.3042245244206	0.688509812480207	-0.425825793298077\\
-0.234662626611892	0.72125536451384	-0.375200019770466\\
-0.163090084788497	0.760131401500791	-0.326837971516642\\
-0.0893268737884853	0.791805202790887	-0.279677400815967\\
-0.0183310397317188	0.838870042194565	-0.230546207273301\\
0.0587946373017586	0.879888778294201	-0.187346580087519\\
0.129542188948448	0.928790274326802	-0.146944594367335\\
0.19870398092916	0.97008979090525	-0.106744648497142\\
0.268992986614762	1.00845715728851	-0.0587876227145755\\
0.342444831359641	1.05597310529209	-0.016633186444905\\
0.416066471449191	1.1013404563555	0.0303418665508237\\
0.493292186449519	1.14913228388169	0.0724549004087658\\
0.565144821047364	1.19875654035141	0.120335642148666\\
0.631988359088721	1.24445046761545	0.164866528774112\\
0.699383810166387	1.29010785268828	0.207833740504836\\
0.766648989026749	1.34489441145531	0.248559227784297\\
0.833580294365854	1.39385174978063	0.297406458174374\\
0.901497318434043	1.43850835907576	0.346483250157958\\
0.966442046604626	1.48763067637605	0.392314535904749\\
1.03047451970741	1.53159672115588	0.440687899918605\\
1.09051333003387	1.57761600039227	0.485585283586414\\
1.15272401877982	1.61953124886624	0.534540816773247\\
1.21364671499112	1.66189468245294	0.57786534400908\\
1.27806458218462	1.71141740171944	0.618109534977801\\
1.33858492863642	1.75846661187408	0.665612352640433\\
1.40684406280712	1.80841245433489	0.704197487856624\\
1.47287973581568	1.85293521433314	0.749909007172522\\
1.5436681275598	1.89714042979675	0.793034464721989\\
1.61550488564297	1.94724852083146	0.834530127630623\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999634859621356	0.239271779481475	-0.998679462684257\\
-0.936111764381054	0.296283614453489	-0.94831683958489\\
-0.879129763640786	0.344920328813215	-0.89736794283437\\
-0.820567957889284	0.392716186502721	-0.844863550836345\\
-0.765485602045061	0.443495726580834	-0.789972709196182\\
-0.71005856716443	0.497655503148952	-0.732126627113771\\
-0.659365634265378	0.550808457412839	-0.676819882311723\\
-0.604592497605471	0.606490147647145	-0.621946983750836\\
-0.55054846969073	0.651072972043645	-0.564630384875968\\
-0.499489541386082	0.699347844936272	-0.507702707992726\\
-0.446330041569933	0.7502738321523	-0.450930613005345\\
-0.396044907406805	0.798113391378133	-0.391029921300544\\
-0.338611297900659	0.849822383643951	-0.331618714582251\\
-0.280690737471354	0.894578984122785	-0.270568912008518\\
-0.224711941751689	0.93849644601338	-0.209683058849851\\
-0.16892685369019	0.986275482886221	-0.155018792153008\\
-0.111134990825546	1.02559974484507	-0.100499468719658\\
-0.0549752908328018	1.06320527674927	-0.0456769296444546\\
-0.000977872683983087	1.09666252849073	0.010302887012338\\
0.0557587964780432	1.13781354447212	0.0607750484519258\\
0.116110577061856	1.17545485565356	0.115959218816399\\
0.175691679666404	1.20992923955523	0.161901311504316\\
0.232748765770166	1.24716034135514	0.210486992358668\\
0.292881897898659	1.28045142232902	0.257209720815239\\
0.351400916583728	1.31226386929515	0.305560539142629\\
0.407759025047308	1.34674089736457	0.353242150936268\\
0.464362193982513	1.38289946352213	0.40354352753329\\
0.519806515232579	1.41766533333554	0.450756754805817\\
0.579791581474152	1.45298806998336	0.49982899465621\\
0.630330461225914	1.48939798469553	0.548791834620117\\
0.680207559994775	1.52433116639941	0.590702092131388\\
0.732210593375266	1.56916542552337	0.64101786961329\\
0.782830371440488	1.60933724902005	0.688040626190246\\
0.835222882756387	1.64714827145702	0.742395842277165\\
0.879167065106617	1.6908307056549	0.787836221186975\\
0.922554779812626	1.73442902138144	0.835343280017121\\
0.968229202375749	1.7800803062225	0.875578095160023\\
1.00468409432214	1.82122244587443	0.920233266083355\\
1.04954752099087	1.86385882139071	0.972889979690468\\
1.09424933934566	1.90572203463849	1.01571907640299\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998820335376772	0.238921318243581	-0.996969581059155\\
-0.937071634582295	0.295140179291052	-0.943756993473794\\
-0.876139596659584	0.344939806167525	-0.897342204977664\\
-0.813721266783148	0.397691538934039	-0.841597462365402\\
-0.748021699902443	0.445484609128519	-0.78301767507068\\
-0.685043459105533	0.499721975901537	-0.73103355466423\\
-0.618842846105844	0.547120151214652	-0.677477946235264\\
-0.546844142562826	0.587095564076127	-0.623561101067313\\
-0.46823195206458	0.632124148862021	-0.571199447699018\\
-0.395515238202973	0.675072970046032	-0.520880772337115\\
-0.319938529664889	0.713615139425768	-0.465927183386198\\
-0.243211956264313	0.752923796959993	-0.410387217377009\\
-0.168155245938329	0.790597964672429	-0.354645879879868\\
-0.0958117218807896	0.829815104746962	-0.301180641105088\\
-0.0259715780474841	0.860550878588039	-0.246873953464595\\
0.0421023788172709	0.904274596508869	-0.195717790601222\\
0.113715180511701	0.951859870071415	-0.141406863864737\\
0.184706948439921	0.997536369595875	-0.091462727889696\\
0.249250946848064	1.04057469957017	-0.0424766261122953\\
0.320079487574856	1.08890931768402	0.0106434234306132\\
0.392174896817315	1.13407108515269	0.0610073539818095\\
0.457136971874876	1.17454222116694	0.112058158005418\\
0.519428042632615	1.22245260767292	0.160549911540699\\
0.584663574066972	1.2627042345698	0.209544686831594\\
0.649822494004643	1.32118306801154	0.26012615385116\\
0.719907162719835	1.36934072698426	0.307409175359373\\
0.78338103065916	1.41597416906786	0.356188806277736\\
0.847678004201852	1.46567996380167	0.406173497391645\\
0.913221152014442	1.5151702694116	0.460843008360163\\
0.98030984083085	1.55695937707148	0.517205072955565\\
1.03952857790341	1.60332881896411	0.571317714147402\\
1.09798755174183	1.65011344344005	0.625106222583626\\
1.1643635454599	1.69280340409992	0.676078149923056\\
1.22877548910632	1.7465278474927	0.734725491744017\\
1.29305008212906	1.79291020122233	0.784666086452308\\
1.36131578464863	1.85129472235578	0.837823693033084\\
1.42229886754359	1.90412508397255	0.884608592598434\\
1.49063846924171	1.9581272450955	0.931869184869564\\
1.56626535556546	2.02545736600662	0.976794527451747\\
1.63564991973717	2.07397037829095	1.02263920234139\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998141641676941	0.240967974914197	-1.00104573129492\\
-0.940289965417701	0.296436333508483	-0.951756290257576\\
-0.880642106735884	0.346193713113848	-0.90194032523838\\
-0.823903869886611	0.394281991098614	-0.848688414968544\\
-0.774515055117073	0.44663042020815	-0.795615391257305\\
-0.718953555876818	0.493396837258269	-0.743592861836015\\
-0.663014760487011	0.540758853407822	-0.691942101793505\\
-0.604643703120425	0.584821925667062	-0.643936819934352\\
-0.551142793187199	0.635150151318448	-0.599578378844916\\
-0.493137791939963	0.678849867648144	-0.552117599593888\\
-0.438176982506915	0.724377433661882	-0.502596057358096\\
-0.381608546230655	0.766878362948332	-0.449712819452601\\
-0.324235174831834	0.806449695532166	-0.399555125349189\\
-0.264110604083804	0.850979232727021	-0.350140378946814\\
-0.206512661124915	0.894379517090073	-0.301081461622054\\
-0.154237726861326	0.941430839990925	-0.250857608285135\\
-0.10086694970637	0.98442856337781	-0.201758719189176\\
-0.0459965825642973	1.03030334795318	-0.152779607595599\\
0.0108273687164005	1.07162883151285	-0.108031767186483\\
0.0630459839546758	1.12172448432462	-0.0640373791277421\\
0.114140364546358	1.16516459074779	-0.0185712643445556\\
0.167483057058572	1.21027796183965	0.0260149100624995\\
0.22499017885151	1.26023140779112	0.0689347587561598\\
0.275815418455338	1.30780796524357	0.112388677324613\\
0.329024379692852	1.35324196944629	0.15361027360572\\
0.38405613968104	1.39732267347827	0.192652958101126\\
0.440666272778179	1.44568166461066	0.23004812488495\\
0.497406879657085	1.49283470924521	0.275313496475246\\
0.559461237584241	1.5377608107421	0.31895704973692\\
0.623380174570776	1.58877975853588	0.360598797189408\\
0.693562409807554	1.62522930427611	0.403593824844869\\
0.765342611122525	1.66695834452229	0.44944560983481\\
0.83752062084654	1.71001844620491	0.494724077995049\\
0.908406001396094	1.75106936413118	0.55064618493569\\
0.983922390329083	1.78547007538123	0.597413206791784\\
1.05826693551764	1.82043870407701	0.655931597015267\\
1.13113499572271	1.85605619904299	0.708403706593457\\
1.20619129348005	1.88540233292976	0.755280510916421\\
1.28143016981168	1.91792636176267	0.811799247013876\\
1.3578558127962	1.94481149689388	0.868215907014479\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999379532098069	0.241223723327276	-0.999920084408998\\
-0.93492165331174	0.295914305409757	-0.946124244297636\\
-0.874994082955451	0.343031763381411	-0.894850305142999\\
-0.809094593462341	0.385981203187363	-0.841311767072062\\
-0.750513715131491	0.435396407421481	-0.789834135005093\\
-0.687586902390309	0.480360499957345	-0.736112328938023\\
-0.632691069686544	0.526903928045293	-0.681665340098762\\
-0.577944258981679	0.572691468807821	-0.626757505663241\\
-0.525543804283991	0.618660045578255	-0.57429801599278\\
-0.473354545274657	0.664572066760024	-0.518335892726232\\
-0.416061773757111	0.71889625048144	-0.461207246992515\\
-0.357857832172204	0.765455440821941	-0.3978378972767\\
-0.302274939986316	0.816627044511738	-0.335877313033306\\
-0.247947521476374	0.862266087482545	-0.275042145613876\\
-0.199879405995406	0.904374457595352	-0.216176381583011\\
-0.156466604454471	0.945687096831013	-0.154985257768373\\
-0.112194634728078	0.992549864846286	-0.0905928258134019\\
-0.0691812259949483	1.03655867008954	-0.0319964039603638\\
-0.0231554325911002	1.07949726980244	0.0243611132704072\\
0.025900862016675	1.12645333379324	0.0791319056483098\\
0.0718501885869285	1.16993008852809	0.136942515132676\\
0.119671273213875	1.21654756500959	0.19367263401488\\
0.168020561329555	1.25850470482246	0.244341762240554\\
0.21802461144304	1.30164387328126	0.304327430250959\\
0.270951950541524	1.34508155835582	0.357294114281204\\
0.321030143896179	1.39422266287677	0.409521576158534\\
0.377994998122363	1.43741189245949	0.461461115991604\\
0.435859567248624	1.48389534083306	0.514845197059223\\
0.496265467782873	1.53040445464621	0.565186714389318\\
0.556299039976345	1.58255010062908	0.615363436602804\\
0.617047681951464	1.63552058297951	0.669227994220004\\
0.680907093515907	1.6872794052462	0.719695355352909\\
0.742044735390273	1.7413481484156	0.76984166661847\\
0.802018594842547	1.79214191244091	0.820403165860948\\
0.859282127973218	1.84274059100774	0.872457664819439\\
0.916853818852517	1.89879759749512	0.931304340332778\\
0.975616134558948	1.9593164400295	0.987942311220517\\
1.02881600198417	2.02219584921213	1.04481651384734\\
1.0832693049385	2.08176642178776	1.09728417561781\\
1.13277286916824	2.14841003268375	1.15596800117175\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999692310620872	0.239927674033235	-0.999472432615463\\
-0.933209819728707	0.294748472255955	-0.952261281905421\\
-0.868577711023995	0.335765656725296	-0.904340802739909\\
-0.799092069724105	0.377827820415651	-0.853678993657259\\
-0.727332144761213	0.422970624041353	-0.807275525685005\\
-0.655851728054118	0.473916580110526	-0.75888187800323\\
-0.587001768519097	0.520084917967592	-0.707430624155749\\
-0.515955211025173	0.567453846966708	-0.656195506366815\\
-0.446198405426685	0.612821995961846	-0.605449946997307\\
-0.373250218732531	0.65216923049297	-0.554816287316858\\
-0.299296176120974	0.690687677149231	-0.501713936178241\\
-0.223971979258598	0.729535119464636	-0.449265513717634\\
-0.152145543292195	0.762859695512808	-0.393640208907787\\
-0.077939023765532	0.792386590549032	-0.334102158390686\\
-0.00772147692959863	0.820768415406884	-0.276871959717681\\
0.0610432880036605	0.845364995915679	-0.214686061882883\\
0.129184138865217	0.869133626882791	-0.159136365829675\\
0.197104110175878	0.898505083067777	-0.105594134850437\\
0.263868304657298	0.92054046392094	-0.0480516806394047\\
0.333409676023692	0.947021412351271	0.00319140706745683\\
0.403062971142568	0.970883716135543	0.0584373869445038\\
0.475682004816493	0.995920020940746	0.11412895053286\\
0.5449443372319	1.01752848431982	0.163525375301499\\
0.610392438290691	1.03998945592692	0.216423960829373\\
0.674330360522012	1.06938989168373	0.271322847711803\\
0.738445814596909	1.09437680542196	0.328401356808452\\
0.801823353084034	1.11926185706369	0.381847195154675\\
0.864314845733103	1.14190470530954	0.438691398473727\\
0.920222809590428	1.16666620393811	0.485574912785679\\
0.977558104172646	1.19310145446199	0.534438156242062\\
1.03463157503337	1.21726284661055	0.580998946992507\\
1.08685230105948	1.23856160545643	0.627852252630681\\
1.13793081805297	1.2593147644309	0.677243817230983\\
1.19545577295665	1.27798699002787	0.728361159733363\\
1.24754004030227	1.30250091317863	0.776440145446456\\
1.30191549833444	1.31824391475217	0.821097606228413\\
1.3575995649498	1.34538921661929	0.86869134821583\\
1.40889647097055	1.37273800670513	0.914263774778509\\
1.46259078616865	1.39435947213133	0.958178684058967\\
1.5196290196583	1.41998842495514	0.99970630630871\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.0008872540537	0.241432926064298	-0.996633556315726\\
-0.937172206737194	0.303169074359908	-0.953146360197932\\
-0.877023053451693	0.345234437205845	-0.905475789191137\\
-0.811349230914318	0.393087850027326	-0.857675931327085\\
-0.748557536889076	0.43950763832727	-0.807468564276365\\
-0.690821605453801	0.49064589322845	-0.757118489027448\\
-0.631296132199868	0.538810205812094	-0.707828558577903\\
-0.571461507142488	0.585759839128613	-0.661269483166922\\
-0.513408007728163	0.6381450439303	-0.610789885088859\\
-0.455146235541629	0.688970344751322	-0.55923029660364\\
-0.401220864936343	0.745194904194207	-0.512607935279978\\
-0.342709330464797	0.798349645315461	-0.463116163216725\\
-0.282164833815141	0.856037033053808	-0.41532914635638\\
-0.222468242143816	0.917796548686238	-0.361975760192633\\
-0.165045956534996	0.981677973042248	-0.309740304771138\\
-0.108364342811272	1.04652973304131	-0.257534753134524\\
-0.0587552517817292	1.11217382389008	-0.206808854252477\\
-0.00200931185334325	1.17737973156386	-0.155243031753258\\
0.0562196644555416	1.24351072637553	-0.100664547768488\\
0.114940699105903	1.30766965566372	-0.0488840862162478\\
0.170919506281538	1.37229158082352	0.00453343930163976\\
0.226041481777202	1.44372672196622	0.0567280100758777\\
0.282446284908058	1.50867484967037	0.110299882473515\\
0.340083934919905	1.57077561906573	0.161165948861961\\
0.390407734954244	1.64136285524902	0.206372763361386\\
0.445499308068681	1.71892544365508	0.255642234222136\\
0.498051206182195	1.79675195542776	0.306691133636599\\
0.551553624648943	1.87939959894694	0.353772234579832\\
0.601596043468437	1.95851317361973	0.403985923034679\\
0.65806362583231	2.04401454564946	0.452116753343756\\
0.709241154377718	2.12176029890201	0.506249261000002\\
0.755720320081895	2.20270713280254	0.554394415598567\\
0.800217191516422	2.29846251561385	0.602512599047508\\
0.852456529453143	2.37994727284175	0.654591488133874\\
0.894773629436084	2.45194429646527	0.712713921456089\\
0.940881650942463	2.5302859323334	0.758885602116381\\
0.985561789341494	2.60697507286057	0.807825988608978\\
1.02382142933863	2.67772575072283	0.853294196716483\\
1.06953942346816	2.75370739644224	0.901880082748034\\
1.12365698166703	2.83573277421499	0.944352229336189\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00082743567633	0.238885170251025	-0.996206865027175\\
-0.940817417922833	0.296881056563082	-0.948557069637876\\
-0.881878366995346	0.35101660361673	-0.897637455255167\\
-0.819402456815038	0.400725296794156	-0.842970874700834\\
-0.758599621810355	0.455218953359551	-0.782301494425766\\
-0.698250709671254	0.516697996269605	-0.724683641260743\\
-0.642195280607129	0.574935395397737	-0.660382756763835\\
-0.591977079946194	0.635209516502012	-0.596605906885547\\
-0.540601864243441	0.701893624195876	-0.534844301705328\\
-0.48334891784124	0.764034702508068	-0.471390740652786\\
-0.429295032459792	0.827783704820473	-0.407844601893901\\
-0.373027477484754	0.899178055716306	-0.347857776586655\\
-0.319733916661838	0.966387419444043	-0.285557069314635\\
-0.268251566022367	1.02707986125062	-0.22193314363696\\
-0.221575564879888	1.09072701171127	-0.160646300653345\\
-0.167831926242652	1.14869201584876	-0.0979971288513163\\
-0.114306874366952	1.21188288584621	-0.039256381790911\\
-0.0568484378683423	1.27135149170009	0.0208765077156277\\
-0.00269477784702398	1.33240485248897	0.0767110264607232\\
0.0553665454390656	1.39401571314772	0.130330605519855\\
0.102977587419805	1.44898789224728	0.183197551203754\\
0.15567900311223	1.50842486891107	0.235722722361896\\
0.207823061891058	1.56571513228968	0.28555200706942\\
0.255135614146583	1.61638481097362	0.337960088325288\\
0.304790259240445	1.67414838607076	0.384614022381312\\
0.355903086354957	1.73159358461473	0.439592646541742\\
0.406634016269651	1.7868743930437	0.491809721004599\\
0.460914263153398	1.8343807011135	0.543374422784016\\
0.511542861930725	1.88494950697514	0.592598079622089\\
0.565263290721416	1.93961102731021	0.646332373128015\\
0.616981555691952	1.99077201622695	0.702819101503462\\
0.671197567301063	2.04015319134609	0.760803284275124\\
0.726075240116637	2.10650310794462	0.81718418991772\\
0.783255221024317	2.16623585687345	0.865259934274922\\
0.853000676037957	2.22763775186827	0.917531008264735\\
0.913478824212786	2.29682918743265	0.966696296980674\\
0.969452970558019	2.36517560733474	1.02015598397779\\
1.02946830395265	2.4281140161147	1.0748752797848\\
1.09250649588298	2.49312186411354	1.13649164958425\\
1.14801020465013	2.55986789988781	1.19054503258881\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00008317066648	0.242834635470484	-0.999899041095014\\
-0.939346175301803	0.296314821407122	-0.949410557679027\\
-0.880099002568571	0.343752438190296	-0.906356273050507\\
-0.824651746555369	0.391426348091208	-0.859385172836208\\
-0.771442787411484	0.437491768170075	-0.813425413378958\\
-0.714945218902297	0.485506554465226	-0.766641089437531\\
-0.662834128060215	0.534399092098705	-0.716416013327529\\
-0.608251504078102	0.584689137110478	-0.662707721076069\\
-0.554193738412495	0.631881020127409	-0.610628535553922\\
-0.500856522659415	0.673592449757168	-0.557450907962817\\
-0.446866294993415	0.723393243569409	-0.508738522550848\\
-0.392892391536904	0.770496439283146	-0.464306520964812\\
-0.333205082199676	0.82227573006045	-0.41442530380006\\
-0.276525099730795	0.873340341902548	-0.362061970649051\\
-0.223084849807473	0.92940436471091	-0.311476610522187\\
-0.168194829036812	0.98411040994248	-0.256843284268853\\
-0.107695320415129	1.04428466753511	-0.203963361014592\\
-0.0511222109411478	1.1030549491784	-0.157362670295097\\
0.00767296756030962	1.15454670598118	-0.108365094141501\\
0.0652733523734312	1.20667399690555	-0.0580264467290626\\
0.124304356030193	1.25576257928068	-0.00255882061443522\\
0.184480909991661	1.30970698496415	0.0576169470209865\\
0.248308933665813	1.35810446897833	0.119255205753347\\
0.312381494076611	1.41291239064518	0.184709998448736\\
0.375793362004162	1.45854951669542	0.249077833742865\\
0.436653862834686	1.50533424380876	0.309392810111666\\
0.502277859071436	1.55091135955666	0.373128960529219\\
0.571816446990701	1.60072996369009	0.437708227074967\\
0.640634339259514	1.64180824132921	0.503741223253932\\
0.702863475564713	1.6938980380019	0.569547105290018\\
0.767703523237002	1.74477144201522	0.640765705504502\\
0.838987846409415	1.80057861810469	0.716908063729262\\
0.905544002759294	1.8570284413532	0.787790908144922\\
0.975474719821674	1.91674420466195	0.86644919650893\\
1.04026145249735	1.96817372844567	0.940443625728088\\
1.10619586999997	2.02246670642592	1.00891639137243\\
1.16765686988811	2.06939376269636	1.07931471959946\\
1.23573994474283	2.12443111378121	1.14497919445465\\
1.30158775659136	2.17076864519567	1.20471193671836\\
1.3671983888644	2.21714675790961	1.25959274581551\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00020775695172	0.241752468326017	-0.998207411825569\\
-0.935412660457032	0.293829513775434	-0.945800936610767\\
-0.871239674859816	0.336606502333263	-0.896456181201684\\
-0.808541806413232	0.383791459409964	-0.843740034979626\\
-0.747295722993108	0.428188110837707	-0.787160495564368\\
-0.685957354453649	0.471724817867047	-0.728515526449395\\
-0.624326120910088	0.517746242483975	-0.671694126636045\\
-0.565079026375145	0.5647115272411	-0.616493908649543\\
-0.506665091639353	0.612639196436584	-0.562975793784745\\
-0.450662943200388	0.666281371968875	-0.514734149996427\\
-0.390564184894974	0.713579958084468	-0.4687636267017\\
-0.332438751806191	0.765269474638649	-0.424816335969826\\
-0.271536519170302	0.817951094590046	-0.383183921346484\\
-0.209292031525921	0.870531366154017	-0.339336111957847\\
-0.146875008068577	0.920883730011517	-0.292182145126404\\
-0.0830619297188933	0.967117923257754	-0.24622403560658\\
-0.0190025917659913	1.01543061657803	-0.197558077179422\\
0.0463146252773338	1.0665823738543	-0.147657825204193\\
0.107590326974069	1.11861402453776	-0.0985198091543596\\
0.172196688471171	1.17227969641039	-0.05130621956541\\
0.237663158652785	1.22669549039476	-0.00404275707666333\\
0.307380372152273	1.28342599295708	0.0408935012984167\\
0.3796894396644	1.33444743074769	0.0868261666490223\\
0.454845401889092	1.38895559911942	0.132489653079162\\
0.531622067764118	1.44535519983395	0.176263967132718\\
0.601800283013693	1.49885816783364	0.222326432057736\\
0.676908940749516	1.55113522791756	0.268860502759302\\
0.748302461751008	1.60708930892292	0.312574123220425\\
0.817069811649118	1.65967719847086	0.356537006104763\\
0.886239338921974	1.71254464257122	0.407946342020007\\
0.957336911433076	1.75698937713088	0.451327092603668\\
1.030913206791	1.79956243382572	0.495754502256299\\
1.1073219333597	1.8619595214226	0.549421259363623\\
1.18463833455541	1.90987749375411	0.603452648070007\\
1.25684062884056	1.96240220296043	0.65338077251216\\
1.32739545930923	2.02083954535988	0.703923561802601\\
1.39664955208251	2.07153467299757	0.755171261002132\\
1.4642169515537	2.13032785613182	0.807560154139646\\
1.54029054503522	2.18966417491797	0.862873472463479\\
1.60160131632678	2.23871556754639	0.910406606830474\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997497770797953	0.241338622250135	-0.997689821932872\\
-0.935305408722999	0.297768099946843	-0.949867904844403\\
-0.875335708765558	0.342110242819317	-0.901852183933097\\
-0.815849241962318	0.393494416689344	-0.8581953643271\\
-0.757742463920341	0.434221336330512	-0.814672587605776\\
-0.699074320449531	0.477099486565259	-0.772991064002535\\
-0.640336141124177	0.512716515695571	-0.727457110946281\\
-0.575840145144716	0.548120828302769	-0.681013638705464\\
-0.518686074606721	0.587661264146064	-0.632144825901329\\
-0.460136356239959	0.622039593487913	-0.585035216907204\\
-0.405973766081343	0.659569930648631	-0.535321942193913\\
-0.351197114697678	0.69908797156257	-0.485978198919754\\
-0.296672365262517	0.734122246153381	-0.438880075596537\\
-0.242053822006569	0.765820407948098	-0.388312838826704\\
-0.186553322901428	0.797359101361913	-0.337177588026869\\
-0.132205049122026	0.834877891222277	-0.287265621766334\\
-0.0820790894718472	0.872534512104874	-0.236114342486902\\
-0.0360199003929473	0.902788813015577	-0.184077630742093\\
0.014504698540903	0.942014452743439	-0.126699027959907\\
0.0580565922504901	0.97575901111624	-0.0709197961710588\\
0.108704760710776	1.01065614913078	-0.0158575813236208\\
0.162441128017141	1.04281582328382	0.0350139541656995\\
0.211868799919124	1.07835584954129	0.0895762618026884\\
0.267614654424767	1.11508846064413	0.145417667938227\\
0.321295401555564	1.14590299024124	0.196990341840391\\
0.376017110984062	1.17830678585824	0.251811820578513\\
0.424864898874264	1.21009749242554	0.306463046234224\\
0.474134593098504	1.24102549811481	0.36185673587438\\
0.526208333874866	1.27205964880837	0.416768847238454\\
0.575730902605529	1.3043520829736	0.468890479567695\\
0.63048359626773	1.34259998022593	0.52301232229123\\
0.681910995817487	1.37421245082713	0.579085006821283\\
0.733135676836192	1.40693314636095	0.636641263658516\\
0.776524622534419	1.44108002332212	0.686512503131546\\
0.8293758470028	1.47087445357308	0.75200471300118\\
0.878038599561469	1.49615492704504	0.809110371381686\\
0.929546584371171	1.5283081672303	0.870945893273693\\
0.979460470974572	1.56142999572212	0.933079533889153\\
1.0321669016887	1.58884239567125	0.998263790334524\\
1.08094257537962	1.62718464447431	1.05514064333366\\
};
\label{pgf:realized-trajectories}

==> figures/results/scenario-rand-traj.tex <==
\addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999097315186919	0.240119845720588	-0.998329213122516\\
-0.938412095353681	0.295440126566335	-0.949231614583555\\
-0.878512791615236	0.340806297596779	-0.897664364211227\\
-0.816611331132436	0.388391284107827	-0.846652518350923\\
-0.756264247299061	0.430953857706298	-0.788542795559308\\
-0.693346798677602	0.477179850170322	-0.732806726098525\\
-0.633599009497513	0.525691123326287	-0.676768599237468\\
-0.577290825638977	0.574995702674751	-0.62150517088954\\
-0.522309512888715	0.624423455192063	-0.563569290256212\\
-0.465574742731491	0.673509682453996	-0.505666770494669\\
-0.408892490796794	0.719829021405084	-0.4466054956301\\
-0.352503658971736	0.766191572476398	-0.387410026197205\\
-0.297805366356346	0.812078150921203	-0.32558236930593\\
-0.243030960615153	0.85623754604451	-0.266362897759654\\
-0.193520760069313	0.904286350006819	-0.206959562961663\\
-0.141157391253395	0.953475887168867	-0.147201815584372\\
-0.0907455166952493	1.00139735951368	-0.0872885080405619\\
-0.0425576690079486	1.04778289551989	-0.0244577705657749\\
0.00282492915169044	1.09781824649243	0.0438777373380001\\
0.0565737955837675	1.15187541298268	0.106313216204646\\
0.10797019440556	1.20087217888338	0.172377656132818\\
0.161325119672917	1.25350548595618	0.237191095676087\\
0.21515978458401	1.31753096196156	0.300213086496812\\
0.271392805977068	1.37424111359057	0.362520098681723\\
0.33201801548201	1.43988655879183	0.427342396078996\\
0.391186315944183	1.50307631027328	0.495517768370902\\
0.445452114069583	1.56734539496914	0.566020288498512\\
0.506908482655378	1.63732088245499	0.634263296387283\\
0.549331935555102	1.6982240836136	0.699553937681523\\
0.604175723754949	1.76574419525826	0.765610972521112\\
0.659242072905705	1.82706975910274	0.835674754685076\\
0.713341541594064	1.89135293476561	0.902719944809226\\
0.770566008293583	1.94223570293987	0.964915878680431\\
0.827908195113713	1.99664706311779	1.02845572132607\\
0.890029784434075	2.04669553968328	1.09704364513822\\
0.955033659834317	2.09854691738488	1.16135988571675\\
1.01606760509757	2.14580206338748	1.21349562315363\\
1.07817559373134	2.21111847854855	1.27513029909803\\
1.1385821153485	2.26186625269289	1.32688609329567\\
1.20282493344029	2.32082152819043	1.39144809294066\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999667657862896	0.238173218303069	-0.997920668690405\\
-0.935784903697031	0.294398781427412	-0.949305133532812\\
-0.871210886795331	0.339217052961964	-0.902298536164682\\
-0.808200323443767	0.381929987661314	-0.849842262277774\\
-0.745813121953649	0.427107037955903	-0.798055905865515\\
-0.685129650788503	0.471942116021726	-0.745323886694096\\
-0.625304784298019	0.513570237308726	-0.693036976465682\\
-0.561810557637919	0.5554630076023	-0.643233500134224\\
-0.497163268612965	0.602609195051863	-0.589181958819995\\
-0.432870421577076	0.647717260435037	-0.541959806017581\\
-0.364732968296831	0.69175127298335	-0.492664363513962\\
-0.293457473207169	0.737765842164415	-0.443461715072101\\
-0.221934597662915	0.781366467477909	-0.396141012609215\\
-0.151103072946458	0.829666097750292	-0.352774052167906\\
-0.079247201751869	0.875330162963369	-0.306992134685458\\
-0.0065383115673814	0.920822809406805	-0.261741840358181\\
0.0644181911695005	0.969729747414371	-0.222088542729676\\
0.133873375463614	1.01213439957069	-0.174695113950791\\
0.211492204651671	1.05545602117726	-0.134289503229383\\
0.285919287914461	1.09413121789221	-0.0965963536127306\\
0.360094750580293	1.141824701382	-0.0564671814732959\\
0.437112530752416	1.18201692282175	-0.0158825087122953\\
0.511901831117608	1.22021870252017	0.0238666390745128\\
0.589930337717635	1.26811685005856	0.0683396505306249\\
0.668505584305252	1.31221622217147	0.102603112503561\\
0.739820170185275	1.35102097343292	0.137093133287093\\
0.817936143758984	1.39689732988944	0.171108615644905\\
0.89195169614011	1.43951244671421	0.204191235630114\\
0.968833705356383	1.47991378231493	0.227407522908481\\
1.04335471652829	1.53088700243087	0.254942466392028\\
1.11826650658343	1.57120971867254	0.276889956690151\\
1.19464354405239	1.61076484245047	0.300673516767108\\
1.272374741656	1.64905852456528	0.32068422032466\\
1.35515506597905	1.68737253394039	0.34225510062944\\
1.43732706164774	1.71610694613945	0.361396622647346\\
1.52164483412661	1.74963531223171	0.381795171980213\\
1.59752818231351	1.7863372178692	0.393402774599737\\
1.68048549684154	1.82243685751266	0.411131597581458\\
1.76939850653048	1.84988554472865	0.429142328458342\\
1.85293455268544	1.88858911443502	0.447308380711106\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999924837645672	0.241729177915146	-0.997478542776999\\
-0.937681164454054	0.292192750777386	-0.946703338527673\\
-0.878568289169036	0.343650225908645	-0.905308451817009\\
-0.818919711852958	0.394420933981825	-0.860678227362683\\
-0.754598519921171	0.440324111021316	-0.816337589535641\\
-0.689433670270014	0.489478495783867	-0.771326094999197\\
-0.626931673928238	0.534328670500652	-0.724755812370957\\
-0.566270433800586	0.583945836072204	-0.673426835276538\\
-0.5027953539105	0.633129182445539	-0.617329134314982\\
-0.443648624447506	0.681483771291245	-0.557108680896433\\
-0.381459744230073	0.724035331737841	-0.500230688911273\\
-0.321631027984259	0.76620000505117	-0.445800818212269\\
-0.259610519426787	0.816590856645716	-0.389021038288267\\
-0.196360582528207	0.863726388066227	-0.329800722523275\\
-0.138093303928964	0.911039500425341	-0.26642811127088\\
-0.0803888829457074	0.964797150196262	-0.208107030910868\\
-0.0211098465411437	1.01986537164632	-0.14941524298466\\
0.0424767654185755	1.0735123437897	-0.0850116423601921\\
0.102890399436442	1.12647594020454	-0.0267406652018197\\
0.1638152334735	1.17812365106589	0.0335642712888511\\
0.217369303309985	1.22710835879745	0.0923958316330016\\
0.273212289080171	1.2769121142545	0.151282815622763\\
0.326735137756616	1.32810755374869	0.208531645226444\\
0.37725296408845	1.37561128013418	0.266859890366238\\
0.429410292599422	1.42541532145426	0.328279951489699\\
0.481162847280057	1.47170369969262	0.389705496781714\\
0.52932906959137	1.52164030506356	0.449005272619135\\
0.574000185312082	1.56991382284694	0.505705798064868\\
0.619548005893587	1.60567741835183	0.55876119786146\\
0.662750942195111	1.64296270893025	0.615527738407152\\
0.707841582658699	1.68811455830587	0.672353114429739\\
0.750445765376639	1.73566971057371	0.730152122611179\\
0.796494069861394	1.78355092966546	0.786834106374463\\
0.839344706221885	1.83297375351583	0.850164601489153\\
0.87931395490178	1.89326684830717	0.90916643430478\\
0.915777648722567	1.94770717605551	0.959944434582392\\
0.949782110304803	1.99867803352606	1.02079645971072\\
0.983925357006963	2.05455423479001	1.08344051779624\\
1.01075553830751	2.10281458745752	1.13305205104931\\
1.04379994530776	2.15211816265308	1.1907194622744\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999478013440514	0.239121487946158	-0.999664169531621\\
-0.937919876202622	0.300262643840738	-0.949440908815235\\
-0.872945467509057	0.340046629608734	-0.896844670300923\\
-0.804632616432495	0.391936590717664	-0.839258657082587\\
-0.742691908422451	0.442684134614955	-0.781659198657779\\
-0.673202502243283	0.495630071255598	-0.719673845258915\\
-0.608168576948165	0.54780125920894	-0.651868795849366\\
-0.544810218600067	0.607407133032499	-0.579597294613321\\
-0.487314311397158	0.665107114801059	-0.509448534652274\\
-0.432317215081443	0.720341586380996	-0.439604476220697\\
-0.376675469530773	0.776095232950088	-0.369240626938829\\
-0.327117596602069	0.838461179420792	-0.302687526082584\\
-0.270657245407119	0.893645480317961	-0.2334230398002\\
-0.217031304029397	0.951272579562135	-0.16979722191176\\
-0.16313207559679	1.0019400607661	-0.101346322294367\\
-0.110643155564647	1.0579217936251	-0.032360869655571\\
-0.0571374588816951	1.11765721426541	0.0321714731982948\\
-0.00268375698680666	1.17624748971723	0.0957200692271709\\
0.0600950417554353	1.23908422052683	0.155574377739027\\
0.116628584544364	1.29854070254098	0.221616645435937\\
0.174352152453095	1.35911963201167	0.282043748453936\\
0.226881686004214	1.41883910376421	0.342040959781102\\
0.278859926509455	1.47489728216788	0.409194268661487\\
0.338077194537511	1.53169947861436	0.478150815151479\\
0.389425510186719	1.59133650957836	0.54159794166849\\
0.440920309230101	1.64134669664039	0.614851913131274\\
0.500769228324601	1.69736098010417	0.684263666035433\\
0.557427566640788	1.74929691731827	0.757367514396136\\
0.620095323988923	1.80111935439877	0.825193497402672\\
0.679861845802182	1.8504353721842	0.888987578365886\\
0.749867191447688	1.9049557385142	0.959037787026043\\
0.816187231743557	1.95461102350735	1.02605016818157\\
0.882605878828086	2.01233926787184	1.09987866918675\\
0.945865302569833	2.06557461300503	1.16485708437803\\
1.0054864236239	2.11745255540829	1.24129861209178\\
1.07355599734616	2.17706887679202	1.30473662224727\\
1.14074214222072	2.22275149504989	1.37680807708408\\
1.21409580086994	2.27917271594911	1.44486037917327\\
1.28265929370191	2.33709720180578	1.51601873073528\\
1.35064422845006	2.39357851378861	1.58384642030979\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998394363748421	0.241391636925528	-0.999676549414364\\
-0.936918381121223	0.298669992849192	-0.952094821158014\\
-0.875767908208196	0.343758352253392	-0.902905729901582\\
-0.815197212569857	0.392635576534526	-0.852626760192742\\
-0.753561249753385	0.440544606832965	-0.804526772703398\\
-0.688172570774846	0.490685192407003	-0.75064146760025\\
-0.624898115728265	0.546176192777976	-0.699077403445479\\
-0.561099281407153	0.602664714348731	-0.647079927584265\\
-0.49883757961662	0.65759771439262	-0.596232810753198\\
-0.435796183985938	0.710038888086768	-0.545440631051465\\
-0.373558648862864	0.769846214817057	-0.498040297105428\\
-0.314811782972639	0.828358498517937	-0.449357447921745\\
-0.2524024449055	0.896486465279975	-0.400265727976023\\
-0.192428253892741	0.962132014710789	-0.352285981124797\\
-0.13614184645904	1.0347170348175	-0.302497530760353\\
-0.0789206302516105	1.10277525703474	-0.248021472590597\\
-0.0251768291052274	1.17080059360707	-0.194291800797375\\
0.0293264326133252	1.2338702608214	-0.139257610005553\\
0.0861150100645423	1.30144023970158	-0.0886725710442827\\
0.143442980144328	1.36360002529055	-0.0369989662238396\\
0.201833597136823	1.43654387106327	0.0139565168372836\\
0.264952058314463	1.49954728847255	0.0605763557484886\\
0.327707811149283	1.56599261571286	0.110653745496687\\
0.394652125690023	1.63494296894629	0.160483867893581\\
0.452484459751574	1.70202312042417	0.210802665712741\\
0.5188420244303	1.76826251934115	0.265571934717872\\
0.583542550314195	1.83009966842947	0.317526540822369\\
0.652423235208146	1.89615201453503	0.371432798691608\\
0.722234329351696	1.95296742904529	0.427563973234104\\
0.797316877094472	2.00265708470708	0.483030450142666\\
0.872521777413502	2.06269868321607	0.544082891500222\\
0.942497800152492	2.10832357916145	0.597794893697672\\
1.02164341774071	2.16643438555882	0.659641741117754\\
1.09658968206325	2.22547782002623	0.722617067153515\\
1.16500599235602	2.28256003924498	0.778822768177995\\
1.23073515842758	2.33094914084345	0.832729757842996\\
1.30930344784289	2.38209429114025	0.887390751044605\\
1.38102199640084	2.43537171679772	0.947746989953797\\
1.45358138892782	2.49672284031577	1.01248982293028\\
1.52283257003745	2.54991729243403	1.0745339534392\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999206536821372	0.240614747710416	-0.999073765700739\\
-0.935747572771599	0.302554105470016	-0.949879809824215\\
-0.870085126440494	0.346651400973685	-0.898353459256663\\
-0.801329617155861	0.391252537491979	-0.844179580165398\\
-0.727861053855633	0.437286842337528	-0.793252966531727\\
-0.659903423554284	0.481716265764999	-0.742017905787137\\
-0.588749767361451	0.526441936775682	-0.687609600606862\\
-0.521788163477617	0.569496176155087	-0.635303353428615\\
-0.452161445437019	0.612263906426604	-0.583944864080208\\
-0.384968777677234	0.653505830051902	-0.53273794985631\\
-0.319373798657001	0.699595877740737	-0.480702393197372\\
-0.25002209192796	0.745477200657465	-0.426650616009033\\
-0.183112722215193	0.790983304225942	-0.367161808439276\\
-0.116039073883759	0.832499824607219	-0.305981387013783\\
-0.0491504999613637	0.872769645838886	-0.239981629032361\\
0.0134816638648992	0.917597551479742	-0.178202779981601\\
0.0776509297510142	0.956300051644895	-0.121771618324796\\
0.14816734953278	1.00064341847066	-0.0626745455673806\\
0.209082679261966	1.03734764337466	-0.00566020908517983\\
0.270636163818125	1.08074926264287	0.0485983283630865\\
0.335290536577594	1.11599847599121	0.111213780993127\\
0.398364715998242	1.15735503127916	0.170549149837201\\
0.462491158506485	1.19526592435404	0.228020511597368\\
0.526985046473297	1.23750385738186	0.281181029826116\\
0.595398138508177	1.28667294923754	0.340404343741137\\
0.654031403299382	1.33332692039148	0.400327171479644\\
0.715529531168409	1.38070372121129	0.464413802530454\\
0.774004358053077	1.42673058628537	0.532988378815541\\
0.832772151192636	1.46705069051013	0.599592577059147\\
0.888441175422733	1.51648837018956	0.662001696238218\\
0.946164642931846	1.56144889657937	0.72553379100922\\
1.00727868284173	1.61147515367677	0.792025434252592\\
1.0605874770109	1.66222244787825	0.852979107012315\\
1.11579267058985	1.71036936269883	0.913129270544734\\
1.17362794424683	1.7652853772959	0.985685724399741\\
1.23473228422935	1.81102251786995	1.05801304258326\\
1.29133062734567	1.86213339013939	1.12443621282147\\
1.35060711126922	1.92355931891312	1.19781805762717\\
1.4072385425516	1.9799713390525	1.26482317833978\\
1.4677627386464	2.03973471946858	1.33607070297014\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997883052500354	0.239562788719727	-0.999762184395189\\
-0.940996731810911	0.299202210121269	-0.948236377052586\\
-0.87911351281499	0.346255871198857	-0.898271486084\\
-0.823675025519549	0.389823822937065	-0.838610405547637\\
-0.769904405349007	0.434968934088193	-0.780165200632715\\
-0.712807781097405	0.474518048507076	-0.71472077338568\\
-0.65255664237385	0.520020696850162	-0.652418996932862\\
-0.595516806784177	0.558357933009645	-0.585080714163673\\
-0.538107912019687	0.602900647134081	-0.527400225730435\\
-0.483908647992432	0.644795766482449	-0.470550629464525\\
-0.43519436620072	0.690958385027276	-0.419232662240288\\
-0.382523690858809	0.735316388859158	-0.362577962272532\\
-0.329902162460523	0.776602583521377	-0.306884233448779\\
-0.278082033030916	0.828359581808442	-0.249840917333089\\
-0.225079816712181	0.876241512989808	-0.19531162091268\\
-0.170900832214055	0.925176847067152	-0.144054855766131\\
-0.116742834690869	0.973018330820666	-0.0893300328887857\\
-0.0624394644136377	1.02153583572487	-0.0448568270436764\\
-0.00577332859339685	1.07044479374776	-0.000920093897412682\\
0.0553641530800267	1.12488706094108	0.0436711281739225\\
0.114230016053197	1.17850102451915	0.0856520695225139\\
0.176789081501078	1.22591104014739	0.125805264868109\\
0.235512507891229	1.28004758400266	0.167331607676494\\
0.295535859530024	1.32939277352212	0.209155733249646\\
0.353722194315284	1.38011443215806	0.249022341216393\\
0.414532535755917	1.43675919406431	0.287667774705727\\
0.479258626095354	1.49600354249477	0.329848877583506\\
0.53173124446456	1.55555084735801	0.369697097335034\\
0.592932355954638	1.60842797308848	0.40975237770025\\
0.655115745090827	1.66474625526034	0.444502588779189\\
0.715754777221152	1.72403338974776	0.483427225629467\\
0.781599442546714	1.77381994572981	0.519613707393719\\
0.838067541498961	1.82717185638151	0.554225113916129\\
0.896449291980583	1.88818802403999	0.595879865356262\\
0.950550526056233	1.94171452484885	0.637873644316729\\
1.00895588826109	1.98508109395879	0.666801709341455\\
1.07027089243773	2.03911541539847	0.697469444289449\\
1.13282803001197	2.09728817885692	0.735774512405907\\
1.20244497662939	2.14622201057137	0.768879084125373\\
1.26927320717982	2.19726941539339	0.796044395505939\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00063716616188	0.241454311329808	-0.998645583687718\\
-0.937205208924317	0.301802541380557	-0.952111243642743\\
-0.876642622141368	0.34868600566378	-0.898622993834135\\
-0.819781338820658	0.395331527475424	-0.847474210687307\\
-0.758410314173534	0.444448998456875	-0.797983044158325\\
-0.693252783818156	0.497173217701488	-0.749053419622195\\
-0.629842025464283	0.550715637495785	-0.701412945984744\\
-0.566563601183096	0.60211363522896	-0.649075231225138\\
-0.506677778174417	0.657528260049903	-0.597745300773904\\
-0.438572139081411	0.717734841290323	-0.546013837285958\\
-0.372168895391132	0.777188744693852	-0.492202320471858\\
-0.315253685667198	0.838041290093364	-0.439557757902515\\
-0.251982770072643	0.897644255227291	-0.389011336626355\\
-0.192999006836236	0.960516347810662	-0.340087475761595\\
-0.136795947951068	1.02179893723344	-0.296563342468607\\
-0.0812706194522889	1.08396767647464	-0.248736117013248\\
-0.019614308991939	1.15097630173867	-0.20135460959152\\
0.0417152550813636	1.20744694247774	-0.154055536670709\\
0.10067181800372	1.26969969681178	-0.111070634989086\\
0.157637409496742	1.33124632079093	-0.0681202175718269\\
0.212813424725048	1.39292093026006	-0.020604002537148\\
0.272804998892333	1.45274837527847	0.0261000654517899\\
0.329804275226962	1.51344214336638	0.0676143578808853\\
0.387463218245537	1.57707583713732	0.118925726664259\\
0.446315174987434	1.63949739106265	0.165910214173213\\
0.5064195008976	1.7003305700312	0.215719432735994\\
0.560510198525291	1.75796494449459	0.260280536278802\\
0.623292017097367	1.825073278648	0.309005428639286\\
0.681940798166191	1.89490853929142	0.351218557850494\\
0.735341556594547	1.96304288399763	0.400036837865433\\
0.787907995854191	2.02429818414479	0.45033159091882\\
0.839314956909585	2.09842254323848	0.498438832575956\\
0.889821271244156	2.15752778842198	0.54592261509251\\
0.945814327792981	2.21859733023748	0.599545551758071\\
0.998989254242033	2.29081859034814	0.65084179676585\\
1.0555744088369	2.35574590616082	0.707343019389085\\
1.10345036676242	2.42200679028767	0.75968714801057\\
1.15266204462236	2.48423228126415	0.810776648317614\\
1.20538345445542	2.56802674263579	0.859657922911382\\
1.25750965581708	2.6253702260006	0.914616958698115\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999761700001014	0.239403006681903	-1.00064917212024\\
-0.937083741657319	0.294373445482623	-0.950469718385001\\
-0.866498553188442	0.339414873676002	-0.902809632387336\\
-0.795910058453806	0.382635376069131	-0.855747809311152\\
-0.722870800432642	0.425582219247966	-0.817688634859142\\
-0.650288491168251	0.468951313780107	-0.767575540394902\\
-0.57731033225852	0.514846285250778	-0.723355474033801\\
-0.509280094747592	0.562004399035181	-0.682855542108367\\
-0.443350252481358	0.615311835089838	-0.641896614799916\\
-0.36974734708259	0.668287915692574	-0.601156746642196\\
-0.297977393833331	0.722467178519768	-0.558465022701712\\
-0.222637099954328	0.771493790058387	-0.511730091595466\\
-0.14733763734938	0.822020443010629	-0.474378458458396\\
-0.0695166124726907	0.87151120941725	-0.431700718223935\\
0.00557842257860166	0.918921857558559	-0.388990247379048\\
0.0786352692641716	0.966885612175444	-0.346295891777934\\
0.151804010102404	1.01138556058554	-0.305464995906099\\
0.229184125424188	1.0587036306456	-0.264266006828897\\
0.303815765674651	1.10430062535515	-0.224765862907762\\
0.373161398829609	1.1514467749324	-0.185326287399925\\
0.449074088647261	1.19623366026015	-0.147777091255457\\
0.523856329732424	1.2401467952344	-0.109307611772504\\
0.597050856067149	1.28166219814115	-0.0733329690362184\\
0.666429531420284	1.34028457446826	-0.0357997775499501\\
0.734325524569692	1.39224101652019	0.00773283710159763\\
0.797214043380172	1.44181150257172	0.0432169956484051\\
0.860060750666171	1.48836632867528	0.0800071987863419\\
0.931424530450094	1.53670570482633	0.121163547677733\\
1.00062948743957	1.58978171720524	0.164634962687663\\
1.06316780852666	1.63763103683876	0.210132750385208\\
1.14239457049625	1.68275328595518	0.253975943840862\\
1.21261184245252	1.7298573092557	0.289613858523382\\
1.2852054776753	1.77838257977673	0.328176939380943\\
1.35716420480542	1.82792492289509	0.367898821959726\\
1.43219241032717	1.8799483647952	0.408911875974675\\
1.50751959665862	1.91701301547635	0.451607809764857\\
1.57498585601223	1.95862414773015	0.49433054244464\\
1.65492450528847	2.00299315142748	0.535073312125774\\
1.72552426370735	2.0446060887609	0.588618345274859\\
1.80027746548308	2.09282137366448	0.638922438455971\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996557484340456	0.238127046917851	-1.00033070407717\\
-0.93513036312295	0.294731733763121	-0.949236022945345\\
-0.872248630463624	0.33502965491585	-0.902049049719279\\
-0.811783366682228	0.373738005004437	-0.850490665650075\\
-0.743483424008749	0.420488362023471	-0.802506016003737\\
-0.678178150151024	0.464440157062153	-0.754900619054351\\
-0.613837722533753	0.505346708182796	-0.703550884169227\\
-0.550773095256114	0.544149676926005	-0.654597133463295\\
-0.484783111725279	0.576553565383625	-0.601380901785099\\
-0.419891026595235	0.602767477244866	-0.549539256249417\\
-0.355936053713014	0.628793672874905	-0.491666868401052\\
-0.287871815613709	0.657796338689459	-0.433591164827056\\
-0.223142450241228	0.687876582257511	-0.37692982574188\\
-0.1576564849622	0.716018257216614	-0.320710851529268\\
-0.0902147955503067	0.747648995606423	-0.260003452656784\\
-0.020992257203037	0.782254675672127	-0.202098856176548\\
0.0447952876140054	0.816035904893276	-0.139867454421879\\
0.107240191087314	0.845079539501693	-0.0830441012464023\\
0.166325622747975	0.878813853349971	-0.0204600605168311\\
0.227368626549095	0.913951924739406	0.0382483035671166\\
0.292686560664903	0.948482884708528	0.0986522426200731\\
0.355256906569886	0.978937354953976	0.159478173175479\\
0.417232181140286	1.00983197106356	0.224787873848702\\
0.481064852892179	1.04740121192606	0.291947225524282\\
0.543566132632117	1.08224217749785	0.357307703517591\\
0.608078679972692	1.11415210912127	0.429078478255093\\
0.672066702127995	1.14766939923219	0.49671352484031\\
0.732981496090601	1.18166390481801	0.568159265928992\\
0.783627929520301	1.21376666421331	0.640942806117818\\
0.8344997953883	1.24690171289741	0.716566771170719\\
0.885039902463244	1.28073374473318	0.786940207782146\\
0.930708452832229	1.3115687574571	0.860905840384476\\
0.98360931213329	1.34306895639374	0.939576414751668\\
1.03603582288931	1.37468961101943	1.01230001250279\\
1.08966971776071	1.40527663662884	1.08296245920174\\
1.13626295165955	1.42561490088607	1.15306202232274\\
1.19215253749428	1.45547645371559	1.22816334027747\\
1.24157209939946	1.47269876202887	1.30333572842356\\
1.30164444783406	1.49081693517748	1.38450619067058\\
1.35424781864775	1.51250693156614	1.46719124853321\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998143503907388	0.237834720674987	-0.997862096085271\\
-0.936119373375667	0.29635870836499	-0.948464643518147\\
-0.877015955066647	0.33924871954674	-0.903160394177027\\
-0.812590672948743	0.384192528212344	-0.858675410842631\\
-0.749281978678445	0.43131747400185	-0.814889078940378\\
-0.683932352360197	0.479000083663537	-0.772748103589553\\
-0.623711676075119	0.531963156861454	-0.73212274666469\\
-0.564845833995446	0.581550208705826	-0.694764928561899\\
-0.5055480002133	0.628453895740117	-0.65908097128571\\
-0.444316879162597	0.674607389249144	-0.623936411013735\\
-0.380007057096599	0.724880882819921	-0.58393302298713\\
-0.309997303481852	0.7756871852443	-0.543238813205964\\
-0.239000843607946	0.830241204981572	-0.500675070154326\\
-0.172836106117607	0.882627757546596	-0.460227256581453\\
-0.106308300553263	0.938201516825577	-0.41703412596941\\
-0.0471534947563634	0.989288780128619	-0.371691141212866\\
0.0117366833573346	1.04837825859809	-0.331429212711511\\
0.0727443352361	1.09819029551659	-0.293151152697399\\
0.135386836081989	1.15896980561673	-0.254126685777976\\
0.198628929069509	1.20673347677698	-0.213717569504495\\
0.258673408497719	1.25994052522973	-0.173099333122474\\
0.320150846837991	1.31866106270209	-0.134773249158211\\
0.378929026791078	1.38521212080011	-0.0983565558729863\\
0.437873959975012	1.44270196064706	-0.0614942750998124\\
0.492321536975069	1.50285652136453	-0.025457833716979\\
0.546318410874817	1.55391028322688	0.0166150332734676\\
0.605540743583913	1.60912346203265	0.0588836632214943\\
0.666835145503873	1.66369002246334	0.101656455169822\\
0.72514641941733	1.71731321995269	0.150913802880084\\
0.782775627550259	1.76859293944252	0.196711908174917\\
0.845024159096932	1.83350206120734	0.240048580285645\\
0.905431261187945	1.89610129815776	0.285097770227969\\
0.967434816477778	1.96053005994677	0.329864810774429\\
1.0263995539753	2.02495426435714	0.372367418412664\\
1.08691134623291	2.08659693821654	0.423219304952599\\
1.14247857492891	2.15222889688014	0.470000266194938\\
1.20268458384461	2.22302768969197	0.520221362073296\\
1.2639002057665	2.29081616581861	0.567124247456189\\
1.31723846452443	2.3636705289299	0.616132282466592\\
1.37474288671603	2.42693167401703	0.661817703761842\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00142900461296	0.240147957678304	-0.998406460851612\\
-0.938197324332236	0.295334718464668	-0.952216015599749\\
-0.876839873964868	0.350178567484294	-0.901017568029402\\
-0.817496685826353	0.39618640386396	-0.849058939655302\\
-0.754302742769883	0.44098662705796	-0.794953670378155\\
-0.69192095378022	0.486774376254353	-0.748227583885473\\
-0.631354894185067	0.540080255498246	-0.701509102663529\\
-0.567160208013936	0.589033886692762	-0.65416397239147\\
-0.498960196856029	0.639448901286538	-0.606626205052239\\
-0.433302647164134	0.690927832605153	-0.559422133930822\\
-0.367502040962729	0.740061535168137	-0.510308694318523\\
-0.304932952225055	0.795547537011483	-0.462312130639576\\
-0.246133728336513	0.844070893732651	-0.416333206049848\\
-0.183151079213261	0.89667013869535	-0.372597622473266\\
-0.123073122467333	0.949187994951381	-0.323872478356829\\
-0.0599848181730635	1.00269707003528	-0.283246784079472\\
-0.000309752347445189	1.0556467315861	-0.235367346343113\\
0.063173487596274	1.10473570297316	-0.189521452313285\\
0.123886762248131	1.15126495604683	-0.149011666221997\\
0.186443847513615	1.19844426176845	-0.107739925708104\\
0.24693645963093	1.24410024797039	-0.0705626168191486\\
0.308258490539158	1.28967133235073	-0.0290909828346624\\
0.367846196243475	1.32535456310175	0.00330638897666914\\
0.427108524834924	1.36331730750391	0.0424891208927427\\
0.487278962720125	1.40173273654597	0.078392918436746\\
0.545400045400908	1.43415701456405	0.118292343076596\\
0.609133393740637	1.46883226202543	0.155340761660565\\
0.665965407605042	1.50147064154481	0.192594451722163\\
0.726813411340104	1.53465599570732	0.231493014982381\\
0.78525879049664	1.56803461360385	0.269073261142687\\
0.838786959347744	1.58847390345152	0.303170465642419\\
0.892005642473626	1.61372688249988	0.343783246671645\\
0.950855960118939	1.64824200717464	0.372693398799394\\
1.0072378680843	1.6714115179774	0.404857575435964\\
1.06370903706535	1.69829559562477	0.440066723251571\\
1.12481121783017	1.73151505961917	0.474039891532218\\
1.18624750005605	1.76011557948633	0.50961939888103\\
1.24513870865576	1.79057214961095	0.545563326536426\\
1.30048742944756	1.81247736836193	0.580687749516901\\
1.35829865956036	1.84178797899312	0.611136084006384\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.000431929394	0.242108810241391	-0.996613678930367\\
-0.935395247542184	0.296696837414976	-0.949268898252742\\
-0.873466293320584	0.336764606567942	-0.904652114447874\\
-0.810857531351084	0.385165017454719	-0.862627261291802\\
-0.745019123144069	0.428570708651443	-0.823328312950029\\
-0.679732999223635	0.477891179298135	-0.778109137581995\\
-0.614085299734276	0.525537029290357	-0.73407857204494\\
-0.553436679857362	0.568002879711038	-0.688347702132144\\
-0.48873106549623	0.614967439871658	-0.643905357028129\\
-0.4257494399878	0.661433413824767	-0.600762487765264\\
-0.363236170211182	0.707915303996083	-0.558763809627151\\
-0.303957803765229	0.753165135814846	-0.520776306799409\\
-0.24553924893707	0.79938725917993	-0.481019442302414\\
-0.188214276627694	0.849078387009438	-0.440856542605533\\
-0.128743658521414	0.894051825053391	-0.404589860691225\\
-0.0744397850636842	0.944413409009806	-0.37611361594768\\
-0.0203425627323284	0.989312849002061	-0.342400349984501\\
0.0359658143602226	1.04358101270269	-0.312861974034751\\
0.0925091039836771	1.09763602470283	-0.286264633099817\\
0.144807044968857	1.15212865150002	-0.25918860109279\\
0.195680860483034	1.21246766894415	-0.233152024596562\\
0.240935939112717	1.27762167330057	-0.204539391843426\\
0.291908249317216	1.34282715546215	-0.175139414471213\\
0.340000559067686	1.4063321122499	-0.147170027959631\\
0.39158194427972	1.46969012595874	-0.118719167386497\\
0.442579932439202	1.5367482694804	-0.0870962927934579\\
0.488893576129766	1.6060146048989	-0.0532176495575057\\
0.532908376754002	1.67309253795844	-0.0226400508827586\\
0.577611649866443	1.75170206681924	0.0101117423579534\\
0.622171702248338	1.82756434998143	0.0446559497183861\\
0.666018123806787	1.8964131217669	0.0834059606004055\\
0.715364591791782	1.97093698788423	0.11904090063922\\
0.759105280982104	2.04473207028721	0.15684534030507\\
0.801045366455763	2.11641537296264	0.198211436191412\\
0.852682136375208	2.19166312589285	0.242416508774737\\
0.897160014769339	2.26941307026482	0.277077230807292\\
0.949585212081186	2.35692661164114	0.316272231060444\\
0.991432937900816	2.43551139464911	0.355832102985598\\
1.04250084342095	2.51861318429785	0.400757017845699\\
1.08025195696505	2.60354495538013	0.44687055238035\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999675674549572	0.240809603814368	-0.996921683921689\\
-0.936509765495007	0.295010362876939	-0.946156867203659\\
-0.877103012466081	0.340598187773546	-0.897014585165409\\
-0.818272275394896	0.387880425247887	-0.845897554927339\\
-0.7612194144048	0.435420541447693	-0.794485899749282\\
-0.704979922365958	0.479729633550489	-0.741286744571794\\
-0.639208909238037	0.52062089366172	-0.692090257591796\\
-0.577984003417673	0.563109006909322	-0.642529064414549\\
-0.517015284371299	0.609516847928064	-0.592728708926859\\
-0.453773579922665	0.653794869828183	-0.541515223852534\\
-0.390079089332476	0.697274369166527	-0.485863733536751\\
-0.327504657776601	0.739934896551448	-0.429486405389553\\
-0.262046441398609	0.782759138766421	-0.37033900678668\\
-0.200656581709071	0.823695585443169	-0.314480824297384\\
-0.135284097210144	0.856714784846357	-0.255904593947051\\
-0.0762283681468417	0.903093108106359	-0.202002253319113\\
-0.0157703330350061	0.945477958711656	-0.149355461581598\\
0.0496086043769402	0.983430956724827	-0.0939053984881232\\
0.118090518779486	1.02445102772296	-0.0402722598189369\\
0.193554947819586	1.06240224522367	0.0130537006441972\\
0.267871710043001	1.09142390631313	0.0672498013698857\\
0.340769264519242	1.13167393744778	0.126832226891232\\
0.415027483905811	1.1684706298973	0.185288116350222\\
0.493316719837835	1.20831694210164	0.246903465407932\\
0.569107983300983	1.24994792427442	0.306778315649002\\
0.643339190981587	1.28563769326021	0.362948265532255\\
0.717433211087527	1.32212580465582	0.420520769832319\\
0.789162984553019	1.36187154184974	0.47776243035757\\
0.857169685997231	1.4034313712596	0.529632835913584\\
0.924296060951781	1.43705292018788	0.591922695395719\\
0.99248551362416	1.46425018627655	0.653714754855534\\
1.06219677563893	1.49906144777219	0.716928985872617\\
1.12793576496037	1.532796602114	0.784138692702429\\
1.19188657303142	1.57148097241137	0.851479263160206\\
1.25398166792128	1.61627880764542	0.925146542849287\\
1.31955955764024	1.6621984086671	0.994470907699137\\
1.38426700887822	1.70276569314377	1.07090787017195\\
1.44694614785174	1.73113117810826	1.13828249090098\\
1.51331152355335	1.77379614841949	1.20205150378024\\
1.58202688317567	1.80498441091493	1.26572979578591\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998523188471092	0.24048552892452	-1.00170842600049\\
-0.935694876595461	0.294255158763531	-0.953312919699704\\
-0.873418569530788	0.338750563478147	-0.903297305057812\\
-0.805937368358524	0.384714228935152	-0.856472366409174\\
-0.73644881916597	0.432362602700558	-0.809117172270303\\
-0.666096514273311	0.47435451738839	-0.762009897867566\\
-0.591687476407541	0.515490821271538	-0.714647926220729\\
-0.520202312442606	0.554686755200702	-0.668895876428494\\
-0.445075328958954	0.597204489312534	-0.620528376394389\\
-0.373611501295216	0.636541202900459	-0.573202326591494\\
-0.295549321703794	0.675197984979172	-0.531126962977454\\
-0.219949517412132	0.716566562050213	-0.489533313473778\\
-0.147744684498745	0.762571193658453	-0.449373578371776\\
-0.0747871774099083	0.805580254413355	-0.405371776163637\\
-0.000202109465291554	0.846650434434639	-0.363725599102718\\
0.0753779075001549	0.888742353086232	-0.324305521727015\\
0.148253855657127	0.930235521506898	-0.283263750983281\\
0.223504508926574	0.977710040914858	-0.241468903491411\\
0.298977616156341	1.02924642998083	-0.201342160570331\\
0.371607400002179	1.08011982849191	-0.158799968742345\\
0.44370301713544	1.12859088483185	-0.119848679034722\\
0.515670821589246	1.17716622598193	-0.0756963960955148\\
0.584310341113133	1.22100853665103	-0.0380155945506723\\
0.659067341253921	1.26929434150498	-0.00232670106254471\\
0.732343555720719	1.32066213858617	0.0353356334245465\\
0.80901870036679	1.36620824688496	0.0765995747885008\\
0.884830417415499	1.42409074044718	0.117268979460787\\
0.953978596030018	1.47702275851655	0.157121450691774\\
1.02794018824188	1.5266594734392	0.194957906169915\\
1.0977445584735	1.5784186864705	0.235820516626036\\
1.16676120248622	1.62998773548756	0.282958365704768\\
1.23308664372872	1.68333826260255	0.329986096163865\\
1.30143636944258	1.7270812039364	0.375240226634142\\
1.36936122985612	1.7726067393875	0.423324001247358\\
1.42882773716402	1.8141801079722	0.465804077238354\\
1.49270864182533	1.86094409073697	0.517680618134507\\
1.55421912696374	1.90875222482126	0.564929672971485\\
1.61189952531815	1.95651327017592	0.617552476208053\\
1.68018299996685	2.01627387974435	0.671481385110162\\
1.74317521048629	2.07317420510261	0.725931570315693\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996266401555801	0.241065408109953	-0.997524270030674\\
-0.935616037530966	0.298961037372814	-0.951290848895173\\
-0.874271186655702	0.341871700352364	-0.899247061247083\\
-0.809770474953617	0.390197258806424	-0.845434199766446\\
-0.744783683903365	0.440345301405434	-0.792957324392102\\
-0.67832651014073	0.489964877939231	-0.74178982719984\\
-0.614311038930228	0.537634431299462	-0.686781912050792\\
-0.550704392560502	0.587461630952286	-0.628914223909\\
-0.485076361067475	0.645340318151365	-0.570181501562755\\
-0.422779396086289	0.693670264799247	-0.513776130221047\\
-0.358407445522421	0.745514559139438	-0.45387248940336\\
-0.294554756489185	0.800494452650882	-0.395580236585909\\
-0.228370504371983	0.857626438502614	-0.340759525021052\\
-0.164919570666964	0.918189069285596	-0.284081000782394\\
-0.100428300424231	0.975671411156861	-0.233126161714587\\
-0.0364873631808184	1.03354529816135	-0.174485607486058\\
0.03039503565278	1.09414494202886	-0.120043416591615\\
0.0966370966310939	1.15705947319445	-0.0604133705478779\\
0.164139675264674	1.21258994170563	-0.00387211094833333\\
0.234579919298428	1.27117994893513	0.0555895249896556\\
0.305604083576958	1.33347476322621	0.115301323866013\\
0.379635059950721	1.3991913971082	0.179514850063613\\
0.445239738524514	1.45915603264508	0.244340787753376\\
0.511424747596353	1.53032589957715	0.308376282465888\\
0.587592606715259	1.59903285665379	0.373734646131174\\
0.662927073760067	1.66167057488262	0.442080929446937\\
0.733463540853294	1.72478466110331	0.505233329322579\\
0.808293643815278	1.79699096215508	0.569880227308837\\
0.8822383050201	1.85960945772145	0.63979966364737\\
0.956602348522238	1.92284929365042	0.707140390382085\\
1.03346178189316	1.98734342347434	0.773131982992607\\
1.09750265277435	2.03994716096301	0.839721978493359\\
1.17178781605971	2.09700204093048	0.91469809006404\\
1.24578754766594	2.1606719798423	0.990379204647398\\
1.32598663784628	2.22737527943389	1.06791622348461\\
1.39326662282973	2.27572595369693	1.14591160953309\\
1.46317253085109	2.3362594425709	1.22851334309658\\
1.53616151781272	2.39669887221766	1.30699230440716\\
1.60590422014942	2.44918304097556	1.38804621914146\\
1.67886003856337	2.51380092142403	1.46795566141155\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.996553195622749	0.241428731307668	-0.998680181989563\\
-0.936946398371795	0.296336888334277	-0.952899488956145\\
-0.868689540023367	0.344896077759647	-0.908049532780763\\
-0.797570013485324	0.392245353521358	-0.858788927314199\\
-0.727135133834651	0.439187572096872	-0.810245505490446\\
-0.656863674494348	0.491748415547409	-0.762986536853851\\
-0.589304108632216	0.535215398766491	-0.710713696252079\\
-0.521841596907772	0.583515855202647	-0.663010546813638\\
-0.459070593961333	0.632181652937738	-0.617375011773583\\
-0.396084333707836	0.68122609357534	-0.566609871526138\\
-0.331537023497307	0.728529095980444	-0.516462479103587\\
-0.270461608280935	0.776666307276697	-0.468661122470562\\
-0.208959096208436	0.82253710485579	-0.418560260672453\\
-0.148109906408346	0.867854260607204	-0.368559657787423\\
-0.0852661901429587	0.911916664075609	-0.322616294682748\\
-0.0281724629784662	0.956549830375345	-0.273431922590461\\
0.0316297453834707	1.00411955573829	-0.226040408533207\\
0.0940424900614943	1.04969457192387	-0.177012415465904\\
0.153463820027174	1.09871927638879	-0.12832482154147\\
0.208426073295889	1.14300127994308	-0.0758349198329008\\
0.263029737410235	1.18294801174318	-0.027244607005956\\
0.309987666860116	1.22848019726555	0.0183252554270275\\
0.355168539900888	1.27011340902465	0.0641514958055227\\
0.400838745159028	1.31232369003444	0.104748933688482\\
0.446210174248702	1.3561230716174	0.14553077380875\\
0.490297226838374	1.39353204803897	0.184628834162501\\
0.53132077982562	1.43449859590389	0.225259351355798\\
0.579360011591246	1.47423522063302	0.265770644211078\\
0.620114687428883	1.5137881427356	0.310008645574089\\
0.662268500042963	1.56344772551497	0.35352676324262\\
0.704181777392747	1.61483448149668	0.393366649469507\\
0.74416992319634	1.67017122458545	0.4359345662294\\
0.786861093748554	1.72853097027624	0.480056910850364\\
0.825863620126442	1.77262520011	0.519936418871072\\
0.867748587436645	1.81846500584132	0.559978643448845\\
0.904348079717769	1.87077411002873	0.601503898989438\\
0.939957131715918	1.91938102343195	0.647163560902774\\
0.984100613984313	1.968429123356	0.687504026488806\\
1.01875351501244	2.01604337703786	0.72948485477501\\
1.04955551295515	2.071497787221	0.76585638322754\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998879902201073	0.240496085513992	-0.99988366606658\\
-0.939370794986175	0.299688628768168	-0.950860526824933\\
-0.873789045122942	0.345583716334724	-0.904156203431173\\
-0.804188423871314	0.397335530731634	-0.85364545886601\\
-0.738232606420457	0.45007556760859	-0.806257935093803\\
-0.673380637037804	0.504234232855233	-0.75674450493024\\
-0.609847130544732	0.562259906775999	-0.704740058997178\\
-0.544257641839152	0.613043902150979	-0.657951432356445\\
-0.474965162789158	0.664304469295863	-0.611695161932119\\
-0.407099820977274	0.724749841543837	-0.558969937446712\\
-0.33348289548803	0.783060905035537	-0.506787300641006\\
-0.26540003473959	0.841948910151505	-0.457250201837349\\
-0.195976614764264	0.897326878189592	-0.409250105902261\\
-0.123554371748513	0.955647713582156	-0.356437774225914\\
-0.0552666572992857	1.00993096643663	-0.308400481284111\\
0.0144717608967379	1.06703826389719	-0.25437161816529\\
0.0911764688052082	1.11871904774566	-0.206025367099183\\
0.163761483087618	1.16945201153436	-0.153264874298582\\
0.237617842680693	1.21996092266649	-0.103993833305754\\
0.31463664029243	1.2789093299813	-0.0549133951063001\\
0.393438353942507	1.33219400122285	-0.00456118324455546\\
0.470623632413837	1.38843610152572	0.0422677329824553\\
0.5526201097657	1.44449013484385	0.0885204495478698\\
0.634651552228326	1.50616302618079	0.136904016950607\\
0.72025096587917	1.5724370314638	0.189311364249635\\
0.794706215447156	1.63153022791049	0.240944076360831\\
0.880896683430186	1.70352199722535	0.295045005811415\\
0.966734560096649	1.76698222317146	0.338746543162434\\
1.05158054734628	1.83490239619738	0.383807170676711\\
1.14501742093597	1.90974711679438	0.428760396921591\\
1.23643583967319	1.97863582803307	0.464731570803217\\
1.32462125867028	2.04379879798905	0.504847827125861\\
1.41534672207407	2.10608913194866	0.539949721838696\\
1.51144870099735	2.16982541766346	0.577831754697006\\
1.59059562940606	2.2382519077932	0.614215323291034\\
1.67620167064393	2.30195908047853	0.648005908040606\\
1.76144098834775	2.36756621870626	0.684560028601531\\
1.85342007642594	2.43203666681135	0.712997443832887\\
1.93248096066779	2.50270747971638	0.742465233245272\\
2.01662392343828	2.55281677520205	0.766402992723045\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998186840084946	0.241238126532768	-0.99575913010429\\
-0.93910655074124	0.295197335550279	-0.94816137861081\\
-0.879566605680491	0.34774384672798	-0.904031152519019\\
-0.815485814067297	0.39518190071445	-0.855337447663044\\
-0.751283235483321	0.447638161782792	-0.807095082872336\\
-0.68777329853078	0.498580686058877	-0.759130780209098\\
-0.623532697387901	0.54981545761173	-0.712553875593714\\
-0.560444288094363	0.596732133763351	-0.669823215352021\\
-0.500923289589524	0.649962270044387	-0.630354768568722\\
-0.439217692788261	0.70269553082119	-0.597529292235517\\
-0.382377505947668	0.753636233053346	-0.565417465490072\\
-0.326986875308349	0.808659484033586	-0.533639240895368\\
-0.276188885195786	0.863493979132822	-0.50445883928031\\
-0.220440558413139	0.922386013886069	-0.476520822699489\\
-0.167307434473189	0.984501715839633	-0.450362731923827\\
-0.115980537432391	1.04575834750217	-0.42361032661191\\
-0.0605358746356502	1.10209660914717	-0.398929354089092\\
-0.0124327974852918	1.16072501346216	-0.371653134877353\\
0.034373815565122	1.22345447538754	-0.342406795347864\\
0.083441933861303	1.28633735897505	-0.315279287820554\\
0.129345241622559	1.3499962899717	-0.286714139511742\\
0.173700219918909	1.40807926239857	-0.261012966568939\\
0.216862447993608	1.46865706647241	-0.23840836540336\\
0.263608652318412	1.53897001686056	-0.205886321889335\\
0.30119146157233	1.60681819495591	-0.181663804550202\\
0.339887347097249	1.6722033398497	-0.155163638663346\\
0.377296124081438	1.73704096989589	-0.129173329717089\\
0.419244588911832	1.80532865269098	-0.103187554488832\\
0.461599638526467	1.874338641162	-0.080219185013098\\
0.500299350194451	1.95379052822162	-0.0602792524145983\\
0.542228900556564	2.02021763986239	-0.0325275099175743\\
0.579641688465665	2.08746259300911	-0.00937972038193605\\
0.623227073988167	2.15365560616595	0.0195321961606601\\
0.665600501944054	2.2253126287606	0.0434950617180265\\
0.712914359812287	2.29086498906892	0.0728816646467084\\
0.762924661189738	2.3626291983752	0.101602939638156\\
0.809700720262381	2.42841258189739	0.128586396792931\\
0.858518206548166	2.49392383211801	0.155222973011852\\
0.908667903130117	2.56441707039368	0.174748914416757\\
0.953441004133035	2.62692835231056	0.193056381098966\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998501463206577	0.240622048850611	-0.997956032982096\\
-0.937380092684389	0.299739589435348	-0.948773765656467\\
-0.87288428821746	0.347166221913456	-0.894320302504629\\
-0.807684610880128	0.396017859973276	-0.835151346077745\\
-0.744529176595335	0.444283635809204	-0.776977159531321\\
-0.684774500862059	0.497270244904476	-0.722827206419273\\
-0.623058659794482	0.552846761725483	-0.674611875493064\\
-0.557856907490218	0.603684184662123	-0.624846806898406\\
-0.496017379702059	0.652288335401447	-0.573934216827273\\
-0.43300214697173	0.697762032164445	-0.529414021468079\\
-0.371599276837317	0.741167709577692	-0.484825068934523\\
-0.309379588785731	0.78443817232376	-0.435807416039495\\
-0.248278621653015	0.823641573001581	-0.391412712832659\\
-0.190766229789827	0.863015670568478	-0.352671634355826\\
-0.132950857574769	0.900897601534577	-0.315171867906392\\
-0.0785247158253818	0.939622352569191	-0.273730439469658\\
-0.0208412267141289	0.977094025030942	-0.236186927751407\\
0.0332996331060053	1.01712525855086	-0.19707575583392\\
0.0849339521357008	1.06091755685768	-0.162941831995224\\
0.143076282026755	1.11128190240168	-0.129669269501444\\
0.20129723334914	1.153573022764	-0.0894201939493836\\
0.259652317216535	1.19729800428796	-0.0599667397297685\\
0.315237186577836	1.24883014064212	-0.024474621888829\\
0.365262307022047	1.29946267625776	0.0084960433227074\\
0.411739106210097	1.35514135094607	0.0410666842690655\\
0.456330172505233	1.39810397050393	0.0749012268964479\\
0.502916568478967	1.4489316490109	0.108553878157218\\
0.550320654886159	1.49342870763487	0.143259081876911\\
0.597633145833903	1.54265003791567	0.186611771047641\\
0.651254439085877	1.58989861541072	0.225795991854095\\
0.706089601716066	1.63824149921117	0.265464746672398\\
0.755232603225867	1.68050412134056	0.302410296115793\\
0.801892633952299	1.72176174228032	0.338168917135952\\
0.851107023511234	1.7598184382646	0.379277603095691\\
0.910045444506951	1.79817423689589	0.419285501841558\\
0.961868295151989	1.84519947095436	0.456521047292635\\
1.01436343173049	1.88725122739054	0.489987371502914\\
1.06542357727094	1.93391401759271	0.52582168386404\\
1.11707626417437	1.98249589454058	0.560983146840853\\
1.16637519937206	2.02691607247731	0.594805476282318\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99941386444476	0.23981958381857	-0.99940192455211\\
-0.935790783494671	0.295973440151058	-0.946644440945783\\
-0.870953484147256	0.337920676615916	-0.895624035090351\\
-0.806049533947736	0.38222421949771	-0.84251474270725\\
-0.740628400801643	0.422809568428598	-0.785407613821271\\
-0.680530627252956	0.462177667265037	-0.732220734954956\\
-0.61755393063427	0.500809723334486	-0.677468006362588\\
-0.553039189053207	0.537744681941029	-0.619959926684529\\
-0.489261787921256	0.578833756878931	-0.563527496873362\\
-0.423585694721391	0.628139430911374	-0.507387672388164\\
-0.358626023549135	0.671992438111445	-0.451438345867636\\
-0.296604452183055	0.718979492251215	-0.394927180571802\\
-0.233893918287818	0.762479305620649	-0.344553852355452\\
-0.167105297522116	0.806033925762861	-0.294907121623299\\
-0.100313319827201	0.85173982157492	-0.243923305374739\\
-0.0347131128428459	0.899667072910527	-0.188163931381889\\
0.0318992766133705	0.951575077588766	-0.1292858123271\\
0.0939587124992772	1.0023203271045	-0.0722763537621054\\
0.155471461729173	1.05367549544397	-0.0178115528891776\\
0.217321132960819	1.11225191889027	0.0369684793519381\\
0.27554528441688	1.16293097072858	0.0897093697707379\\
0.326660311383942	1.21901725621047	0.140407098341125\\
0.385442278344885	1.27733913367489	0.19077295311036\\
0.442732556338243	1.33109214322283	0.242704778539406\\
0.496396603946829	1.38733670957261	0.29438914405709\\
0.555329633902037	1.44313816929292	0.346349961766558\\
0.620033187587347	1.49933564394949	0.390839968070357\\
0.681681133192265	1.55385734626562	0.444059387189137\\
0.744135120431133	1.60681685856481	0.497028103161948\\
0.806308037579827	1.66159800091263	0.548153405497722\\
0.868407163507737	1.71062740831277	0.599199521246646\\
0.934676220674764	1.76448356459484	0.647910551823576\\
0.994983441668676	1.81627499769647	0.706145087474844\\
1.05601828200952	1.87000952781779	0.763689518130537\\
1.11861872131484	1.92268947511914	0.822631392863396\\
1.18239123002556	1.97118733942239	0.883338236373165\\
1.24547410558845	2.00886829986752	0.942097873926395\\
1.30541690925659	2.06605985835185	1.00160730671751\\
1.37020522015701	2.1142811032267	1.06388348153475\\
1.43553978055996	2.15908326526873	1.1259099546486\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999628468123505	0.239790642200563	-0.99897927759309\\
-0.939925800908706	0.296042592806576	-0.949064983131013\\
-0.875266349827194	0.341981759663927	-0.899805478039031\\
-0.804988157029969	0.388379733543896	-0.848054750657497\\
-0.730863878676326	0.439183077783096	-0.798524228362854\\
-0.657229628784629	0.486499827915499	-0.74908000212884\\
-0.591572705893785	0.534692114499472	-0.692385359734553\\
-0.523491044983277	0.580256089716363	-0.637898006433409\\
-0.457554556262484	0.626900853575511	-0.579719222240134\\
-0.389307561274564	0.675277867740183	-0.520757303740208\\
-0.321688393728467	0.722238445144696	-0.462161158743266\\
-0.261025051333469	0.772806747316398	-0.398790377925144\\
-0.201063345419251	0.825260249199859	-0.33289621954988\\
-0.142939694616152	0.880967357489524	-0.271365782089549\\
-0.0813910921469937	0.936155200593185	-0.207630848641898\\
-0.0210017469487869	0.98501080558381	-0.146600239202634\\
0.0408571880641842	1.03141430640984	-0.0835191396259772\\
0.102559629102903	1.08339897598826	-0.0226885379086642\\
0.163285941463538	1.13423531389365	0.0368329525571538\\
0.219276401783637	1.17918896804226	0.0982186832816128\\
0.276765559566223	1.23679105028662	0.163320752261187\\
0.333328969610198	1.28749214820276	0.231279035800933\\
0.388619171172642	1.34493843504955	0.292770640756229\\
0.444828414861031	1.40285138095071	0.357407266050898\\
0.494106637458335	1.45481133434207	0.417668955022045\\
0.551519976997145	1.50744282891953	0.479277005462752\\
0.609527334442341	1.56374080085298	0.533384600137526\\
0.660641882932611	1.61065360475036	0.591186262409852\\
0.707875668819173	1.6616160999572	0.644315273213129\\
0.759877049222264	1.70183406754071	0.698100463494905\\
0.807391382574032	1.74113329991917	0.747273110092868\\
0.860306972237768	1.78248401822611	0.806325190862904\\
0.913578169490901	1.82597288384577	0.87063592936746\\
0.969532391995316	1.86960373815914	0.930738166463832\\
1.01990463281503	1.91287429474502	1.00193963235164\\
1.07299453257888	1.95180604141512	1.07103755000408\\
1.12383537811516	1.99496799553102	1.13293339534748\\
1.17997811518489	2.032273860388	1.20544540890979\\
1.23499557658421	2.06542254474042	1.27272747378511\\
1.29846587084545	2.10068936214979	1.33756443870261\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999289387007216	0.237332812311051	-0.99865554709324\\
-0.936795955100432	0.295679216182619	-0.947864624687105\\
-0.876927253238595	0.343276485769654	-0.901835879960475\\
-0.807559195861177	0.394613411621275	-0.854747083355907\\
-0.743768546633476	0.446741482146726	-0.809483242443629\\
-0.678382896751087	0.498546391877843	-0.768793193958187\\
-0.610558805239572	0.546513126155076	-0.724701612024884\\
-0.544798088817717	0.594782594672072	-0.682477760140318\\
-0.477717423893348	0.644362771969552	-0.639171197285377\\
-0.414418358748862	0.691799180516605	-0.600266258985882\\
-0.351400665563637	0.73769750361156	-0.560931573073746\\
-0.285030344315029	0.792222367499755	-0.520799493921138\\
-0.215875518663512	0.839978188612703	-0.482957520864315\\
-0.150297843540294	0.886646079218679	-0.447237042402936\\
-0.0834243279194481	0.941460547367289	-0.410865954985957\\
-0.0120904358143467	0.989775199494328	-0.368771018321348\\
0.0604389596442129	1.03455854433696	-0.321992784550233\\
0.128151640113722	1.08341974135171	-0.279405541600614\\
0.196461201678463	1.12184412337843	-0.236337765105618\\
0.261364979629248	1.16835261839804	-0.194519704650955\\
0.321670162964917	1.21348011410584	-0.148443088243086\\
0.386880370280435	1.25469593481258	-0.101284454693346\\
0.450604139635742	1.29798441047623	-0.0553452158533105\\
0.519616769322175	1.33857252486657	-0.00927014479227918\\
0.586521906558447	1.38208814561038	0.0334872371659635\\
0.651479688190949	1.42906114369178	0.0822244820957161\\
0.715133057155426	1.46881180996613	0.134969932829681\\
0.778497133532508	1.50840607572028	0.184921140176153\\
0.844392620888717	1.55205640548613	0.235492388502672\\
0.913743415717288	1.60113650258431	0.288495733080519\\
0.978645205210958	1.63933218766213	0.338369617629305\\
1.04825500823173	1.68263559166572	0.393018859135845\\
1.12063304513119	1.7377561187081	0.436865577122685\\
1.18924802745821	1.78313708669981	0.487671860194042\\
1.25671338534207	1.82607100488179	0.540897220914599\\
1.33248467847619	1.87102929043667	0.581395060032421\\
1.39846247339973	1.91831311160546	0.624230507074932\\
1.46414328393671	1.9681844481162	0.672364141523025\\
1.53497308785455	2.01054778187278	0.70841517391463\\
1.60973388371968	2.06134501267281	0.757824264378024\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998744597993324	0.239697364611478	-1.00082330309869\\
-0.934967296140122	0.29989064312524	-0.950157034366223\\
-0.86972779897256	0.344447275570136	-0.898492931569805\\
-0.80380434347782	0.395393403286442	-0.847069314899717\\
-0.736630584077776	0.442494611847942	-0.789790776091889\\
-0.674003912521172	0.487020472623881	-0.73099047887085\\
-0.611323579525427	0.536326358550417	-0.679711199720687\\
-0.547947112786439	0.579137292523701	-0.625531639441308\\
-0.481311197084737	0.625684368217938	-0.576752741050633\\
-0.409642341342085	0.671437090276521	-0.524345978719481\\
-0.336718700514058	0.719340455289502	-0.468647733249641\\
-0.263515877624212	0.764537815183044	-0.412902093600487\\
-0.193170181448085	0.817074647324963	-0.355392900262836\\
-0.121621247147764	0.85974469495509	-0.296083232311909\\
-0.0529290729005914	0.913964513283499	-0.234183540893584\\
0.018066553158035	0.967257398950404	-0.174826262009692\\
0.0855842031244479	1.01565889554435	-0.109527439163188\\
0.153506741555135	1.06719276334748	-0.0450340921768153\\
0.220285061205617	1.11310777866069	0.0210252373313124\\
0.281497338579451	1.17102949831046	0.0829191434970286\\
0.339841322499021	1.22475310286617	0.142844238515142\\
0.401649742735817	1.28167213514423	0.201115439123611\\
0.463472286329777	1.32816451866386	0.255587450212393\\
0.529027501161274	1.38937239025773	0.310707537689259\\
0.596295164673068	1.44161626270088	0.360966187991806\\
0.665240306388588	1.49373270512595	0.418294113130643\\
0.734892174207189	1.54703805668162	0.471188238947233\\
0.802609297475846	1.59677301506572	0.519727335807\\
0.876217114705428	1.64423008323368	0.577104341061865\\
0.946329772400645	1.69834838831746	0.636998461431551\\
1.01487012611064	1.74117426820574	0.693202951143347\\
1.07895364097138	1.80104867708122	0.747922193424177\\
1.14008865783622	1.84884542085864	0.792570040054611\\
1.19945130966865	1.90334134584269	0.842317791907883\\
1.25928968363361	1.96176365750833	0.888586581774754\\
1.32203621734675	2.01759594992835	0.933677571088026\\
1.38257667373151	2.0641937818398	0.978972812005777\\
1.44072191073415	2.12339258232747	1.03295774611234\\
1.50546098626268	2.18206423228079	1.07036803043518\\
1.55975887555877	2.23136827473192	1.11391344887868\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998885511378266	0.241910664800918	-0.996976547477393\\
-0.940040387614954	0.29766777320707	-0.951626881813066\\
-0.875761564352633	0.347260468102953	-0.907998660757468\\
-0.816470024118318	0.392983354135737	-0.858395523848572\\
-0.754390311738232	0.436969118715538	-0.807615616507622\\
-0.696814774846039	0.489813934789821	-0.756835415722019\\
-0.638662270138816	0.541508877072344	-0.704843504179646\\
-0.574028968528997	0.591552378645295	-0.647513506425095\\
-0.509217796623769	0.641755340240551	-0.592825936813614\\
-0.443576874144499	0.690388034449658	-0.536188529144945\\
-0.383392334500443	0.745883388683918	-0.481844860460854\\
-0.32076791702083	0.799986152509635	-0.427792737651208\\
-0.262775469604114	0.850507944820221	-0.372664024183134\\
-0.205120722121782	0.902966353198475	-0.317669078495082\\
-0.146466695321946	0.95216406785298	-0.262405454807257\\
-0.0944402357188441	1.00064680946135	-0.211676887176349\\
-0.0387710902211556	1.04811022977455	-0.155471755459173\\
0.0155118148154992	1.09073778226011	-0.100539150071169\\
0.0740883287702382	1.13531226263472	-0.0482031999438352\\
0.133198466176663	1.17946127642741	0.00682531674891407\\
0.186390976823255	1.22438350327784	0.0622041620040903\\
0.240426482745683	1.27381480766936	0.118910359755193\\
0.298220804718212	1.31774535893661	0.182176961892837\\
0.350962282352541	1.36020652557454	0.240485424587223\\
0.415578450780406	1.40564377342666	0.305952817557809\\
0.470425707641884	1.44524272280929	0.372190904752373\\
0.529456695012825	1.48131013532241	0.43712942967256\\
0.585962618128176	1.51817796589832	0.499198162661889\\
0.637974139056772	1.56445863246761	0.565512641325222\\
0.694442306998844	1.61081872437219	0.633828917433982\\
0.744965992305821	1.66223244724247	0.702182438107963\\
0.798239336855592	1.70818277921315	0.770943857544714\\
0.847036322537959	1.75413794824888	0.842854623769122\\
0.900452089866363	1.79544184131232	0.915267609387747\\
0.948305547722496	1.83679549021743	0.983009012267143\\
0.998056758900664	1.88047852779191	1.05674893858474\\
1.05288580690814	1.92371468087948	1.13069712490679\\
1.1109080787291	1.96615330191371	1.20299207227131\\
1.171317220047	2.001858577902	1.27624387367332\\
1.23238388325872	2.03815751318162	1.34446825975575\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00001242079505	0.236996152839202	-0.99819153226049\\
-0.934071827168765	0.296812721566474	-0.94900119376642\\
-0.869154732172692	0.344744304962989	-0.900387001894552\\
-0.79642778770078	0.394936458189387	-0.850653752790028\\
-0.724114088376697	0.438060104253512	-0.801718915695451\\
-0.650537362239834	0.485391800508191	-0.747573480286097\\
-0.57773296631891	0.529078210200821	-0.692855667079673\\
-0.504445910849418	0.582120446020019	-0.638795725563779\\
-0.429242111180558	0.633573562556222	-0.581522457967665\\
-0.355596050621327	0.689397248334908	-0.529820957518047\\
-0.277605823264592	0.744025645700843	-0.47633578096978\\
-0.199464303040165	0.801486135250879	-0.41671253912194\\
-0.122780568721429	0.861266032837976	-0.362785688665567\\
-0.0440789177556352	0.915108996921414	-0.311361944494187\\
0.0376143232755785	0.964246304458507	-0.259084321432278\\
0.114555016102637	1.01717209054488	-0.197963055414828\\
0.187652303337601	1.06501729941302	-0.137974963125784\\
0.26584750854522	1.12235537817069	-0.0722826722553435\\
0.342214514737491	1.17232645876298	-0.00694439717821829\\
0.425095419691448	1.23003949135393	0.0603241347804975\\
0.506051039720301	1.28562175609566	0.127239496273135\\
0.588726789046525	1.3455447752446	0.196363111926027\\
0.672750288388868	1.39837087970005	0.266023417678813\\
0.763300391205067	1.4537587327465	0.340530625352004\\
0.845050678727478	1.51670035775515	0.415465343803769\\
0.933384432083729	1.5761458834542	0.491962714885336\\
1.02078988600718	1.63705539115459	0.571323212294579\\
1.10603932995362	1.70225133901559	0.650189837848793\\
1.18831784754637	1.76770875406839	0.733853873662714\\
1.26777717813386	1.82873884287846	0.812237617839167\\
1.34952679680076	1.9049332078562	0.899655597811849\\
1.43023232104486	1.97248192837176	0.982938615477784\\
1.50815864026067	2.03757105632708	1.06420760837613\\
1.59801144846906	2.1096956557521	1.14491569803146\\
1.67678481840977	2.16956626187837	1.224696605501\\
1.75765028520496	2.23070549876961	1.29624968926503\\
1.84149806923614	2.29541484691098	1.37234131875728\\
1.92514715181643	2.37122963631975	1.44830650358269\\
1.9971120621971	2.43906794267888	1.52812329081828\\
2.08444550915334	2.50715141416051	1.60504175661068\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998959593193632	0.240823525972835	-0.999191176356675\\
-0.937010795032799	0.300216708677304	-0.950798757480133\\
-0.87334516007607	0.346598183946491	-0.898595061458361\\
-0.807243845062648	0.395176248501185	-0.846686296870997\\
-0.738726750337258	0.44901308854195	-0.792835340129378\\
-0.674809951292105	0.501516665581982	-0.735094708555018\\
-0.613246013689922	0.565083374984484	-0.683987868051571\\
-0.54891879701058	0.620154772982619	-0.626935790129387\\
-0.494581278850229	0.678818587696362	-0.570675149732432\\
-0.437961561225523	0.736192162727018	-0.510339127697848\\
-0.382006970165087	0.792729988358544	-0.456813446877408\\
-0.324940245612966	0.845608906805838	-0.406925583598001\\
-0.265459355197348	0.901028253007747	-0.358317956109875\\
-0.208780879225109	0.955769508095268	-0.312279004473023\\
-0.148822244643829	1.01457655363819	-0.268603560105727\\
-0.0903744801752249	1.06876803256187	-0.224527404626605\\
-0.0304028315660734	1.1214519565387	-0.178812812022271\\
0.0261867198232864	1.1799634297082	-0.135150437802118\\
0.0842436869465917	1.23110491121767	-0.0898054785672626\\
0.146511414082153	1.281126012722	-0.0454046688802251\\
0.200467321021819	1.32709893484523	-0.00216007815982188\\
0.257103877359511	1.3730911663498	0.0435746712649696\\
0.309144408186614	1.42404195628767	0.0868939116132905\\
0.360342798483346	1.47345591400591	0.134641943185379\\
0.414149720803435	1.5178097101618	0.18064810862728\\
0.472514186448061	1.56764316127003	0.229361709620298\\
0.527780466255169	1.62124292067037	0.283387300713208\\
0.581130005235912	1.66993874378876	0.342200478945902\\
0.634407725475579	1.72488377066727	0.396223324057947\\
0.692139517135441	1.77217418895066	0.454341751580407\\
0.743921075392271	1.82214649284332	0.51454618724282\\
0.79654300926419	1.87985002499337	0.577410328918531\\
0.854115664323511	1.92543174209933	0.644217003467266\\
0.90022435501774	1.96793687696675	0.709619137513361\\
0.966890599445676	2.01567905004838	0.781902994752975\\
1.02199232452066	2.0599629255512	0.849641584649331\\
1.07923862695916	2.10860169005699	0.922623894353172\\
1.13476459690299	2.1487117346492	0.992759550697976\\
1.19308301456914	2.2052443731381	1.06277004046379\\
1.23738648649508	2.25464620386159	1.12787503622771\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997171050210162	0.242309090692241	-0.996856148079034\\
-0.937953212107463	0.291755435391893	-0.950300294838887\\
-0.874338901098554	0.338380256899547	-0.897086027350147\\
-0.809936557705549	0.386072686519136	-0.848017856588324\\
-0.745226017347575	0.428677698644661	-0.794412132155935\\
-0.682260929886819	0.46539293664249	-0.741298955255845\\
-0.614482118094976	0.501047798801286	-0.686561242554906\\
-0.548526305100165	0.542715800119847	-0.631653466289102\\
-0.485189318634579	0.576620933496199	-0.574101718415877\\
-0.422431078751044	0.615974476458091	-0.515009777648744\\
-0.361523563236864	0.654856634204266	-0.456808022333485\\
-0.303253140899515	0.694586018559849	-0.399680829704244\\
-0.246141853522201	0.728963767175671	-0.336187767877396\\
-0.18904891675754	0.767986409842892	-0.277333602911615\\
-0.134219016517722	0.808695614020911	-0.215408219074509\\
-0.0747573033008048	0.843606849702167	-0.156692217518261\\
-0.020439103678019	0.880994131762678	-0.100807855237628\\
0.0308231566903629	0.920606330591664	-0.0416489872792073\\
0.0808987896925517	0.960693259966886	0.0132311483872555\\
0.13503506867386	0.998287652151354	0.0690422961662859\\
0.189121798651164	1.04605663037633	0.126899421908199\\
0.241632307076704	1.09533521782169	0.18321581161012\\
0.289088449535143	1.14818569882429	0.240838878250628\\
0.341635793937148	1.19844786306698	0.298515739981637\\
0.390620499027097	1.2514446960535	0.358623049495604\\
0.44037802866175	1.3057942783143	0.423754115037171\\
0.492366191100857	1.35979320576295	0.487627553340278\\
0.546959208579579	1.41876008517543	0.548116684093643\\
0.604939244749512	1.46904829359612	0.607578124750659\\
0.660573994833797	1.51906110742651	0.670788838088915\\
0.714346576479404	1.56530781521669	0.734290947927073\\
0.773232220495355	1.61769114305016	0.795908073882546\\
0.827056078168975	1.6685483539366	0.865222302470622\\
0.884649168799789	1.71609847453967	0.931142573225979\\
0.94279561381222	1.75541818859283	0.996761328191133\\
1.00365240816101	1.80281039374679	1.0601130003862\\
1.06139464529507	1.84850973278397	1.1218372490159\\
1.11176811346607	1.9064506906578	1.19580671838589\\
1.16752068001643	1.96114731062464	1.26199259438727\\
1.21242801334302	2.01176867289048	1.33151190333676\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99881542207184	0.239720675091591	-0.997009706141376\\
-0.93765438649253	0.293302287911362	-0.950338539456461\\
-0.869224040670987	0.341062677973897	-0.908219846069401\\
-0.802830145121424	0.384962598225273	-0.860089905537413\\
-0.736439119814415	0.428485983725362	-0.810663876648319\\
-0.6720725014157	0.473118919162488	-0.76157666135308\\
-0.60245268510537	0.512837574179635	-0.713395481161917\\
-0.535784511961406	0.553593169948548	-0.669184674280052\\
-0.46943362475402	0.590316720273654	-0.62140876858919\\
-0.405174768763193	0.627116208757717	-0.567639410473795\\
-0.341413477227322	0.658247247352008	-0.511749739559889\\
-0.274952109312681	0.686808168155472	-0.452594442425038\\
-0.212133355944118	0.712822282752146	-0.392052513313729\\
-0.150238256484949	0.747561761275763	-0.33143886344707\\
-0.0880784706303454	0.779728865981586	-0.274808037601344\\
-0.027241009211033	0.812778617646553	-0.217757421531806\\
0.0295094920265874	0.845846977734625	-0.158777798795608\\
0.0844644599779759	0.87003809891487	-0.101148612229172\\
0.136126783426729	0.901627949880876	-0.0450344538206197\\
0.185331432392828	0.934700539268137	0.0137375670675768\\
0.239245711797525	0.970980696186618	0.0698762516650012\\
0.293065230290556	1.00615936608342	0.126745002362658\\
0.3467361272706	1.04080800777651	0.181111997680564\\
0.40050250221656	1.06991908897503	0.243173940796566\\
0.45338491730481	1.10579333147593	0.298056240101713\\
0.505927408420464	1.14584979740738	0.358049174784228\\
0.557187442254682	1.18059088957487	0.419798414594443\\
0.612581072679843	1.21840820756129	0.480505434749133\\
0.668686584045907	1.26003803946999	0.538491828149655\\
0.718193141856078	1.29689957895612	0.598880508895309\\
0.768156830112073	1.33572758034375	0.660334870951474\\
0.823054801709109	1.37014354126151	0.721016806931345\\
0.872970513785764	1.4010853048614	0.778265407102967\\
0.916461767262063	1.42736373941219	0.841438082322793\\
0.9581234247532	1.46346311122217	0.908784035508842\\
1.00940237580738	1.48260922256318	0.977998602327537\\
1.05518353083684	1.50182569737712	1.04318962620448\\
1.10058996882661	1.52886099630075	1.10921458286862\\
1.14632596156738	1.55772619054662	1.17340932362644\\
1.19255061153981	1.5795581201526	1.23465112685251\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997012033215349	0.24330068421086	-0.997794551516377\\
-0.935046798425955	0.298331143526988	-0.948599736134172\\
-0.877277236483502	0.342459339848217	-0.902726415850275\\
-0.814669154167901	0.393082259395234	-0.856981882805012\\
-0.749920772611216	0.437942885646406	-0.807679066289984\\
-0.683661094653007	0.48777849040452	-0.755918285862468\\
-0.615854413113115	0.535417746192292	-0.699236077390068\\
-0.547529425554012	0.585554814945076	-0.646623772223913\\
-0.480691576204443	0.634305277389931	-0.595065014043382\\
-0.419153196352777	0.677119078228366	-0.539491424340906\\
-0.355294414861889	0.721092523051041	-0.486892311783569\\
-0.2908482045041	0.76611903355803	-0.431675315929284\\
-0.223698482560711	0.813334032213213	-0.37485043208904\\
-0.152302963352282	0.858028083916582	-0.32025107240638\\
-0.0841121191825706	0.914284559544938	-0.262546904637881\\
-0.0112241195221479	0.960153916225502	-0.207302417851785\\
0.0611541607231782	1.01720944185419	-0.154038639758797\\
0.130875427844638	1.07857116786437	-0.0947173547830037\\
0.200704812438192	1.13373001560595	-0.0419674127951958\\
0.274121980040014	1.19084234531123	0.00894577875177411\\
0.347242506776232	1.24223765103077	0.0546834713958657\\
0.418169622218477	1.29420207593525	0.0981704153936394\\
0.493912617695954	1.3510320642693	0.142897087055774\\
0.567470216808397	1.41680221662017	0.188926013040699\\
0.642893850621634	1.4797344126437	0.235581895090041\\
0.712250478568749	1.54312912430285	0.277834221027388\\
0.781320156877461	1.60995409592037	0.31834794263671\\
0.851328636946908	1.66759827741845	0.356788027957719\\
0.922317692307335	1.73136632070841	0.394917838158719\\
0.993139273470782	1.79275987572677	0.433501894570389\\
1.06208109058572	1.85260995675399	0.478472772888404\\
1.13085998158348	1.9080268871646	0.526415361146105\\
1.20561838425786	1.96031745717501	0.573650695661233\\
1.27940775815342	2.02909199764573	0.615813676925079\\
1.34812676516791	2.08579132681223	0.662019367126311\\
1.42323235006741	2.15256453372894	0.709438559981014\\
1.50163366840412	2.22009740292004	0.768343110669741\\
1.57865052890917	2.27819189196283	0.825738759724162\\
1.64886201638829	2.3423943225935	0.882816717518549\\
1.71839996723213	2.40376474448927	0.939394887715484\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998176300892813	0.237865833133155	-0.998194406771928\\
-0.937303139918043	0.301206038514602	-0.955159411637351\\
-0.877955500618571	0.341612321654935	-0.901700143340558\\
-0.815697139260197	0.38866548598159	-0.847394338464941\\
-0.754143895367212	0.430870756298495	-0.795036705558929\\
-0.695123827072046	0.47192298746436	-0.740694369683829\\
-0.636612473235756	0.513406346603183	-0.689101644847527\\
-0.575032286854936	0.553967385215815	-0.638111316675945\\
-0.513083470553701	0.595876225786883	-0.587766782640912\\
-0.444961479073543	0.640597481984597	-0.537032591693204\\
-0.375109129653081	0.686710488668791	-0.487021612306725\\
-0.305788006071599	0.738137242989012	-0.436234430769775\\
-0.236235057231604	0.790671883468174	-0.386684809936003\\
-0.166272574417097	0.844525951527236	-0.33937749510591\\
-0.0957488805514085	0.899234206104683	-0.294071544167977\\
-0.0287840323751033	0.947013920874275	-0.251677305336781\\
0.0370096021764849	0.998177322843597	-0.217118878873802\\
0.106559765166078	1.04915798202384	-0.185801895940089\\
0.175524576186528	1.09731864515887	-0.159031018255411\\
0.247090072300033	1.14257724693	-0.130554407973902\\
0.320650086654296	1.18591216187324	-0.0992287650876434\\
0.396506940491463	1.23054750219539	-0.0663487510487194\\
0.473262288155237	1.27090201263435	-0.0358039625641331\\
0.547150548605702	1.32022030747578	-0.00922259580246202\\
0.617612867216872	1.3638636895872	0.0196621500621873\\
0.694060621126363	1.41300564579005	0.0496943384016945\\
0.766817069046539	1.4620538715338	0.0795899787416229\\
0.840694727531361	1.51379585644396	0.107119387534553\\
0.916371968829657	1.55932985424325	0.137390991854598\\
0.986270069766298	1.60614246401446	0.157036274438943\\
1.05994897286179	1.65659647997805	0.177171941443293\\
1.14236102668261	1.70095270256798	0.198267012071467\\
1.22077245933225	1.7449746750989	0.217168008824423\\
1.30174902847641	1.80233641298785	0.236217088454865\\
1.38498294775674	1.84450456804972	0.257150003929835\\
1.46323256195656	1.89905012349442	0.281349483875322\\
1.54165447658842	1.94970008162033	0.299185692966051\\
1.61540358604717	1.9928729763946	0.317860407036865\\
1.69469191291839	2.04210792162139	0.335359285789529\\
1.7690063979206	2.08325071458976	0.348953423649663\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999026809756535	0.240084072736964	-0.997186525363316\\
-0.937873815393769	0.28967113699289	-0.947090346365476\\
-0.876860272021384	0.336162596714522	-0.899783480302242\\
-0.815991866953933	0.374145979761952	-0.845304774590324\\
-0.751994476824377	0.415632959899356	-0.794475312091002\\
-0.686778194362638	0.458797438851635	-0.739701187755375\\
-0.627605385818242	0.503830515606959	-0.68005789915831\\
-0.566547545387096	0.545637617384054	-0.622607224593526\\
-0.503936658596177	0.594855401902417	-0.564993427143466\\
-0.438320011588788	0.642782608333275	-0.504658429485865\\
-0.375478476232125	0.687192464260465	-0.44526305176219\\
-0.308159911482955	0.73004697263157	-0.39000716087015\\
-0.241156607477187	0.777411022254915	-0.336463856328745\\
-0.174061770631356	0.82403155585738	-0.277345976009463\\
-0.10486370531114	0.873540001962725	-0.215885276501215\\
-0.0368351010875903	0.921968606119207	-0.154301419672757\\
0.0352965784408696	0.969923748653492	-0.0985417381874972\\
0.107365650539453	1.01483411074924	-0.0439649237183216\\
0.17852823118301	1.06499157184381	0.0123500405207406\\
0.252988118991231	1.10798188326143	0.0692998063376193\\
0.324674321103164	1.15050947084429	0.121003339138511\\
0.397949577684284	1.19501616192912	0.180555936746498\\
0.473364431316479	1.24268040914959	0.239097947298748\\
0.545629887653631	1.28511754885857	0.29474247897868\\
0.624062823757318	1.33446554971271	0.348368203238439\\
0.696902145321275	1.37974103052407	0.39702875778487\\
0.765864186848373	1.42323863456084	0.448953727889677\\
0.835407573261454	1.47151330209006	0.496716204694803\\
0.911822953534982	1.52218291835479	0.545612252387766\\
0.987355304340101	1.57533580662666	0.597840773942296\\
1.06699119232964	1.62074241684759	0.640775965105837\\
1.1443542979802	1.66500212822931	0.694792355215661\\
1.22386349796091	1.71069188308638	0.740759768098063\\
1.30120078908873	1.75939351204546	0.780265499927767\\
1.38056713543597	1.8047598494121	0.824418111341939\\
1.45858501764373	1.8591800544068	0.867882324642663\\
1.53586213295151	1.90467116231381	0.911349175518199\\
1.61166310691167	1.95393255513782	0.950029641586803\\
1.69261146201018	2.00780060703468	0.993757001465706\\
1.76463446750705	2.05253411494051	1.03503570205977\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997879915141782	0.240723834463188	-0.999168889014659\\
-0.93748846371567	0.29578431763191	-0.949112663857146\\
-0.877506879767706	0.340666471202947	-0.901367203309815\\
-0.81828102223304	0.385778399581687	-0.851568414035801\\
-0.758475161648497	0.41728631044418	-0.790800486192482\\
-0.696758803682568	0.450605705924523	-0.733853644270089\\
-0.63012978521123	0.483857723835722	-0.676504194955924\\
-0.559901449700274	0.51515558376121	-0.620472334296321\\
-0.486488222387591	0.548557895308757	-0.560535094181325\\
-0.414254584382845	0.58645423104225	-0.50402883411144\\
-0.34326554769929	0.620158009652069	-0.444362201889022\\
-0.270252541405304	0.656875971545244	-0.386990669966016\\
-0.196781722409483	0.691933541867233	-0.327018374141601\\
-0.119339712032173	0.728207606773953	-0.270446554979799\\
-0.0392375618379667	0.762284876798912	-0.212516762445096\\
0.0415057536030486	0.804345008496095	-0.157295862094667\\
0.121531736053101	0.844624971425868	-0.0991319209041784\\
0.203639614171569	0.888855805124475	-0.0394044528791185\\
0.289487572404761	0.928857570711002	0.0231126599104726\\
0.376117204545984	0.968847786826805	0.0854360726969179\\
0.465095317817891	1.00740476415502	0.146591123438999\\
0.557493651169457	1.04422051330196	0.203524848471919\\
0.646824089656116	1.0780964891026	0.264323063934983\\
0.742863385230756	1.11676734553909	0.321822907861678\\
0.837293289437147	1.14754467520788	0.378478008567543\\
0.930407683833772	1.18480623858365	0.435963850931195\\
1.02223084245309	1.21310923073638	0.493826434766483\\
1.11237642567779	1.24304141275884	0.552845848946321\\
1.20135571679794	1.27085977331896	0.607994156445073\\
1.28703691402899	1.29764923427642	0.66330445628818\\
1.37928290914193	1.32455573233626	0.723390635976518\\
1.46633572506791	1.34360319370611	0.784467614375736\\
1.55746169070873	1.37249197476557	0.839519989063708\\
1.64768587859859	1.40569684452051	0.896841338311787\\
1.73632235954012	1.43182115355377	0.95415872997896\\
1.83167783360269	1.46284562124802	1.00858384733011\\
1.92885825317725	1.50539079342544	1.06530005971972\\
2.01950827512859	1.53759128973342	1.11422387640636\\
2.10790145732014	1.57350020728463	1.1586601154678\\
2.20074517062483	1.6147083344714	1.21414273416725\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998900049507609	0.23946258346467	-1.00236186302348\\
-0.93806067009773	0.302519151556484	-0.950950613184611\\
-0.875000445130725	0.34699679525257	-0.898855919643974\\
-0.807523332820102	0.399939492504463	-0.851285822771237\\
-0.738732635501012	0.445773708896972	-0.796963483493859\\
-0.669092704552241	0.501131436994574	-0.745389357327111\\
-0.60005637424219	0.548687998038143	-0.69339381968737\\
-0.533763555398126	0.601989143068871	-0.640513674384112\\
-0.466344084745919	0.654606823009821	-0.586634068745826\\
-0.398007404048346	0.710458816879273	-0.538198073873161\\
-0.327189986256386	0.759940545504296	-0.487007320007984\\
-0.257946654787438	0.809827569760894	-0.43996819690865\\
-0.191281519487314	0.861244261710227	-0.390965179810164\\
-0.12319918263032	0.911170938031984	-0.338469896876595\\
-0.0529063399520557	0.960457796370175	-0.284931000275585\\
0.0121370572840651	1.01574173164898	-0.229259852347004\\
0.0765303206470667	1.06787582952735	-0.170580592335158\\
0.143069308250466	1.11454289464276	-0.109509190008538\\
0.213559308238234	1.16392499238551	-0.0477897791321512\\
0.28721610406568	1.20789589857908	0.0114510218586177\\
0.358532529241753	1.25616075697514	0.0722959106392453\\
0.429327405177635	1.30578607630807	0.134477890687541\\
0.497203519831442	1.34870442139244	0.203180353825679\\
0.562254232382814	1.38330899227083	0.272396949975959\\
0.627976942961598	1.42390989812496	0.339621055467874\\
0.692711245350603	1.4621327251151	0.407176703813703\\
0.762052428146664	1.50546194634553	0.471666439366706\\
0.827083674656355	1.54118103022161	0.533528892923807\\
0.890655771335466	1.58813836406917	0.599556143715644\\
0.954075158083042	1.63126448288713	0.663433784543702\\
1.02342161611523	1.6765237438917	0.71983928635955\\
1.08952057837475	1.71923291006883	0.788377876124591\\
1.15523463036122	1.76660637978147	0.848800343627862\\
1.22134094805314	1.80706547855688	0.911423939221318\\
1.29078921686894	1.84387595527152	0.97058517630706\\
1.36389256135558	1.88184790069749	1.0292848380178\\
1.43414786255193	1.91928223170295	1.08661624506537\\
1.505150003754	1.964961398413	1.14547873735732\\
1.58129992660558	2.01361853179068	1.20726886686901\\
1.65858077122085	2.04374268460611	1.26623010975458\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998224655000947	0.239227642880987	-0.999584344680839\\
-0.938183365774556	0.296710244772038	-0.946828230357148\\
-0.879421108616024	0.342070775244995	-0.900653004904123\\
-0.82166056995277	0.388358721989544	-0.848728249590131\\
-0.758672746177095	0.437676404337165	-0.788815227408785\\
-0.696234678416448	0.483323644158982	-0.729668316975941\\
-0.630062237071506	0.526957723359955	-0.667599634269856\\
-0.56084383392734	0.573351786524257	-0.607117278261738\\
-0.494568391194088	0.623461572408495	-0.543282847000905\\
-0.430201062649796	0.67302141323129	-0.487191414986097\\
-0.365669219281314	0.710817066887927	-0.429540589155897\\
-0.301635764688841	0.757472276670488	-0.374631948451446\\
-0.238711485346451	0.794631524275093	-0.317800635707675\\
-0.176862364651176	0.832099208634916	-0.263700362004811\\
-0.113587870139848	0.871146482061936	-0.205391907212626\\
-0.052673869772478	0.906205089617722	-0.144114067397178\\
0.00804271305616219	0.948575148488696	-0.0829298377588602\\
0.0674849271209098	0.982415880306125	-0.0180213627134236\\
0.128903075544697	1.01730880235047	0.0530535798275169\\
0.190907749431681	1.04886893016138	0.121320853201782\\
0.252379156510826	1.08621983747133	0.193804436751609\\
0.315139499419469	1.12452651095244	0.26797162831777\\
0.378953618905509	1.15149262954047	0.340684298480034\\
0.442835878587877	1.18590449879145	0.416311108173326\\
0.505513346867512	1.2138013079254	0.484497381543919\\
0.566919430330379	1.24261920680413	0.555585856389909\\
0.631971287720878	1.27395118423471	0.631424174361061\\
0.693379736982473	1.30330890834518	0.706850974285168\\
0.753057309240758	1.33605743490273	0.779416091847091\\
0.816047411858848	1.36629210562833	0.853668317339531\\
0.884083930531003	1.40540869704547	0.926000431825431\\
0.947072681365749	1.43618280163544	1.00001698100536\\
1.00663420203886	1.47123221470779	1.07640235977588\\
1.0691447990303	1.5009622286756	1.15093479724517\\
1.12606186973462	1.5446864200095	1.22701164262742\\
1.17974472675541	1.58769448825149	1.30355404511283\\
1.2329264835621	1.62665571917759	1.37577149928208\\
1.28210258936641	1.66271999651647	1.44977142231725\\
1.33055578649617	1.7028061616776	1.52665462199228\\
1.37903574812156	1.74629378364962	1.60168294795199\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00068039801429	0.240653644756187	-0.999024335894011\\
-0.937253295640987	0.300747056284595	-0.948466637951207\\
-0.873652877040978	0.338650004030541	-0.895336306301265\\
-0.808113604720478	0.388253193978652	-0.841404607716261\\
-0.743978307833414	0.436430858469606	-0.788134022778441\\
-0.682478371160331	0.490718587451654	-0.737315538042155\\
-0.620992286937752	0.5365139577963	-0.68702622812266\\
-0.559126266454237	0.586339083846549	-0.638445314630722\\
-0.494960379644859	0.633528757751934	-0.589898566209941\\
-0.428543946918859	0.683150244550394	-0.542683692201893\\
-0.362373878711569	0.73042517132893	-0.492837526232333\\
-0.292264814548535	0.778709195805616	-0.443338481202199\\
-0.222913209015542	0.818688459852304	-0.39347693392683\\
-0.151905178353261	0.855789346155398	-0.347375085952224\\
-0.0786397332109598	0.893602641023956	-0.298894449829859\\
-0.0083435986758045	0.933263829790044	-0.255519614643458\\
0.0692654400206779	0.972730838622875	-0.207740520051098\\
0.143898911173719	1.00587304301728	-0.157196654923438\\
0.224904696508977	1.03794175311786	-0.110746295232362\\
0.308109665172005	1.07450635599904	-0.0650790587178632\\
0.391693928912089	1.10759844889851	-0.016851449573118\\
0.475247228923485	1.14339743846377	0.0330466799342419\\
0.558987369576932	1.1779462152993	0.0877520837481897\\
0.641236597108186	1.21279989619249	0.139539230690144\\
0.730327880690867	1.24736327756213	0.196787522417735\\
0.818403581360737	1.27869592800771	0.254486754886065\\
0.911133894349329	1.32304172617135	0.311510344469394\\
1.00196265849277	1.36857489729479	0.363292126884496\\
1.08499303940429	1.41039054155304	0.416193982274278\\
1.17357355895132	1.45437433853469	0.465193744115268\\
1.27108916573045	1.49585615817136	0.511198188920007\\
1.36738815203217	1.5288777946603	0.559249988865571\\
1.46459792584918	1.57099099022238	0.60704842066653\\
1.56212782255143	1.61255482846046	0.657140249559243\\
1.65101905229456	1.64009040659743	0.697355172143784\\
1.73689753157938	1.68738904946681	0.743162119241309\\
1.83612693015357	1.72298066468903	0.788077066694301\\
1.93577383028603	1.7571649821941	0.834936806521095\\
2.03580061539425	1.79740284902888	0.871827160397645\\
2.14640774918638	1.82927946907133	0.91891253168607\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00078365475287	0.23992355535741	-0.999728671012028\\
-0.935891642953166	0.300091825089731	-0.951474389462341\\
-0.87418466838095	0.346093476197099	-0.909218351198902\\
-0.812655596659914	0.38997905399921	-0.866003938379414\\
-0.752169420156563	0.43787424959484	-0.822649289058851\\
-0.693160374216775	0.485257210769055	-0.783997105360234\\
-0.633899961413753	0.536927934143049	-0.750349007416267\\
-0.578063148420872	0.585347426857786	-0.713390213594638\\
-0.522336889168724	0.633788617358528	-0.680267083935142\\
-0.466170272683795	0.679281679845899	-0.648519521131764\\
-0.413201259798065	0.729604239953143	-0.61380063664545\\
-0.356193498793296	0.777507316190032	-0.577618642803768\\
-0.300237980555567	0.824550367130647	-0.539948180551264\\
-0.239572284860228	0.872342499049926	-0.501372323047942\\
-0.180259819052109	0.922921441578816	-0.462921887665123\\
-0.121082899804986	0.974075155469182	-0.427164662472606\\
-0.0596028969316553	1.02779599155048	-0.389515978863963\\
0.00501546932763867	1.07894707697658	-0.348259722788119\\
0.0710579821881429	1.13287548301642	-0.309723734836253\\
0.14031608034427	1.18204009515857	-0.272939079172506\\
0.201524037587837	1.22856440719882	-0.238853614006538\\
0.263305609475994	1.2749900556921	-0.205138519084251\\
0.32685918959988	1.32175041691463	-0.173873034309376\\
0.391412762787077	1.3758752709622	-0.14299065739635\\
0.452820392377637	1.42970299149503	-0.115271006907894\\
0.517680455999868	1.47537224732817	-0.0883101602986723\\
0.579419045623243	1.53030767951344	-0.0581559539972585\\
0.637925300760748	1.5806756508248	-0.0350750467162361\\
0.695185422632207	1.63571118302487	-0.00440397548219863\\
0.756929900314464	1.69009717857704	0.0185571639265925\\
0.815811620634022	1.75058499785149	0.042499890303336\\
0.870765183520883	1.80180156512811	0.064911783031098\\
0.928885152338001	1.84612847431331	0.0876981845852584\\
0.989320626855028	1.90289284182915	0.104575673815243\\
1.04275871276515	1.96252053390895	0.120934328141935\\
1.09530686760527	2.02619255868345	0.1387665029957\\
1.15094350015327	2.09891026242926	0.154727215184451\\
1.20222732319365	2.16430494030975	0.169206799873526\\
1.2573556028871	2.22674555926012	0.181193062032712\\
1.31218258441105	2.28963419120086	0.191422453652016\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997765059396343	0.239368119619885	-0.998632467358541\\
-0.93937373323242	0.30214329108609	-0.949185409875145\\
-0.875430882826985	0.348818635030752	-0.899319098786669\\
-0.814920588751239	0.390444458877849	-0.849219374066013\\
-0.756449272533883	0.434456193704606	-0.804731821703027\\
-0.697587230861426	0.479936607372494	-0.758398834170475\\
-0.639413273211574	0.532570180522667	-0.716201607484398\\
-0.583250669876915	0.580930796622951	-0.66750582265269\\
-0.527361234888502	0.625535916742555	-0.619366080362518\\
-0.473860540054439	0.675138429741735	-0.573455403431676\\
-0.416842602137691	0.718787849718638	-0.526531922360328\\
-0.355517228729186	0.761941008670046	-0.481906741047513\\
-0.29924429795684	0.797860286506303	-0.43411365788437\\
-0.241579316760711	0.842665495279437	-0.38576965554492\\
-0.186214436407172	0.884510695935943	-0.33955466820198\\
-0.131472460259029	0.922322507515103	-0.291391040471825\\
-0.0818283018778097	0.965781306244273	-0.243710623772155\\
-0.0289450444715565	1.01362678155263	-0.196341134494746\\
0.0192766868295891	1.06065271318524	-0.147124525310489\\
0.0663651930763715	1.10930768509397	-0.095297947451749\\
0.117825522326872	1.15754189666042	-0.0483557043478084\\
0.164682153080368	1.20379487712617	-0.00279573383468452\\
0.211010479540805	1.25258364544966	0.0411455465734933\\
0.255594040030545	1.30692149575259	0.0922078762991131\\
0.298254564870538	1.35645848800623	0.142000608966418\\
0.342873876235389	1.40253907038574	0.189173183692991\\
0.392926276047407	1.4486794048328	0.23175092839643\\
0.43680424289492	1.48816583448801	0.276156170773253\\
0.4807378215762	1.53137364047456	0.322775513737631\\
0.526620198531542	1.56920228882126	0.359127831373691\\
0.56591489672637	1.61693229148691	0.404238742203233\\
0.610099917813616	1.65270722008485	0.447338321696072\\
0.652502599965383	1.69384746474384	0.485782584780267\\
0.700410178129929	1.73198556856864	0.52402903078929\\
0.752113576201318	1.76889797773974	0.565405797293733\\
0.801923949775538	1.80660358681109	0.605765402145737\\
0.857822291965766	1.84933557779032	0.644559486875519\\
0.914588074077971	1.88384810618892	0.689810740450099\\
0.961631798383387	1.92606158107412	0.731858711330456\\
1.0148826543844	1.96115444333319	0.774784027441618\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00124092589185	0.239816003778784	-0.998979463466204\\
-0.937288483883964	0.298652216485728	-0.947305080414681\\
-0.874324015956683	0.346679988346124	-0.895911654551714\\
-0.813086423541777	0.396488056541292	-0.843166313898894\\
-0.751010436713365	0.446269804704144	-0.78817970307042\\
-0.682882612520197	0.493528138625298	-0.736862023324279\\
-0.613861780293297	0.545395910931668	-0.682527468420955\\
-0.538838020915168	0.590867343909261	-0.625300948241179\\
-0.466039239828263	0.641714009902162	-0.569903590745812\\
-0.398667635275314	0.69222350235383	-0.520227774555629\\
-0.330008627457289	0.747162137589701	-0.46170774691253\\
-0.260499094905648	0.801375354698887	-0.40616405740866\\
-0.186767739138402	0.856294633077699	-0.351163497386381\\
-0.111019062347564	0.908056769338158	-0.294500064696019\\
-0.0350835522365496	0.958857705356086	-0.240772170645303\\
0.0426463628396927	1.0186034213848	-0.190925113936523\\
0.11791103936777	1.0705704139845	-0.141053473742598\\
0.197839296599261	1.12843363279935	-0.0872794812274623\\
0.277347790307844	1.1823768445215	-0.0310909748515738\\
0.360988620334964	1.23250037248435	0.026051780568783\\
0.438124102287111	1.27967137325163	0.0790201668357556\\
0.515206366190743	1.33008348979629	0.129780283140996\\
0.599816880653003	1.38299679982594	0.182631115781806\\
0.678888828794389	1.43166401753439	0.234165040762675\\
0.758029893448463	1.48160154547055	0.286636606059209\\
0.841015536434754	1.52993908396869	0.336523085378486\\
0.924889234355651	1.581273031991	0.381659253479001\\
1.00387249973436	1.62711092001131	0.425831594133192\\
1.08168968192146	1.67569786099973	0.463410534659372\\
1.16164203108494	1.72351386188058	0.504984800696315\\
1.23737000582405	1.77232198652142	0.549479689877577\\
1.31104377052331	1.82690193330057	0.595304293111153\\
1.38668724076	1.87766090010812	0.632646767553519\\
1.46437653667485	1.92354642765666	0.674047007503459\\
1.54456738776447	1.97765707938978	0.710337580898264\\
1.62013027426845	2.02878200653533	0.745168892467828\\
1.70279727725444	2.08362349291647	0.787683450570283\\
1.78568175922823	2.13599486884661	0.819525740697244\\
1.87154876593784	2.19139625223957	0.863728576209412\\
1.94806169574255	2.24685221306749	0.907639684684533\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.99935194721902	0.238681935338578	-0.998614880487704\\
-0.940335836971935	0.294976492649077	-0.948870499024057\\
-0.874908791475569	0.341477802018139	-0.896921152791689\\
-0.812388641867099	0.385690279888144	-0.844281874115211\\
-0.750864214281315	0.429173650735838	-0.792088891824479\\
-0.690905511463685	0.464874821347287	-0.740351533534099\\
-0.631977740516516	0.503337534656834	-0.685425691263554\\
-0.571132209431751	0.54134772890941	-0.631745062895502\\
-0.507316451248349	0.579404089114587	-0.579542816811058\\
-0.441180989267618	0.615904911165074	-0.528489391519457\\
-0.372345206888199	0.650356337398777	-0.47468554690201\\
-0.3042245244206	0.688509812480207	-0.425825793298077\\
-0.234662626611892	0.72125536451384	-0.375200019770466\\
-0.163090084788497	0.760131401500791	-0.326837971516642\\
-0.0893268737884853	0.791805202790887	-0.279677400815967\\
-0.0183310397317188	0.838870042194565	-0.230546207273301\\
0.0587946373017586	0.879888778294201	-0.187346580087519\\
0.129542188948448	0.928790274326802	-0.146944594367335\\
0.19870398092916	0.97008979090525	-0.106744648497142\\
0.268992986614762	1.00845715728851	-0.0587876227145755\\
0.342444831359641	1.05597310529209	-0.016633186444905\\
0.416066471449191	1.1013404563555	0.0303418665508237\\
0.493292186449519	1.14913228388169	0.0724549004087658\\
0.565144821047364	1.19875654035141	0.120335642148666\\
0.631988359088721	1.24445046761545	0.164866528774112\\
0.699383810166387	1.29010785268828	0.207833740504836\\
0.766648989026749	1.34489441145531	0.248559227784297\\
0.833580294365854	1.39385174978063	0.297406458174374\\
0.901497318434043	1.43850835907576	0.346483250157958\\
0.966442046604626	1.48763067637605	0.392314535904749\\
1.03047451970741	1.53159672115588	0.440687899918605\\
1.09051333003387	1.57761600039227	0.485585283586414\\
1.15272401877982	1.61953124886624	0.534540816773247\\
1.21364671499112	1.66189468245294	0.57786534400908\\
1.27806458218462	1.71141740171944	0.618109534977801\\
1.33858492863642	1.75846661187408	0.665612352640433\\
1.40684406280712	1.80841245433489	0.704197487856624\\
1.47287973581568	1.85293521433314	0.749909007172522\\
1.5436681275598	1.89714042979675	0.793034464721989\\
1.61550488564297	1.94724852083146	0.834530127630623\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999634859621356	0.239271779481475	-0.998679462684257\\
-0.936111764381054	0.296283614453489	-0.94831683958489\\
-0.879129763640786	0.344920328813215	-0.89736794283437\\
-0.820567957889284	0.392716186502721	-0.844863550836345\\
-0.765485602045061	0.443495726580834	-0.789972709196182\\
-0.71005856716443	0.497655503148952	-0.732126627113771\\
-0.659365634265378	0.550808457412839	-0.676819882311723\\
-0.604592497605471	0.606490147647145	-0.621946983750836\\
-0.55054846969073	0.651072972043645	-0.564630384875968\\
-0.499489541386082	0.699347844936272	-0.507702707992726\\
-0.446330041569933	0.7502738321523	-0.450930613005345\\
-0.396044907406805	0.798113391378133	-0.391029921300544\\
-0.338611297900659	0.849822383643951	-0.331618714582251\\
-0.280690737471354	0.894578984122785	-0.270568912008518\\
-0.224711941751689	0.93849644601338	-0.209683058849851\\
-0.16892685369019	0.986275482886221	-0.155018792153008\\
-0.111134990825546	1.02559974484507	-0.100499468719658\\
-0.0549752908328018	1.06320527674927	-0.0456769296444546\\
-0.000977872683983087	1.09666252849073	0.010302887012338\\
0.0557587964780432	1.13781354447212	0.0607750484519258\\
0.116110577061856	1.17545485565356	0.115959218816399\\
0.175691679666404	1.20992923955523	0.161901311504316\\
0.232748765770166	1.24716034135514	0.210486992358668\\
0.292881897898659	1.28045142232902	0.257209720815239\\
0.351400916583728	1.31226386929515	0.305560539142629\\
0.407759025047308	1.34674089736457	0.353242150936268\\
0.464362193982513	1.38289946352213	0.40354352753329\\
0.519806515232579	1.41766533333554	0.450756754805817\\
0.579791581474152	1.45298806998336	0.49982899465621\\
0.630330461225914	1.48939798469553	0.548791834620117\\
0.680207559994775	1.52433116639941	0.590702092131388\\
0.732210593375266	1.56916542552337	0.64101786961329\\
0.782830371440488	1.60933724902005	0.688040626190246\\
0.835222882756387	1.64714827145702	0.742395842277165\\
0.879167065106617	1.6908307056549	0.787836221186975\\
0.922554779812626	1.73442902138144	0.835343280017121\\
0.968229202375749	1.7800803062225	0.875578095160023\\
1.00468409432214	1.82122244587443	0.920233266083355\\
1.04954752099087	1.86385882139071	0.972889979690468\\
1.09424933934566	1.90572203463849	1.01571907640299\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998820335376772	0.238921318243581	-0.996969581059155\\
-0.937071634582295	0.295140179291052	-0.943756993473794\\
-0.876139596659584	0.344939806167525	-0.897342204977664\\
-0.813721266783148	0.397691538934039	-0.841597462365402\\
-0.748021699902443	0.445484609128519	-0.78301767507068\\
-0.685043459105533	0.499721975901537	-0.73103355466423\\
-0.618842846105844	0.547120151214652	-0.677477946235264\\
-0.546844142562826	0.587095564076127	-0.623561101067313\\
-0.46823195206458	0.632124148862021	-0.571199447699018\\
-0.395515238202973	0.675072970046032	-0.520880772337115\\
-0.319938529664889	0.713615139425768	-0.465927183386198\\
-0.243211956264313	0.752923796959993	-0.410387217377009\\
-0.168155245938329	0.790597964672429	-0.354645879879868\\
-0.0958117218807896	0.829815104746962	-0.301180641105088\\
-0.0259715780474841	0.860550878588039	-0.246873953464595\\
0.0421023788172709	0.904274596508869	-0.195717790601222\\
0.113715180511701	0.951859870071415	-0.141406863864737\\
0.184706948439921	0.997536369595875	-0.091462727889696\\
0.249250946848064	1.04057469957017	-0.0424766261122953\\
0.320079487574856	1.08890931768402	0.0106434234306132\\
0.392174896817315	1.13407108515269	0.0610073539818095\\
0.457136971874876	1.17454222116694	0.112058158005418\\
0.519428042632615	1.22245260767292	0.160549911540699\\
0.584663574066972	1.2627042345698	0.209544686831594\\
0.649822494004643	1.32118306801154	0.26012615385116\\
0.719907162719835	1.36934072698426	0.307409175359373\\
0.78338103065916	1.41597416906786	0.356188806277736\\
0.847678004201852	1.46567996380167	0.406173497391645\\
0.913221152014442	1.5151702694116	0.460843008360163\\
0.98030984083085	1.55695937707148	0.517205072955565\\
1.03952857790341	1.60332881896411	0.571317714147402\\
1.09798755174183	1.65011344344005	0.625106222583626\\
1.1643635454599	1.69280340409992	0.676078149923056\\
1.22877548910632	1.7465278474927	0.734725491744017\\
1.29305008212906	1.79291020122233	0.784666086452308\\
1.36131578464863	1.85129472235578	0.837823693033084\\
1.42229886754359	1.90412508397255	0.884608592598434\\
1.49063846924171	1.9581272450955	0.931869184869564\\
1.56626535556546	2.02545736600662	0.976794527451747\\
1.63564991973717	2.07397037829095	1.02263920234139\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.998141641676941	0.240967974914197	-1.00104573129492\\
-0.940289965417701	0.296436333508483	-0.951756290257576\\
-0.880642106735884	0.346193713113848	-0.90194032523838\\
-0.823903869886611	0.394281991098614	-0.848688414968544\\
-0.774515055117073	0.44663042020815	-0.795615391257305\\
-0.718953555876818	0.493396837258269	-0.743592861836015\\
-0.663014760487011	0.540758853407822	-0.691942101793505\\
-0.604643703120425	0.584821925667062	-0.643936819934352\\
-0.551142793187199	0.635150151318448	-0.599578378844916\\
-0.493137791939963	0.678849867648144	-0.552117599593888\\
-0.438176982506915	0.724377433661882	-0.502596057358096\\
-0.381608546230655	0.766878362948332	-0.449712819452601\\
-0.324235174831834	0.806449695532166	-0.399555125349189\\
-0.264110604083804	0.850979232727021	-0.350140378946814\\
-0.206512661124915	0.894379517090073	-0.301081461622054\\
-0.154237726861326	0.941430839990925	-0.250857608285135\\
-0.10086694970637	0.98442856337781	-0.201758719189176\\
-0.0459965825642973	1.03030334795318	-0.152779607595599\\
0.0108273687164005	1.07162883151285	-0.108031767186483\\
0.0630459839546758	1.12172448432462	-0.0640373791277421\\
0.114140364546358	1.16516459074779	-0.0185712643445556\\
0.167483057058572	1.21027796183965	0.0260149100624995\\
0.22499017885151	1.26023140779112	0.0689347587561598\\
0.275815418455338	1.30780796524357	0.112388677324613\\
0.329024379692852	1.35324196944629	0.15361027360572\\
0.38405613968104	1.39732267347827	0.192652958101126\\
0.440666272778179	1.44568166461066	0.23004812488495\\
0.497406879657085	1.49283470924521	0.275313496475246\\
0.559461237584241	1.5377608107421	0.31895704973692\\
0.623380174570776	1.58877975853588	0.360598797189408\\
0.693562409807554	1.62522930427611	0.403593824844869\\
0.765342611122525	1.66695834452229	0.44944560983481\\
0.83752062084654	1.71001844620491	0.494724077995049\\
0.908406001396094	1.75106936413118	0.55064618493569\\
0.983922390329083	1.78547007538123	0.597413206791784\\
1.05826693551764	1.82043870407701	0.655931597015267\\
1.13113499572271	1.85605619904299	0.708403706593457\\
1.20619129348005	1.88540233292976	0.755280510916421\\
1.28143016981168	1.91792636176267	0.811799247013876\\
1.3578558127962	1.94481149689388	0.868215907014479\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999379532098069	0.241223723327276	-0.999920084408998\\
-0.93492165331174	0.295914305409757	-0.946124244297636\\
-0.874994082955451	0.343031763381411	-0.894850305142999\\
-0.809094593462341	0.385981203187363	-0.841311767072062\\
-0.750513715131491	0.435396407421481	-0.789834135005093\\
-0.687586902390309	0.480360499957345	-0.736112328938023\\
-0.632691069686544	0.526903928045293	-0.681665340098762\\
-0.577944258981679	0.572691468807821	-0.626757505663241\\
-0.525543804283991	0.618660045578255	-0.57429801599278\\
-0.473354545274657	0.664572066760024	-0.518335892726232\\
-0.416061773757111	0.71889625048144	-0.461207246992515\\
-0.357857832172204	0.765455440821941	-0.3978378972767\\
-0.302274939986316	0.816627044511738	-0.335877313033306\\
-0.247947521476374	0.862266087482545	-0.275042145613876\\
-0.199879405995406	0.904374457595352	-0.216176381583011\\
-0.156466604454471	0.945687096831013	-0.154985257768373\\
-0.112194634728078	0.992549864846286	-0.0905928258134019\\
-0.0691812259949483	1.03655867008954	-0.0319964039603638\\
-0.0231554325911002	1.07949726980244	0.0243611132704072\\
0.025900862016675	1.12645333379324	0.0791319056483098\\
0.0718501885869285	1.16993008852809	0.136942515132676\\
0.119671273213875	1.21654756500959	0.19367263401488\\
0.168020561329555	1.25850470482246	0.244341762240554\\
0.21802461144304	1.30164387328126	0.304327430250959\\
0.270951950541524	1.34508155835582	0.357294114281204\\
0.321030143896179	1.39422266287677	0.409521576158534\\
0.377994998122363	1.43741189245949	0.461461115991604\\
0.435859567248624	1.48389534083306	0.514845197059223\\
0.496265467782873	1.53040445464621	0.565186714389318\\
0.556299039976345	1.58255010062908	0.615363436602804\\
0.617047681951464	1.63552058297951	0.669227994220004\\
0.680907093515907	1.6872794052462	0.719695355352909\\
0.742044735390273	1.7413481484156	0.76984166661847\\
0.802018594842547	1.79214191244091	0.820403165860948\\
0.859282127973218	1.84274059100774	0.872457664819439\\
0.916853818852517	1.89879759749512	0.931304340332778\\
0.975616134558948	1.9593164400295	0.987942311220517\\
1.02881600198417	2.02219584921213	1.04481651384734\\
1.0832693049385	2.08176642178776	1.09728417561781\\
1.13277286916824	2.14841003268375	1.15596800117175\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.999692310620872	0.239927674033235	-0.999472432615463\\
-0.933209819728707	0.294748472255955	-0.952261281905421\\
-0.868577711023995	0.335765656725296	-0.904340802739909\\
-0.799092069724105	0.377827820415651	-0.853678993657259\\
-0.727332144761213	0.422970624041353	-0.807275525685005\\
-0.655851728054118	0.473916580110526	-0.75888187800323\\
-0.587001768519097	0.520084917967592	-0.707430624155749\\
-0.515955211025173	0.567453846966708	-0.656195506366815\\
-0.446198405426685	0.612821995961846	-0.605449946997307\\
-0.373250218732531	0.65216923049297	-0.554816287316858\\
-0.299296176120974	0.690687677149231	-0.501713936178241\\
-0.223971979258598	0.729535119464636	-0.449265513717634\\
-0.152145543292195	0.762859695512808	-0.393640208907787\\
-0.077939023765532	0.792386590549032	-0.334102158390686\\
-0.00772147692959863	0.820768415406884	-0.276871959717681\\
0.0610432880036605	0.845364995915679	-0.214686061882883\\
0.129184138865217	0.869133626882791	-0.159136365829675\\
0.197104110175878	0.898505083067777	-0.105594134850437\\
0.263868304657298	0.92054046392094	-0.0480516806394047\\
0.333409676023692	0.947021412351271	0.00319140706745683\\
0.403062971142568	0.970883716135543	0.0584373869445038\\
0.475682004816493	0.995920020940746	0.11412895053286\\
0.5449443372319	1.01752848431982	0.163525375301499\\
0.610392438290691	1.03998945592692	0.216423960829373\\
0.674330360522012	1.06938989168373	0.271322847711803\\
0.738445814596909	1.09437680542196	0.328401356808452\\
0.801823353084034	1.11926185706369	0.381847195154675\\
0.864314845733103	1.14190470530954	0.438691398473727\\
0.920222809590428	1.16666620393811	0.485574912785679\\
0.977558104172646	1.19310145446199	0.534438156242062\\
1.03463157503337	1.21726284661055	0.580998946992507\\
1.08685230105948	1.23856160545643	0.627852252630681\\
1.13793081805297	1.2593147644309	0.677243817230983\\
1.19545577295665	1.27798699002787	0.728361159733363\\
1.24754004030227	1.30250091317863	0.776440145446456\\
1.30191549833444	1.31824391475217	0.821097606228413\\
1.3575995649498	1.34538921661929	0.86869134821583\\
1.40889647097055	1.37273800670513	0.914263774778509\\
1.46259078616865	1.39435947213133	0.958178684058967\\
1.5196290196583	1.41998842495514	0.99970630630871\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.0008872540537	0.241432926064298	-0.996633556315726\\
-0.937172206737194	0.303169074359908	-0.953146360197932\\
-0.877023053451693	0.345234437205845	-0.905475789191137\\
-0.811349230914318	0.393087850027326	-0.857675931327085\\
-0.748557536889076	0.43950763832727	-0.807468564276365\\
-0.690821605453801	0.49064589322845	-0.757118489027448\\
-0.631296132199868	0.538810205812094	-0.707828558577903\\
-0.571461507142488	0.585759839128613	-0.661269483166922\\
-0.513408007728163	0.6381450439303	-0.610789885088859\\
-0.455146235541629	0.688970344751322	-0.55923029660364\\
-0.401220864936343	0.745194904194207	-0.512607935279978\\
-0.342709330464797	0.798349645315461	-0.463116163216725\\
-0.282164833815141	0.856037033053808	-0.41532914635638\\
-0.222468242143816	0.917796548686238	-0.361975760192633\\
-0.165045956534996	0.981677973042248	-0.309740304771138\\
-0.108364342811272	1.04652973304131	-0.257534753134524\\
-0.0587552517817292	1.11217382389008	-0.206808854252477\\
-0.00200931185334325	1.17737973156386	-0.155243031753258\\
0.0562196644555416	1.24351072637553	-0.100664547768488\\
0.114940699105903	1.30766965566372	-0.0488840862162478\\
0.170919506281538	1.37229158082352	0.00453343930163976\\
0.226041481777202	1.44372672196622	0.0567280100758777\\
0.282446284908058	1.50867484967037	0.110299882473515\\
0.340083934919905	1.57077561906573	0.161165948861961\\
0.390407734954244	1.64136285524902	0.206372763361386\\
0.445499308068681	1.71892544365508	0.255642234222136\\
0.498051206182195	1.79675195542776	0.306691133636599\\
0.551553624648943	1.87939959894694	0.353772234579832\\
0.601596043468437	1.95851317361973	0.403985923034679\\
0.65806362583231	2.04401454564946	0.452116753343756\\
0.709241154377718	2.12176029890201	0.506249261000002\\
0.755720320081895	2.20270713280254	0.554394415598567\\
0.800217191516422	2.29846251561385	0.602512599047508\\
0.852456529453143	2.37994727284175	0.654591488133874\\
0.894773629436084	2.45194429646527	0.712713921456089\\
0.940881650942463	2.5302859323334	0.758885602116381\\
0.985561789341494	2.60697507286057	0.807825988608978\\
1.02382142933863	2.67772575072283	0.853294196716483\\
1.06953942346816	2.75370739644224	0.901880082748034\\
1.12365698166703	2.83573277421499	0.944352229336189\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00082743567633	0.238885170251025	-0.996206865027175\\
-0.940817417922833	0.296881056563082	-0.948557069637876\\
-0.881878366995346	0.35101660361673	-0.897637455255167\\
-0.819402456815038	0.400725296794156	-0.842970874700834\\
-0.758599621810355	0.455218953359551	-0.782301494425766\\
-0.698250709671254	0.516697996269605	-0.724683641260743\\
-0.642195280607129	0.574935395397737	-0.660382756763835\\
-0.591977079946194	0.635209516502012	-0.596605906885547\\
-0.540601864243441	0.701893624195876	-0.534844301705328\\
-0.48334891784124	0.764034702508068	-0.471390740652786\\
-0.429295032459792	0.827783704820473	-0.407844601893901\\
-0.373027477484754	0.899178055716306	-0.347857776586655\\
-0.319733916661838	0.966387419444043	-0.285557069314635\\
-0.268251566022367	1.02707986125062	-0.22193314363696\\
-0.221575564879888	1.09072701171127	-0.160646300653345\\
-0.167831926242652	1.14869201584876	-0.0979971288513163\\
-0.114306874366952	1.21188288584621	-0.039256381790911\\
-0.0568484378683423	1.27135149170009	0.0208765077156277\\
-0.00269477784702398	1.33240485248897	0.0767110264607232\\
0.0553665454390656	1.39401571314772	0.130330605519855\\
0.102977587419805	1.44898789224728	0.183197551203754\\
0.15567900311223	1.50842486891107	0.235722722361896\\
0.207823061891058	1.56571513228968	0.28555200706942\\
0.255135614146583	1.61638481097362	0.337960088325288\\
0.304790259240445	1.67414838607076	0.384614022381312\\
0.355903086354957	1.73159358461473	0.439592646541742\\
0.406634016269651	1.7868743930437	0.491809721004599\\
0.460914263153398	1.8343807011135	0.543374422784016\\
0.511542861930725	1.88494950697514	0.592598079622089\\
0.565263290721416	1.93961102731021	0.646332373128015\\
0.616981555691952	1.99077201622695	0.702819101503462\\
0.671197567301063	2.04015319134609	0.760803284275124\\
0.726075240116637	2.10650310794462	0.81718418991772\\
0.783255221024317	2.16623585687345	0.865259934274922\\
0.853000676037957	2.22763775186827	0.917531008264735\\
0.913478824212786	2.29682918743265	0.966696296980674\\
0.969452970558019	2.36517560733474	1.02015598397779\\
1.02946830395265	2.4281140161147	1.0748752797848\\
1.09250649588298	2.49312186411354	1.13649164958425\\
1.14801020465013	2.55986789988781	1.19054503258881\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00008317066648	0.242834635470484	-0.999899041095014\\
-0.939346175301803	0.296314821407122	-0.949410557679027\\
-0.880099002568571	0.343752438190296	-0.906356273050507\\
-0.824651746555369	0.391426348091208	-0.859385172836208\\
-0.771442787411484	0.437491768170075	-0.813425413378958\\
-0.714945218902297	0.485506554465226	-0.766641089437531\\
-0.662834128060215	0.534399092098705	-0.716416013327529\\
-0.608251504078102	0.584689137110478	-0.662707721076069\\
-0.554193738412495	0.631881020127409	-0.610628535553922\\
-0.500856522659415	0.673592449757168	-0.557450907962817\\
-0.446866294993415	0.723393243569409	-0.508738522550848\\
-0.392892391536904	0.770496439283146	-0.464306520964812\\
-0.333205082199676	0.82227573006045	-0.41442530380006\\
-0.276525099730795	0.873340341902548	-0.362061970649051\\
-0.223084849807473	0.92940436471091	-0.311476610522187\\
-0.168194829036812	0.98411040994248	-0.256843284268853\\
-0.107695320415129	1.04428466753511	-0.203963361014592\\
-0.0511222109411478	1.1030549491784	-0.157362670295097\\
0.00767296756030962	1.15454670598118	-0.108365094141501\\
0.0652733523734312	1.20667399690555	-0.0580264467290626\\
0.124304356030193	1.25576257928068	-0.00255882061443522\\
0.184480909991661	1.30970698496415	0.0576169470209865\\
0.248308933665813	1.35810446897833	0.119255205753347\\
0.312381494076611	1.41291239064518	0.184709998448736\\
0.375793362004162	1.45854951669542	0.249077833742865\\
0.436653862834686	1.50533424380876	0.309392810111666\\
0.502277859071436	1.55091135955666	0.373128960529219\\
0.571816446990701	1.60072996369009	0.437708227074967\\
0.640634339259514	1.64180824132921	0.503741223253932\\
0.702863475564713	1.6938980380019	0.569547105290018\\
0.767703523237002	1.74477144201522	0.640765705504502\\
0.838987846409415	1.80057861810469	0.716908063729262\\
0.905544002759294	1.8570284413532	0.787790908144922\\
0.975474719821674	1.91674420466195	0.86644919650893\\
1.04026145249735	1.96817372844567	0.940443625728088\\
1.10619586999997	2.02246670642592	1.00891639137243\\
1.16765686988811	2.06939376269636	1.07931471959946\\
1.23573994474283	2.12443111378121	1.14497919445465\\
1.30158775659136	2.17076864519567	1.20471193671836\\
1.3671983888644	2.21714675790961	1.25959274581551\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-1.00020775695172	0.241752468326017	-0.998207411825569\\
-0.935412660457032	0.293829513775434	-0.945800936610767\\
-0.871239674859816	0.336606502333263	-0.896456181201684\\
-0.808541806413232	0.383791459409964	-0.843740034979626\\
-0.747295722993108	0.428188110837707	-0.787160495564368\\
-0.685957354453649	0.471724817867047	-0.728515526449395\\
-0.624326120910088	0.517746242483975	-0.671694126636045\\
-0.565079026375145	0.5647115272411	-0.616493908649543\\
-0.506665091639353	0.612639196436584	-0.562975793784745\\
-0.450662943200388	0.666281371968875	-0.514734149996427\\
-0.390564184894974	0.713579958084468	-0.4687636267017\\
-0.332438751806191	0.765269474638649	-0.424816335969826\\
-0.271536519170302	0.817951094590046	-0.383183921346484\\
-0.209292031525921	0.870531366154017	-0.339336111957847\\
-0.146875008068577	0.920883730011517	-0.292182145126404\\
-0.0830619297188933	0.967117923257754	-0.24622403560658\\
-0.0190025917659913	1.01543061657803	-0.197558077179422\\
0.0463146252773338	1.0665823738543	-0.147657825204193\\
0.107590326974069	1.11861402453776	-0.0985198091543596\\
0.172196688471171	1.17227969641039	-0.05130621956541\\
0.237663158652785	1.22669549039476	-0.00404275707666333\\
0.307380372152273	1.28342599295708	0.0408935012984167\\
0.3796894396644	1.33444743074769	0.0868261666490223\\
0.454845401889092	1.38895559911942	0.132489653079162\\
0.531622067764118	1.44535519983395	0.176263967132718\\
0.601800283013693	1.49885816783364	0.222326432057736\\
0.676908940749516	1.55113522791756	0.268860502759302\\
0.748302461751008	1.60708930892292	0.312574123220425\\
0.817069811649118	1.65967719847086	0.356537006104763\\
0.886239338921974	1.71254464257122	0.407946342020007\\
0.957336911433076	1.75698937713088	0.451327092603668\\
1.030913206791	1.79956243382572	0.495754502256299\\
1.1073219333597	1.8619595214226	0.549421259363623\\
1.18463833455541	1.90987749375411	0.603452648070007\\
1.25684062884056	1.96240220296043	0.65338077251216\\
1.32739545930923	2.02083954535988	0.703923561802601\\
1.39664955208251	2.07153467299757	0.755171261002132\\
1.4642169515537	2.13032785613182	0.807560154139646\\
1.54029054503522	2.18966417491797	0.862873472463479\\
1.60160131632678	2.23871556754639	0.910406606830474\\
};
 \addplot3 [color=black, line width=0.08pt, draw opacity=0.3]
 table[row sep=crcr] {%
-0.997497770797953	0.241338622250135	-0.997689821932872\\
-0.935305408722999	0.297768099946843	-0.949867904844403\\
-0.875335708765558	0.342110242819317	-0.901852183933097\\
-0.815849241962318	0.393494416689344	-0.8581953643271\\
-0.757742463920341	0.434221336330512	-0.814672587605776\\
-0.699074320449531	0.477099486565259	-0.772991064002535\\
-0.640336141124177	0.512716515695571	-0.727457110946281\\
-0.575840145144716	0.548120828302769	-0.681013638705464\\
-0.518686074606721	0.587661264146064	-0.632144825901329\\
-0.460136356239959	0.622039593487913	-0.585035216907204\\
-0.405973766081343	0.659569930648631	-0.535321942193913\\
-0.351197114697678	0.69908797156257	-0.485978198919754\\
-0.296672365262517	0.734122246153381	-0.438880075596537\\
-0.242053822006569	0.765820407948098	-0.388312838826704\\
-0.186553322901428	0.797359101361913	-0.337177588026869\\
-0.132205049122026	0.834877891222277	-0.287265621766334\\
-0.0820790894718472	0.872534512104874	-0.236114342486902\\
-0.0360199003929473	0.902788813015577	-0.184077630742093\\
0.014504698540903	0.942014452743439	-0.126699027959907\\
0.0580565922504901	0.97575901111624	-0.0709197961710588\\
0.108704760710776	1.01065614913078	-0.0158575813236208\\
0.162441128017141	1.04281582328382	0.0350139541656995\\
0.211868799919124	1.07835584954129	0.0895762618026884\\
0.267614654424767	1.11508846064413	0.145417667938227\\
0.321295401555564	1.14590299024124	0.196990341840391\\
0.376017110984062	1.17830678585824	0.251811820578513\\
0.424864898874264	1.21009749242554	0.306463046234224\\
0.474134593098504	1.24102549811481	0.36185673587438\\
0.526208333874866	1.27205964880837	0.416768847238454\\
0.575730902605529	1.3043520829736	0.468890479567695\\
0.63048359626773	1.34259998022593	0.52301232229123\\
0.681910995817487	1.37421245082713	0.579085006821283\\
0.733135676836192	1.40693314636095	0.636641263658516\\
0.776524622534419	1.44108002332212	0.686512503131546\\
0.8293758470028	1.47087445357308	0.75200471300118\\
0.878038599561469	1.49615492704504	0.809110371381686\\
0.929546584371171	1.5283081672303	0.870945893273693\\
0.979460470974572	1.56142999572212	0.933079533889153\\
1.0321669016887	1.58884239567125	0.998263790334524\\
1.08094257537962	1.62718464447431	1.05514064333366\\
};
\label{pgf:realized-trajectories}



==> figures/results/visibility.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.


\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  legend style={font=\scriptsize},
  tick label style={font=\footnotesize},
}}


\def\datapath{./figures/data}   % path to data files

\begin{tikzpicture}

\begin{axis}[%
width=0.465\figurewidth,
height=0.485\figureheight,
at={(0\figurewidth,0.5\figureheight)},
name=boundaryLeft,  % [B] defined for custom "legend"
axis line style = thick,	% [B] thick axis lines 
scale only axis,
xmin=1,
xmax=200,
%xlabel={Step $n$},                     % [B] remove x-axis label
xticklabel=\empty,                      % [B] remove x-axis tick annotation
ymin=0,
ymax=5.5,
ytick = {0,1,...,5.5},
ylabel={Num. paths},
tick align=inside,
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 1, 
    major grid style={very thin, lightgray!50}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\addplot [color=white!70!black, line width=2.0pt,line join=round, line cap=round]
  table{\datapath/visibilities/vis-coh-det-j1.dat};%
    \label{pgf:vis-coh}

\addplot [color=IEEEgreen, line width=0.7pt,line join=round, line cap=round]
table{\datapath/visibilities/sum-exist-prob-j1.dat};%
    \label{pgf:sum-exist-prob}

\node[above left, align=right,font={\footnotesize},fill=white,
opacity=0.9,inner sep=0.75mm, xshift=0.5mm, yshift=-0.7mm, draw, line width = 0.8pt] at %
(axis cs:200,0){a) $j\!=\!1$};

\end{axis}

\begin{axis}[%
width=0.465\figurewidth,
height=0.485\figureheight,
at={(0.475\figurewidth,0.5\figureheight)},
name=boundaryRight,  % [B] defined for custom "legend"
axis line style = thick,	% [B] thick axis lines 
scale only axis,
xmin=1,
xmax=199,
%xlabel={Step $n$},                     % [B] remove x-axis label
xticklabel=\empty,                      % [B] remove x-axis tick annotation
ymin=0,
ymax=5.5,
ytick = {0,1,...,5.5},
%ylabel={Num. paths},                % [B] remove y-axis label
yticklabel=\empty,                      % [B] remove y-axis tick annotation
tick align=inside,
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 1, 
    major grid style={very thin, lightgray!50}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\addplot [color=white!70!black, line width=2.0pt,line join=round, line cap=round]
  table{\datapath/visibilities/vis-coh-det-j2.dat};%
    %\label{pgf:vis-coh}

\addplot [color=IEEEgreen, line width=0.7pt,line join=round, line cap=round]
table{\datapath/visibilities/sum-exist-prob-j2.dat};%
    %\label{pgf:sum-exist-prob}
    
\node[above left, align=right,font={\footnotesize},fill=white,
opacity=0.9,inner sep=0.75mm, xshift=0.5mm, yshift=-0.7mm, draw, line width = 0.8pt] at %
(axis cs:200,0){b) $j\!=\!2$};

\end{axis}

\begin{axis}[%
width=0.465\figurewidth,
height=0.485\figureheight,
at={(0\figurewidth,0\figureheight)},
axis line style = thick,	% [B] thick axis lines 
scale only axis,
xmin=1,
xmax=200,
xlabel={Step $n$},
ymin=0,
ymax=5.5,
ytick = {0,1,...,5.5},
yticklabels={0,1,...,4},
ylabel={Num. paths},
tick align=inside,
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 1, 
    major grid style={very thin, lightgray!50}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\addplot [color=white!70!black, line width=2.0pt,line join=round, line cap=round]
  table{\datapath/visibilities/vis-coh-det-j3.dat};%
    %\label{pgf:vis-coh}

\addplot [color=IEEEgreen, line width=0.7pt,line join=round, line cap=round]
table{\datapath/visibilities/sum-exist-prob-j3.dat};%
    %\label{pgf:sum-exist-prob}

\node[above left, align=right,font={\footnotesize},fill=white,
opacity=0.9,inner sep=0.75mm, xshift=0.5mm, yshift=-0.7mm, draw, line width = 0.8pt] at %
(axis cs:200,0){c) $j\!=\!3$};
\end{axis}

\begin{axis}[%
width=0.465\figurewidth,
height=0.485\figureheight,
at={(0.475\figurewidth,0\figureheight)},
axis line style = thick,	% [B] thick axis lines 
scale only axis,
xmin=1,
xmax=199,
xlabel={Step $n$},
ymin=0,
ymax=5.5,
ytick = {0,1,...,5.5},
yticklabels={0,1,...,4},
%ylabel={Num. paths},
%ylabel={Num. paths},                % [B] remove y-axis label
yticklabel=\empty,                      % [B] remove y-axis tick annotation
tick align=inside,
grid=both, 
    minor grid style={ultra thin, lightgray!20}, 
    minor x tick num = 4, 
    minor y tick num = 1, 
    major grid style={very thin, lightgray!50}
]
\pgfplotsset{every major tick/.append style={-Triangle Cap,thick},thick}

\addplot [color=white!70!black, line width=2.0pt,line join=round, line cap=round]
  table{\datapath/visibilities/vis-coh-det-j4.dat};%
    %\label{pgf:vis-coh}

\addplot [color=IEEEgreen, line width=0.7pt,line join=round, line cap=round]
table{\datapath/visibilities/sum-exist-prob-j4.dat};%
    %\label{pgf:sum-exist-prob}

\node[above left, align=right,font={\footnotesize},fill=white,
opacity=0.9,inner sep=0.75mm, xshift=0.5mm, yshift=-0.7mm, draw, line width = 0.8pt] at %
(axis cs:200,0){d) $j\!=\!4$};

\end{axis}

\node[below,draw,thick,fill=white,inner sep=0pt,above right=0.0em,line cap = round, fill opacity=0.8, text opacity = 1, draw opacity = 1 , yshift = 2.5mm, minimum height=0.4cm, fit = (boundaryLeft.north west) (boundaryRight.north east)] %at (boundaryLeft.north west) 
{~\vspace{-3mm}

\footnotesize
    \setlength{\tabcolsep}{3pt} % Default is 6pt
    \begin{tabular}{rl|rl} %\footnotesize
    \ref{pgf:vis-coh} & true num. vis. paths &
    \ref{pgf:sum-exist-prob} & existence prob. sum \,
    \end{tabular}};
    
\end{tikzpicture}%

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
